Dark Matter Phenomenology: Sterile Neutrino Portal and Gravitational Portal in Extra-Dimensions

The Standard Model of Fundamental Interactions (SM) represents one of the most precise theories in physics. Among the predictions of the SM we find, for instance, the anomalous magnetic moment of the electron $a_e = 0.001159652181643(764)$. This prediction agrees with the experimental results to more than ten significant digits, the most accurate prediction in the history of physics. However, nowadays we have several evidences that the SM only explains $5 \%$ of the matter content of the Universe. The other $95 \%$ are composed by the so-called Dark Energy and Dark Matter. As their names suggest, the nature of these two components of the energy/matter content of the Universe is still unclear and represents one of the most important challenges for the particle physicists. In this Thesis we have focused in the study of the phenomenology of one of these mysterious components of the Universe, the Dark Matter. Although we have many evidences of its existence, this new type of matter has not been detected yet. As a consequence, the landscape of the models that can explain the Dark Matter properties is huge. In the present work we propose and study several Dark Matter models, setting limits by using experimental results.

==> Chapters/Acknowledgements/Acknowledgements_plain.tex <==

\chapter*{Acknowledgements}
\addcontentsline{toc}{chapter}{Acknowledgements}  

Many! To be written!

==> Chapters/Chapter7NR.tex <==
\chapter{Summary of the Results}
\label{sec:summary}
%####################################################################
%####################################################################
In Chapters \ref{sec:SM} to \ref{sec:ED} a summary of the most relevant aspects of the Dark Matter and Extra-Dimensions has been made. The aim of the introduction is to offer the tools needed to understand the different models that compose the original work of this Thesis.
In this Chapter on the other hand, we summarize the basic ideas and results of the four papers that \nr{constitute} the second part of the Thesis. Technical details can be found in the complete \n {articles that are collected } in Part \ref{sec:papers}.

\section{Probing the sterile neutrino portal to Dark Matter with $\gamma$-rays}

One of the great open problems in high-energy physics is Dark Matter, but, as we commented in Sect.~\ref{sec:openproblems}, it is not the only one. Among the various problems that currently exist in the Standard Model of particles, one of them is the neutrino masses. The model as it is predicts zero mass for them. However, neutrino oscillations was suggested more than half a century ago as distinctive signature of neutrino masses. This curious effect, which has been observed practically since the moment it was predicted, consists of a quantum-mechanical oscillation in the leptonic flavor. The phenomenon has deep implications: the effect can only happen if at least two of the three SM neutrino are massive. However, the mass of these particles must be much smaller than the SM masses in order to scape observation. \nr{las oscilaciones pueden existir si solo un neutrino fuera masivo, lo que pasa es que no explicaria que se vean en neutrinos atmosfericos y solares, pero eso es diferente}
This fact favoured the development of models in which the mass of the neutrinos are generated by the so-called \textit{seesaw mechanisms}. In Sect.~\ref{sec:neutrinomasses} a small review about  this topic can be found.

The attempt to solve both, the Dark Matter and the neutrino mass problems, at the same time\footnote{The most economical scenario, namely that the sterile neutrinos constitute the DM \cite{Dodelson:1993je}, has been thoroughly studied \cite{Adhikari:2016bei}.} led to the development of models with a \textit{sterile neutrino portal to dark matter} \cite{Escudero:2016tzx,Macias:2015cna,Escudero:2016ksa}. This \nr{scenario} has been studied by several authors, putting limits on it using Direct Detection experiments. \nr{y tambien indirect, los papers que nos chafaron el nuestro}. However, it is a very interesting model from the point of view of Indirect Detection for different reasons (see Sects.~\ref{Sec:DD} and \ref{Sec:ID} for details on DD and ID). On the one hand, Direct Detection does not happen at the lowest order in perturbation theory. As a consequence, the limits on the model due to Direct Detection experiments are worse than in other models. On the other hand, the connection of sterile neutrinos with active neutrinos causes Dark Matter annihilations to produce \nr{quitar: (excesses of)} photons and charged particles, as a result of several decays. All this makes it the perfect candidate to be studied from the point of view of Indirect Detection, as we have done in Ref.~\cite{Folgado:2018qlv}.

\nr{We analyze a particular model in which,} besides the sterile neutrinos, the SM is extended by a dark sector that contains a scalar field 
$\phi$ and a fermion $\Psi$. These fields are both singlets of the SM gauge group but charged under a dark sector symmetry group, $ G_{dark}$, such that the combination $ \overline{\Psi} \phi$ is a singlet of this hidden symmetry. 

\begin{figure}[htbp]
\centering
\includegraphics[width=120mm]{figures/resultados_paper_1.pdf}
\caption[Results from \textit{Probing the sterile neutrino portal to Dark Matter with $\gamma$-rays}.]{\it Limits over the \textit{sterile neutrino portal to Dark Matter} model in the sterile neutrino and DM masses space ($M_\psi,M_N$). The yellow region shows the antiproton limits, whereas the blue region are the DSphs limits. The different contours represent the region where the GCE can be fitted with its respective $p$-value (with increasing $p$-value going from outer to inner contours). Finally, the blue-dashed line shows our prediction about the foreseen future limit from the DSphs in the next 15 years the Fermi-LAT experiment.}
 \label{fig:resultados_paper_1_ingles}
\end{figure}

The lighter of the two dark particles ($\phi$ and $\Psi$) turns out to be stable if all SM particles, as well as the sterile neutrinos, are singlets of $ G_{dark}$, \nr{(disregarding) irrespective of} the nature of the dark group. The stable particle is a good DM candidate. We assume for simplicity that the dark symmetry $G_{dark}$ is a global symmetry at low energies, although \nr{quitar:(our analysis is equally valid whether it is local) we do not expect significant changes in our analysis if it were local.}

The most relevant terms in the lagrangian are given by:
\bea
\mathcal{L} &=& \mu_H^2 H^\dagger H - \lambda_H (H^\dagger H)^2  -
\mu_\phi^2 \phi^\dagger \phi - \lambda_\phi (\phi^\dagger \phi)^2 - 
\lambda_{H\phi} (H^\dagger H) \, (\phi^\dagger \phi)   
\nonumber \\
&-&\left( \phi \overline{\Psi}(  \lambda_a +  \lambda_p \gamma_5) N 
 + Y \overline {L}_L H N_{R}  + {\rm h.c.}  \right)  \, .
\eea
The Yukawa couplings $Y$ between the right-handed fermions $N_R$ and the SM leptons lead to masses for the active neutrinos after electroweak symmetry breaking, via type I seesaw mechanism. Although at least two sterile neutrinos are required to generate the neutrino masses observed in oscillations, in our analysis we consider that only one species is lighter than the DM and therefore relevant for the determination of its relic abundance and indirect searches. The results can be easily extended to the case of two or more sterile neutrinos lighter than the DM. Under the assumption that the DM  is described by the fermionic field $\Psi$ (the analysis would be valid also if dark matter were $\phi$) the masses of the model fulfill of the relation $m_N < m_\Psi < m_\phi$.

Fig.~\ref{fig:resultados_paper_1_ingles} summarizes the final results of our analysis. 
\nr{quitar:(Under the assumption that the DM is WIMP and the mass of the scalar mediator field is always the one needed to obtain the correct relic abundance )
 Fixing the  mass of the scalar mediator field such as to obtain the correct relic abundance via the freeze-out mechanism
(this means $\langle \sigma \, v \rangle \sim 2 \times 10^{-26} cm^3/s$), }
the figure shows the different limits from photons and antiprotons  in the parameter space $(M_N,M_\Psi)$. As it has been commented in Sect.~\ref{sec:GCE}, the Fermi-LAT experiment has reported a Galaxy-Center $\gamma$-ray Excess (GCE). The studied model predicts a photon excess that can be compatible with the GCE in to small region of the parameter space $(M_N,M_\Psi)$. The contour areas in Fig.~\ref{fig:resultados_paper_1_ingles} show the region where this is possible with different $p$-values (where the inner contours have a lower $p$-value than the outer contours). However, the extra photons predicted by the model must also be compatible with the rest of the measurements made on the different photon fluxes. Specifically, the same experiment performs measurements on the $\gamma$-rays from 15 different dwarf spheroidal galaxies\footnote{See Sect.~\ref{sec:gammaraysearches} for more information about this measurement.} (DSphs). The dark blue-shaded region shows the area of the parameter space in which the results obtained are not compatible with these measurements.
On the other hand, the model also predicts an increase in antiproton flux. This increase has been compared with the \nr{sera antiproton, no ?positron} flux from the galactic center measured by the AMS-02 experiment\footnote{See Sect.~\ref{sec:charged} for a description of the experimental results and Sect.~\ref{sec:antiprot} for the details of the antiprotons propagation along the galaxy.}, seeing that there are areas in which the predictions of the model would not be compatible with what was observed experimentally (light yellow-shaded area in the Figure). \miguel{However, notice that the antiproton limits are less robust than the DSphs bounds, due to the large astrophysical uncertainties in the propagation models of charged particles\footnote{See Sect.~\ref{sec:antiprot} for a description of the antiproton propagation along the galaxy.}.}
Finally, an analysis of the possible impact of future Indirect Detection experiments on the model has also been carried out. In particular, it has been seen that the \nr{expected improvement in DSphs data  }by Fermi-LAT could put strong bounds on the studied model (blue-dashed line). As a final comment, we may say that the model in its present form would only marginally solve the GCE, but anyway it could be fully tested in the \nr{next} decade.

\section{Gravity-mediated Scalar Dark Matter in Warped Extra-Dimensions}
\label{sec:paper2ing}

All the evidence we have today about the existence of dark matter is related only to gravitational interaction. This leads us to think about the possibility that dark matter particles may only interact gravitationally. \nr{quitar, esto no es un problema, creo, porque podria no ser WIMP :(This idea has already been explored and presents a serious problem: the intensity of the gravitational interaction is very small and makes it impossible to obtain the amount of abundance of dark matter that is currently observed (at least in the WIMP scenario).)
In this case, DM would be undetectable by current and future particle physics experiments and it could not be a WIMP, since the  gravitational interaction is too weak to produce the observed dark matter abundance via de freeze-out mechanism.}
 However, what happens if we \nr {quitar(think) leave } in more than 4 dimensions? This is the idea that inspired Ref.~\cite{Folgado:2019sgz}.

In this work we explored whether it is possible to obtain the current DM abundance, under the assumption that is composed by WIMP scalar particles, only through gravitational interaction and assuming a 5-dimensional RS space-time. In the described scenario, Dark Matter and the Standard Model live confined in the TeV-brane. Both types of matter interact through gravity, which propagate along the brane in the form of 4-dimensional massive gravitons.

The model is described using four physical parameters: the scale of the interaction of 4-dimensional gravitons with matter, $\Lambda$; the mass of the first graviton of the 4-dimensional KK-tower, $ m_{1} $; the Dark Matter, $ m_{\text {DM}} $; and, the radion mass, $ m_r $. Our study of the model shows that the results obtained are practically independent of the value of $ m_r $: \miguel{the only dependence of the radion mass in the virtual radion-exchange annihilation cross-section is in the propagator. However, Since the radion decay width is rather small, for allowed values of $\Lambda$ and radion masses in the TeV range or below, a significant amount of fine-tuning is needed in order to get the resonant behaviour}. Therefore, for the study of the phenomenology, this parameter is irrelevant.
\nr { pero que sea fine-tuned no significa que sea irrelevante. ademas no lo entiendo, si fijamos $m_r$, solo hay resonancia cuando $m_{DM} = m_r/2$, que ni siquiera está en la fig. 7.2. Yo creo que es más bien:
 Our analysis shows that  when $m_r < m_{\text {DM}} $ and therefore the annihilation channel into radions is open, the results obtained are largely independent of the particular value of $ m_r $.  Regarding the virtual radion-exchange annihilation cross-section into SM particles, it becomes relevant only near the resonance, $m_{DM} \sim m_r/2$.
 Thus, for the study of the phenomenology we fix the radion mass and focus on the remaining parameters. }


\begin{figure}[t]
\centering
\includegraphics[width=150mm]{figures/resultados_paper_2.png}
\caption[Results from \textit{Gravity-mediated Scalar Dark Matter in Warped Extra-Dimensions}.]{\it Region of the $(m_{S}, m_{G_1})$ plane for which 
$\left\langle \sigma v \right\rangle = \left\langle \sigma_{\rm FO} v \right\rangle$. 
Left panel:  the radion and the extra-dimension stabilization mechanism play no role 
in DM phenomenology.
%length is stabilized without using the  mechanism. 
Right panel:  the extra-dimension length is stabilized with  the Goldberger-Wise mechanism, 
with radion mass $m_r = 100$ GeV.
In both panels, the grey area represents the part of the parameter
space where it is impossible to achieve the correct relic abundance; 
the red-meshed area is the region for 
which the low-energy RS effective theory is untrustable, as $\Lambda < m_{G_1}$; 
the wiggled red area in the lower left corner is the region excluded by DD experiments; 
the blue area is excluded by resonant KK-graviton searches at the LHC with 36 fb$^{-1}$ at $\sqrt{s} = 13$ TeV; 
the dotted blue lines represent the expected LHC exclusion bounds at the end of the Run III (with $\sim 300$ fb$^{-1}$)
and at  the HL-LHC (with $\sim 3000$ fb$^{-1}$); eventually, the green-meshed area on the right is
the region where the theoretical unitarity constraints are not fulfilled.
In the left panel, the allowed region is represented by the white area, for which $\left\langle \sigma_{\rm FO} v \right\rangle$
is obtained through on-shell KK-graviton production. In the right panel, in addition to the white area, 
within the tiny orange region  $\left\langle \sigma_{\rm FO} v \right\rangle$
is obtained through on-shell radion production and virtual radion exchange.
The dashed lines depicted in the white region represent the values of $\Lambda$ needed to obtain the correct relic abundance.
}
\label{fig:resultados_paper_2_ingles}
\end{figure}
The method followed for the analysis of the model has been the following: we have first computed the relevant annihilation cross-sections for DM into SM particles and KK-gravitons; then, we have studied a
two-dimensional grid with different values of the mass parameters $ (m_{1}, m_\text{DM}) $; for each of the points in this grid, we have searched if there is some value of $ \Lambda $ for which it is possible to obtain the current abundance of dark matter (for which $\langle \sigma \, v \rangle \backsimeq \langle \sigma \, v \rangle_\text{fo} = 2 \times 10^{-26} \text{cm}^3/\text{s}$). In this way, for each point of the grid the three free parameters ($m_{1}$, $m_\text{DM}$, $\Lambda$) are fully defined, which allows us to establish different theoretical and experimental limits on them. 

Fig.~\ref{fig:resultados_paper_2_ingles} shows the final results of the phenomenological analysis on the model. Following the above strategy, in the left panel the case without radion has been explored, assuming that some alternative method could be found to stabilize the radius of the fifth dimension. On the other hand, in the right panel it has been considered that the mass of the radion is $ m_r = 100 $ GeV (it is important to remember that the phenomenology is not affected by the value of this mass). The dark gray-shaded area is the region in which it is not possible to obtain the current abundance of dark matter for any value of $ \Lambda $, while the orange area represents the region of the parameter space in which the abundance is achieved thanks to the contributions of radionic interaction channels. The green-meshed area represents the region where we found unitarity problems\footnote {\miguel{Dark Matter particles have a small relative velocity and  to obtain the correct relic abundance $\sigma = \sigma_{\text{fo}}$. Then, this limit becomes a restriction directly on the DM mass, $m_{\text{DM}}^2 \lesssim 1/\sigma_{\text{fo}}$. Therefore, in the mass plane ($m_\text{DM}$, $m_1$) this bound appear as a vertical line.}}, $\sigma > 1/s$. In addition to this limit, there is another theoretical constraint: if $ \Lambda < m_{\text {DM}}, m_{1} $ the effective theory that describes the interaction of these quantum fields is not valid (as they should have been integrated out). This occurs in the red-meshed region.

So far we have talked about the different limits to the model for theoretical reasons, but these are not the only bounds that can be established. The current Direct Detection experiments and the resonance searches in the ATLAS and CMS experiments at the LHC can provide much information to our analysis. Thus, the red areas represent the points where a cross section of DM-nucleon interaction is already excluded by Xenon1T Direct Detection experiment. On the other hand, the blue area is the one excluded by the resonance searches (4-dimensional massive gravitons searches, in our case) at the LHC. More concretely, the strongest bound comes from searches at the LHC with 36 fb$^{-1}$ at $\sqrt{s} = 13$ TeV in the $\gamma \gamma$ channel. The two dotted lines show our prediction of the limits imposed by the LHC after the future Run III (with $\sim 300$ fb$^{-1}$) and at the HL-LHC (with $\sim 3000$ fb$^{-1}$).

The results of this work have been very rich: although similar analysis had already been carried out in the Randall-Sundrum scenario, this is the first paper that takes into account the dark matter annihilation channels directly into KK-gravitons in such high regions of mass space (various TeV). Likewise, a \nr{diagram (no channel)} totally forgotten in the literature has been studied so far: the annihilation into gravitons without a mediator, coming from the second order development of the interaction Lagrangian. On the other hand, it should be noted that this analysis has only been carried out for scalar Dark Matter. However, in Ref.~\cite{Folgado:2020vjb}, which is currently in the process of publication, the fermionic and vector Dark Matter cases are analysed.

\section{Gravity-mediated Dark Matter in CW/LD Extra-Dimensions}

Having analysed the implications of the existence of purely gravitational WIMP Dark Matter in Randall-Sundrum scenario, the question of what would occur in the recent CW/LD model almost naturally arises. This idea inspired Ref.~\cite{Folgado:2019gie}. CW/LD scenario presents more technical complications than RS: the KK-tower of massive gravitons in this case has a very small and \miguel{variable} separation that makes more complicated the numerical analysis of its phenomenology. A brief review about CW/LD extra-dimensions can be found in Sect.~\ref{sec:cw_ld}.

The strategy to analyse the model is the same that we used in RS case. The main difference with the previous model is the parameters chosen to study the phenomenology. In CW/LD the couplings of the massive 4-dimensional gravitons to the rest of the particles are not universal, as in RS. Therefore, it is more useful to characterize the model in terms of $ M_5 $ and not of the effective coupling $\Lambda_n$, that depends on the particular KK-mode considered. On the other hand, the mass of the first graviton coincides with the value of the curvature along the fifth dimension, $ m_{1} = k $.
Another important difference is the stabilization mechanism. In RS is necessary a new scalar field to stabilise the fifth dimension. In CW/LD the zero KK-mode of the 5-dimensional dilaton field takes this role. Unlike RS, where the radion mass is a new parameter, in this scenario the mass of the radion depends on the fundamental parameters of the model. However, there are several ways to stabilise the size of the extra-dimension with the dilaton fields. The minimal case assumes that the tension of the 4-dimensional branes is infinite. This framework receives the name of \textit{rigid limit} and it is the assumed case in this work. Currently, we are working in the study of the implications of the phenomenology out of the rigid limit. \miguel{There is other important difference between both frameworks relevant for the phenomenological study: In CW/LD the complete dilaton KK-tower is relevant. In RS the dilaton tower of the Goldberger-Wise scalar field was present, but heavy \cite{Goldberger:1999un}. As a consequence, the only light field present in the spectrum in that case was the radion.}

\begin{figure}[htbp]
\centering
\includegraphics[width=150mm]{figures/resultados_paper_3.png}
\caption[Results from \textit{Gravity-mediated Dark Matter in CW/LD Extra-Dimensions}.]{\it Region of the $(m_{\rm DM}, k)$ plane for which $\left\langle \sigma v \right\rangle = \left\langle \sigma_{\rm FO} v \right\rangle$. 
Upper left panel: scalar DM (unstabilized extra-dimension);
Upper right panel:  scalar DM (stabilized extra-dimension in the rigid limit); 
Lower left panel: fermion DM (stabilized extra-dimension in the rigid limit);
Lower right panel: vector DM (stabilized extra-dimension in the rigid limit).
In all panels, the grey-shaded area represents the part of the parameter space for which it is impossible to achieve the correct relic abundance; 
the red diagonally-meshed area is the region for which the low-energy CW/LD effective theory is untrustable, as $M_5 < k$; 
%the wiggled pink area in the lower left corner is the region excluded by Direct Dark Matter searches; 
the blue-shaded area is excluded by non-resonant searches at the LHC with 36 fb$^{-1}$ at $\sqrt{s} = 13$ TeV \cite{Giudice:2017fmj}; 
eventually, the green vertically-meshed area on the right is the region where the theoretical unitarity constraints are not fulfilled, 
$m_{\rm DM} \gtrsim 1/\sqrt{\sigma_{\rm FO}}$.
In all panels, the white area represents the region of the parameter space for which the correct relic abundance is achieved
(either through direct KK-graviton and/or radion/KK-dilaton production, as in the case of scalar DM, or through virtual KK-graviton exchange,
as for fermion and vector DM) and not excluded by experimental bounds and theoretical constraints.
The dashed lines depicted in the white region represent the values of $M_5$ needed to obtain the correct relic abundance.
}
 \label{fig:resultados_paper_3_ingles}
\end{figure}

Fig.~\ref{fig:resultados_paper_3_ingles} shows the results obtained for this scenario, following the same strategy outlined in Sect.~\ref{sec:paper2ing}. As in the RS case, $ M_5 $ has been used to set the current abundance of Dark Matter for each point in the parameter space ($ m_{\text{DM}}, k $). The different limits studied are the same as in the RS case: The red-meshed region shows the bounds of validity if the effective theory, $M_5 < m_{\text{DM}}, m_{G_1}$; the green-meshed region is where we have problems with the unitarity, $\sigma < 1/m_{\text{DM}}^2$; eventually, the blue-shaded area represent the limits imposed by the LHC Run II. As a consequence of the small separation between the KK-gravitons, the strongest bound imposed by the LHC comes from non-resonant searches in $\gamma \gamma$ channel. Finally, it should be noted that in the CW/LD case the limits imposed by the Direct Detection of Dark Matter are so small, that as a consequence, they do not appear in the Figure.

In this case, three possible Dark Matter particles spin have been analysed: scalar, fermion and vector. The two upper plots correspond to the scalar case without taking into account the radion and the dilaton-tower (left) and taking it into account (right). This is the only case in which dilatons play an important role in the phenomenology of the model and therefore it is worth showing what their impact is on the final results. The lower panels correspond to the fermionic case (left) and the vector case (right). In both cases the radion and the dilatons do not play any role. The Figure shows that the fermionic case is disfavoured with respect to the other two: the non-resonant searches at LHC impose strong limits in this case. This is due to the fact that in the fermionic case the dominant channel, the annihilation of Dark Matter directly into gravitons, is suppressed in velocity.

\miguel{As a final comment to gravitational-interacting DM in RS and/or CW/LD scenarios, we can say that in both cases a viable region of the parameter space exists, for the DM masses in the range $[1,10]$ TeV approximately and moderate values of the first KK-graviton mass. Most of the allowed region could be tested by the LHC Run II or its high luminosity upgrade. Notice that in the allowed region typically the scale of new physics (either $\Lambda$ or $M_5$) is a bit too large to solve the hierarchy problem.}

\section{Kaluza-Klein FIMP Dark Matter in Warped Extra-Dimensions}

In the three models analysed before it has been considered that the DM is composed by WIMP particles. However, FIMP Dark Matter\footnote{Described in Sect~\ref{sec:FIMP_intro}.} presents interesting properties for the purely gravitational case. In the last work included in this Thesis we explore if it is possible to obtain the DM abundance using gravitational interaction and FIMP particles in the RS scenario \cite{Bernal:2020fvw} (an extension to the CW/LD is under development). The FIMP case raises very different mathematical and numerical difficulties from the WIMP case: \miguel{due the small interaction that presents this kind of particles, the mechanism to obtain the DM abundance for FIMP particles is the freeze-in\footnote{For a complete description of the freeze-in mechanism see Sect.~\ref{Sec:freezein}.}, instead the freeze-out.} As it has been explained in Sect.~\ref{Sec:freezein}, in the WIMP DM case, the abundance is always obtained for $\left\langle \sigma v \right\rangle = \left\langle \sigma_{\rm FO} v \right\rangle$ for DM masses in the  GeV-TeV range. However, in the FIMP scenario the strong dependence of the evolution with the initial conditions makes necessary to solve the Boltzmann Equation, Eq.~\ref{BEFIMP}, for each point of the parameter space.

\begin{figure}[t]
\begin{center}
\includegraphics[height=0.5\textwidth]{figures/resultados_paper_4.pdf}
	\caption[Results from \textit{Kaluza-Klein FIMP Dark Matter in Warped Extra-Dimensions}.]{Parameter space required to reproduce the observed DM abundance for $m_\text{DM}=1$~MeV and $m_r=m_1/10^3$, for several values of the reheating temperature $T_\text{rh}$.
	The blue areas are excluded by resonant searches at LHC and represent the current bound and our prospects for the LHC Run-3 and the High-Luminosity LHC in the $\gamma \, \gamma$ channel~\cite{Aaboud:2017buh,Aaboud:2017yyg}.
	The upper left green corner corresponds to radion lifetimes longer than 1~s.
	In the lower right red area ($m_1>\Lambda$) the EFT approach breaks down.
}
	\label{fig:resultados_paper_4_ingles}
\end{center}
\end{figure}

In the FIMP case, the abundance also has a strong dependence on a new parameter: the highest temperature of the universe, the so-called \textit{reheating temperature} $T_{\text{rh}}$. Due to the complexity of the parameter space, the analysis in this scenario has been performed for a specific value of the Dark Matter mass: $ m_{\textit{DM}} = 1 $ MeV. The values of $T_\text{rh}$ needed to obtain the observed DM relic abundance are shown in Fig. \ref{fig:resultados_paper_4_ingles}. The blue-shaded region shows the experimental limits imposed by resonance searches in $pp \rightarrow G_1 \rightarrow \gamma \, \gamma$ channel at the LHC  (and the two predictions for the Run-3 and the HL-LHC). The red-shaded area represents the region where the EFT approach breaks down. On the other hand, the upper left green corner corresponds to radion lifetimes higher than $1$ s, potentially problematic for BBN (all the KK-graviton states are heavier than the radion and therefore will have naturally shorter lifetimes)

In contrast with the WIMP case, this work shows that, at an experimental level, the RS model with FIMP is much less constrained and opens up a whole range of possibilities to be explored by future experiments.

==> Chapters/Resumen_Tesis/Resumen_Tesis.tex <==
\inputencoding{latin1}
\include{Umlaute}       % ISO-8859-1 encoding
\inputencoding{utf8} % back to UTF-8


\chapter{Resumen de la Tesis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Motivaci\'on Hist\'orica}

Desde tiempos inmemoriales, uno de los más profundos deseos del ser humano ha sido descubrir la composición última de la materia que nos rodea. Ya los primeros escritos griegos hablan sobre la modelización de la naturaleza en base a cuatro elementos fundamentales; a saber, agua, tierra, fuego y viento. El paso de los siglos afinó mucho más esta prematura descripción. En el siglo XVII, se sintetizó por primera vez un elemento químico\footnote{En 1669 el alquimista Hennig Brand sintetizó por accidente fósforo, bautizándolo con este nombre por el brillo que desprendía.}, y tan solo dos siglos después (1869), ya existía una tabla periódica de los elementos, un claro reflejo de nuestro anhelo por encontrar orden en el caos.

El elevado número de elementos descubiertos en el siglo XX motivó la búsqueda de una estructura mucho más fundamental, aún totalmente desconocida. Fue Niels Bohr quien dió forma a esta idea, al sentar las bases de la teoría atómica actual \cite{Bohr:1913:CAMa,Bohr:1913:CAMb,Bohr:1913:CAMc}, apoyándose en los modelos atómicos propuestos previamente por Joseph John Thomson y Ernest Rutherford. Su elegante modelo explicaba toda forma de materia utilizando únicamente tres tipos de partículas: neutrones y protones, que componían el núcleo de los diferentes elementos atómicos, y electrones, los cuales orbitaban alrededor de dichos núcleos con energías cuantizadas. Los átomos quedaban descritos pues como pequeños sistemas planetarios, solo que las fuerzas implicadas en su estabilidad eran totalmente diferentes a la gravitatoria.

\begin{figure}[htbp]
\centering
\includegraphics[width=80mm]{figures/Standard_Model_of_Elementary_Particles.pdf}
\caption[Modelo Est\'andar de las interacciones fundamentales]{\it Modelo Estándar de las interacciones fundamentales: las partículas moradas, verdes y rojas representan, respectivamente, los quarks, leptones y bosones de gauge. Por otro lado, la amarilla representa el Bosón de Higgs. Imagen tomada de Ref.~\cite{citaSM}.}
 \label{fig:modelo_estandar}
\end{figure}

A lo largo del siglo XX el desarrollo de la mecánica cuántica cambió totalmente la forma de entender el mundo microscópico. A la fuerza gravitatoria y electromagnetica se le sumaron dos nuevas interacciones: débil y fuerte. Por otro lado, los protones y neutrones, que en el modelo de Bohr eran constituyentes fundamentales de la materia, pasaron a ser partículas compuestas por quarks, mientras una nueva plétora de partículas eran descubiertas gracias a los rayos cósmicos y a la construcción de nuevos experimentos y detectores. El resultado último de toda la revolución cuántica fue el Modelo Estándar de la física de partículas \cite{PhysRevLett.19.1264,GLASHOW1961579,Salam:1968rm,PhysRevLett.13.321,PhysRev.145.1156,PhysRevLett.13.508,PhysRevLett.13.585,PhysRev.155.1554,PhysRev.139.B1006,PhysRevD.2.1285,FRITZSCH1973365}, esquematizado en la Fig.~\ref{fig:modelo_estandar}. El modelo describe la naturaleza a nivel microscópico utilizando un total de doce partículas elementales, o campos, y cuatro tipos de interacción. Los éxitos del Modelo Estándar fueron totalmente rotundos, con él se han realizado las predicciones más precisas de la historia de la ciencia. No obstante, tiene ciertas limitaciones, como el hecho de que es incapaz de describir la gravedad cuántica. En el Capitulo \ref{sec:SM} se ha realizado una exposición detallada del modelo, profundizando en sus predicciones y fallos.

Hoy, casi medio siglo después de que fuese propuesto, sabemos que el Modelo Estandar únicamente es capaz de explicar el $5\%$ del contenido del Universo, el $95\%$ restante continua envuelto en un halo de misterio. Observaciones astrofísicas y cosmológicas indican que el $26\%$ del Universo está compuesto por un nuevo tipo de materia cosmológicamente estable que no emite luz, y que no puede identificarse con ninguna de las partículas del Modelo Estándar. Esta curiosa característica inspiró su nombre, \textit{Materia Oscura}. El resto del Universo es aún más enigmático si cabe. Actualmente se cree que está compuesto por algún tipo de energía que explicaría la expansión acelerada del Universo, pero esto es otra historia muy diferente a la de la Materia Oscura y queda lejos de los objetivos del trabajo aquí realizado.

La motivación de esta Tesis es intentar arrojar algo de luz sobre ese gran porcentaje de materia que nuestra ciencia actual no ha sido capaz de explicar, haciéndola un poco menos oscura de lo que su nombre indica.


\section{El Modelo Est\'andar de las Interacciones Fundamentales: La Piedra Angular de la F\'isica de Altas Energ\'ias} 
\label{sec:modelo_estandar}

En esta sección vamos a realizar un breve resumen de los conceptos más importantes del Modelo Estándar (en el Capitulo \ref{sec:SM} se han explicado todos los detalles técnicos del mismo). El Modelo Estándar de la física de partículas\footnote{Típicamente abreviado como SM, del inglés Standard Model.} es una teoría cuántica de campos con simetría gauge de los grupos unitarios $SU(3)_C \times SU(2)_L \times U(1)_Y$. El modelo describe con gran precisión tres de las cuatro interacciones fundamentales que existen en la naturaleza: débil, electromagnética y fuerte. La complejidad de la estructura de la interacción gravitatoria hace que sea muy complicado describirla como una teoría de campos gauge, actualmente se trabaja activamente en el tema\footnote{Algunos autores defienden que quizá el origen de la interacción gravitatoria sea totalmente diferente al resto de fuerzas fundamentales. La gravedad emergente (propuesta por Andrei Sakharov en 1967, el artículo original en inglés puede encontrarse en Ref.~\cite{Sakharov_1991}), por ejemplo, sugiere que dicha interacción no es más que el residuo de una serie de grados de libertad aún desconocidos, tal como la mecánica de fluidos, que deriva de la mecánica estadística.}. El resto de las interacciones fundamentales quedan descritas con gran precisión por el modelo mediante el intercambio de diferentes campos de spin 1, que constituyen el sector gauge de la teoría. Mientras que el grupo $SU(3)_C$  se asocia a la interacción fuerte, los grupos $SU(2)_L \times U(1)_Y$ describen la interacción electrodébil\footnote{Las interacciones electromagnéticas y débiles fueron unificadas en los años 70 por Sheldon Lee Glashow, Abdus Salam y Steven Weinberg.}


Las partículas de spin $1$, o bosones, describen las interacciones del modelo,  en tanto que  los constituyentes fundamentales de la materia son los fermiones, partículas de spin $1/2$: quarks y leptones. Curiosamente, la naturaleza replica los fermiones en 3 familias casi idénticas, únicamente diferenciadas por las masas de sus constituyentes: 
\bea
\label{familia_1_CS}
\nth{1} \, \text{Family}: L_{1} \equiv \left( \begin{array}{c}
\nu_e  \\
e^{-}  \end{array} \right)_{L} \, ; \, e_1 \equiv e^{-}_{_R} \, ; \, 
Q_1 \equiv \left( \begin{array}{c}
u  \\
d  \end{array} \right)_{L} \, ; \, U_1 \equiv u_R \, ; \, D_1 \equiv d_R \, , \nonumber \\
\label{familia_2_CS}
\nth{2} \, \text{Family}: L_{2}\equiv\left( \begin{array}{c}
\nu_{\mu}  \\
\mu^{-}  \end{array} \right)_{L} \, ; \, e_2 \equiv \mu^{-}_{_R} \, ; \,
Q_2 \equiv\left( \begin{array}{c}
c  \\
s  \end{array} \right)_{L} \, ; \, U_2 \equiv c_R \, ; \, D_2 \equiv s_R \, , \nonumber \\
\label{familia_3_CS}
\nth{3} \, \text{Family}: L_{3}\equiv\left( \begin{array}{c}
\nu_{\tau}  \\
\tau^{-}  \end{array} \right)_{L} \, ; \, e_3 \equiv \tau^{-}_{_R} \, ; \, 
Q_3 \equiv\left( \begin{array}{c}
t  \\
b  \end{array} \right)_{L} \, ; \, U_3 \equiv t_R \, ; \, D_3 \equiv b_R \, . \nonumber
\eea
Por otro lado, el modelo trata de forma diferente a partículas con quiralidad dextrógira y levógira, agrupando las primeras en singletes y las segundas en dobletes de $SU(2)_L$. De este modo, los quarks y leptones levógiros vienen representados por $Q_i$ (compuesto por los quarks tipo \textit{up} y tipo \textit{down}, con cargas eléctricas $+2/3$ y $-1/3$ de la carga fundamental del electrón, respectivamente) y $L_i$ (compuesto por los leptones cargados y los neutrinos, con cargas eléctricas $-1$ y $0$, respectivamente). Por otro lado, los quarks dextrógiros están representados por los singletes $U_i$ y $D_i$, mientras que los leptones cargados dextrógiros vienen dados por $e_i$.
Los neutrinos dextrógiros no están incluidos en el modelo original, aunque hay muchas líneas de investigación abiertas en la actualidad sobre la posibilidad de su existencia.

Aparte de todo lo comentado, el modelo incluye un campo de spin 0, el campo de Higgs. Los bosones gauge de la teoría débil, es decir $Z$ y $W^\pm$, tienen masa. Este hecho parecía incompatible con la construcción de un modelo basado en simetrías ya que la invariancia gauge prohíbe términos de masa para los bosones gauge. Por ello, fue necesario desarrollar un mecanismo que dotase de masa a estas partículas. La solución a este problema llegó de la mano de Robert Brout, Francois Englert, Gerald Guralnik, Carl Richard Hagen, Peter Higgs y Tom Kibble (en estricto orden alfabético), constituyendo lo que popularmente se conoce como \textit{mecanismo de Higgs} \cite{PhysRevLett.13.321,PhysRev.145.1156,PhysRevLett.13.585,PhysRev.155.1554}.

La idea del mecanismo de Higgs se basa en la \textit{ruptura espontánea de la simetría}\footnote{Del inglés \textit{Spontaneous Symmetry Breaking}.} (SSB) y consiste en agregar a la teoría un campo complejo escalar doblete de $SU(2)_L$:
\be
\Phi = \left( \begin{array}{c}
\Phi^+  \\
\Phi^0  \end{array} \right) = 
\left( \begin{array}{c}
\Phi^+  \\
\dfrac{1}{\sqrt{2}}(v + \phi_1 + i\phi_2)  \end{array} \right) \, .
\ee
Este peculiar campo presenta lo que se conoce como \textit{valor esperado de vacío}\footnote{Del inglés de \textit{Vacuum Expectation Value}.} (VEV) no nulo en su componente neutra, produciendo de este modo una ruptura de la simetría electrodébil (que no es una simetría exacta del vacío) y dando como resultado la simetría electromagnética\footnote{La abreviación QED viene de \textit{Quantum Electrodynamics} \cite{10.1143/PTP.1.27,10.1143/ptp/2.3.101,10.1143/ptp/3.2.101,PhysRev.74.224,PhysRev.74.1439,Feynman:1948ur,Feynman:1949zx}, nombre que recibe la teoría gauge que describe la interacción electromagnética.},
\be
SU(2)_L\times U(1)_Y \longrightarrow U(1)_{QED}.
\ee

Durante la SSB, tanto la parte cargada del doblete como la parte imaginaria de la componente neutra son absorbidos como grados de libertad longitudinales por los bosones gauge de la teoría, los cuales pasan a comportarse como bosones masivos. Por otro lado, la parte real del campo cargado, $\phi_1$, se queda presente en el espectro de partículas del Modelo Estándar como una partícula de spin 0, el popular \textit{bosón de Higgs}, que fue detectado en 2012 por los experimentos ATLAS \cite{Aad_2012} y CMS del LHC \cite{Chatrchyan_2012}, confirmando el modelo.

Las representaciones de los fermiones del Modelo Estándar bajo el grupo $SU(2)_L\times U(1)_Y$ no presentan simetría quiral, necesaria para que los correspondientes términos de masa puedan aparecer en el lagrangiano del modelo. No obstante, el mecanismo de Higgs soluciona este problema ya que bajo el grupo $U(1)_{\text{QED}}$ si que presentan dicha simetría. En consecuencia, después de la SSB, el VEV del campo de Higgs permite la formación de los términos de masa para estas partículas.

Para una exposición detallada y completa del Modelo Estándar en español ver Ref.~\cite{gelmini2014el}.

\section{La Necesidad de la Materia Oscura}

Como ya hemos comentado, el Modelo Estandar de partículas solo puede explicar un porcentaje pequeño de la materia que nos rodea, conocida como \textit{bariónica}\footnote{Nombre que recibe la materia descrita por el Modelo Estándar.}. El resto de materia que puebla el Universo recibe el nombre de Materia Oscura. A pesar de que este exótico tipo de materia es un activo campo de estudio en la actualidad, los primeros indicadores de su existencia son ya casi centenarios \cite{Zwicky:1933gu}. No obstante, las primeras pruebas sólidas se las debemos a los trabajos de Vera Cooper Rubin, Kent Ford y Ken Freeman, llevados a cabo allá por los años 60 \cite{1970ApJ...159..379R,1970ApJ...160..811F}.

\subsection{Evidencias de la Existencia de Materia Oscura}
\label{sec:res:evidencias}

La evidencia más clara que tenemos a día de hoy de la existencia de la Materia Oscura son las curvas de rotación de las galaxias. El contenido en masa de una galaxia puede medirse en base a su luminosidad, mediante técnicas astrofísicas. De este modo, tenemos una clara idea de cuanta materia bariónica hay en una determinada galaxia y como está distribuida dentro de ella. Conocida la masa de la galaxia, la velocidad de rotación de un objeto situado a una distancia $R$ del centro de la misma puede determinarse a partir de las leyes de Kepler\footnote{$v = \sqrt{MG/R}$, donde $M$ es la masa contenida en la esfera de radio $R$ y $G$ la constante de gravitación universal.}. De acuerdo con esto, la distribución de materia bariónica observada nos indica que la velocidad de rotación debería disminuir conforme nos acercamos al borde galáctico. Sin embargo, medidas directas sobre la velocidad de rotación indican lo contrario: en la mayoría de los casos esta velocidad de rotación permanece constante.

Las curvas de rotación de las galaxias son la evidencia más famosa de la existencia de este exótico tipo de materia, pero no la única. La teoría de la Relatividad General predice que el campo gravitatorio producido por un gran cúmulo de materia es capaz de desviar los rayos de luz, el conocido como efecto \textit{lente gravitatoria}. De este modo, puede utilizarse la luz procedente de galaxias lejanas para, mediante ciertos estudios sobre la trayectoria de los haces de luz, determinar la cantidad de materia que hay en los cúmulos de galaxias situados en su trayectoria. Este análisis confirma la presencia de Materia Oscura en la mayoría de cúmulos de galaxias estudiados.

Aparte de las evidencias astrofísicas, hay tambi\'en  evidencias cosmológicas que confirman la existencia de la Materia Oscura. En la Sec.~\ref{sec:evidences} se ha realizado una breve descripción de todas ellas.

\subsection{Caracter\'isticas Fundamentales}

A pesar de las evidencias de su existencia, a día de hoy aún no se ha realizado ninguna observación directa de la Materia Oscura. No obstante, podemos inferir mucho acerca de su naturaleza:
\begin{itemize}
\item La Materia Oscura debe ser no bariónica: algunos candidatos bariónicos han sido propuestos a lo largo de los años, como es el caso de los MACHOs\footnote{Del inglés \textit{Massive Compact Halo Objects}.} \cite{1986ApJ...304....1P}. No obstante, los límites sobre esta clase de modelos son tan fuertes en la actualidad que están prácticamente descartados en su totalidad.
\item Debe ser \textit{fría} o \textit{cálida}: según la distancia recorrida, como consecuencia de movimientos aleatorios, por las partículas de Materia Oscura en el Universo primigenio, podemos catalogarla en tres grandes grupos: \textit{calinte}, \textit{cálida} y \textit{fría}. Si la distancia recorrida es mayor, igual o menor que el tamaño de una protogalaxia (unos 100 años luz), la Materia Oscura será caliente, cálida o fría, respectivamente. En la actualidad se han realizado numerosas simulaciones numéricas de la evolución del Universo con diferentes tipos de materia. Si la Materia Oscura fuese caliente, de acuerdo con estas simulaciones, el Universo tendría un aspecto muy diferente al que conocemos hoy en día \cite{primack2001happened}.
\item Debe colisionar muy débilmente consigo misma: el motivo de esto es que recientes observaciones astrofísicas, tales como las realizadas sobre el conocido como \textit{cúmulo bala}\footnote{Este curioso cúmulo es el resultado de dos cúmulos actualmente en colisión. En él se observa un efecto muy exótico, el centro de masas del cúmulo resultante se encuentra desplazado. Esta característica solo puede ser explicada mediante la existencia de grandes cantidades de Materia Oscura en su composición. La alternativa requeriría una modificación de las leyes más fundamentales de la dinámica relativista.}, imponen restricciones a la autointeracción de la Materia Oscura \cite{Dave_2001,Feng_2009,Agrawal_2017,Randall_2008,Kahlhoefer_2013}:
\be
\sigma/m \lesssim 10^{-24} \, \text{cm}^2/\text{GeV} .
\ee
\item Débilmente interactiva con la materia bariónica: aparte de la interacción gravitatoria, la única interacción posible que podría llegar a tener la Materia Oscura es la débil. Respecto a lo que al electromagnetismo se refiere, las diversas implicaciones que supone la existencia de Materia Oscura cargada han sido profundamente estudiadas en la literatura \cite{DERUJULA1990173}, descartando prácticamente esta opción por motivos experimentales\footnote{En la actualidad las técnicas de detección de partículas cargadas son tan avanzadas que de existir la Materia Oscura eléctricamente cargada, esta ya debería haber sido observada.} \cite{Taoso:2007qk}.
Por otro lado, de existir la Materia Oscura fuertemente interactiva\footnote{Fuertemente en el sentido de interacción a través de la interacción fuerte.}, ésta dejaría huella incluso en el flujo de calor terrestre \cite{Mack:2007xj}. Las fuertes implicaciones de este tipo de candidatos hacen que esten excluidos casi en su totalidad.
\item Debe ser estable: la Materia Oscura que observamos hoy en día en el Universo es prácticamente un fósil térmico: es el remanente de la que la que componía el Universo primigenio. La única forma de que ese remanente haya sobrevivido hasta nuestros días es que la Materia Oscura sea estable o, en su defecto, que su vida media sea mayor que la edad del Universo.
\end{itemize}

En la Sec.~\ref{sec:Properties} se ha realizado un estudio mucho más profundo de todas estas propiedades.

\subsection{Candidatos Estudiados}

Hasta el momento hemos hablado de las diferentes evidencias y características de la Materia Oscura. Pero ¿cuál es su naturaleza? En el escenario científico actual se han propuesto muchos candidatos a Materia Oscura, desde todo tipo de partículas con interacciones parecidas a las que ya conocemos, hasta candidatos altamente exóticos como agujeros negros primigenios \cite{10.1093/mnras/168.2.399,1975ApJ...201....1C,10.1093/mnras/152.1.75}. Todo esto ha sido detallado en la Sec.~\ref{sec:candidates}. En este resumen únicamente hablaremos sobre los dos candidatos estudiados en esta Tesis: las partículas WIMP \cite{PhysRevLett.39.165} y las FIMP \cite{Hall:2009bx}.

\subsubsection{Materia Oscura tipo WIMP}

Las partículas WIMP\footnote{Su nombre deriva del inglés \textit{Weakly Interactive Massive Particles}, es decir, partículas masivas débilmente interactivas.} son partículas con masas típicamente desde el GeV hasta varios TeV. Este candidato se basa en la suposición de que las partículas de Materia Oscura se encontraban en equilibrio térmico con el resto de partículas del Modelo Estándar en el Universo primigenio. La abundancia que observamos en la actualidad sería pues el resultado de un proceso denominado \textit{freeze-out}.

Para entender bien el concepto de \textit{freeze-out}, debemos remontarnos a los primeros instantes del Universo, justo después del Big Bang. En aquella época, los átomos no existían, las diferentes partículas que poblaban el Universo se encontraban en un equilibrio continuo de aniquilación/producción, formando un plasma de altísima temperatura. Poco a poco, el Universo fue expandiéndose, enfriando dicho plasma. El enfriamiento del Universo provocó que algunos de los procesos que mantenían este equilibrio dejasen de tener lugar, desacoplando de este modo las diferentes especies de partículas de este \textit{caldo} primigenio.

Cuando la temperatura del Universo fue demasiado baja como para que la creación de partículas de Materia Oscura fuese posible, está se desacopló del \textit{caldo} primigenio. Como consecuencia, la abundancia de estas partículas comenzó a disminuir, hasta que fue tan pequeña que la probabilidad de que dos partículas de Materia Oscura se encontrasen y se aniquilasen se volvió prácticamente nula. A dicha temperatura, conocida como temperatura de \textit{freeze-out}, la abundancia de Materia Oscura superviviente se convirtió en un leve remanente, un mero fósil térmico, que ha llegado hasta nuestros días.

Este candidato a Materia Oscura ha gozado de gran acogida por los físicos teóricos desde que fuese propuesto alla por los años 70. El motivo de tal popularidad es que en el rango de masas mencionado, curiosamente, para reproducir la abundancia de Materia Oscura actual, se necesita que la interacción entre ésta y las partículas del Modelo Estándar sea justo del orden de la interacción electrodébil. Hecho, cuanto menos sorprendente, que se conoce como \textit{Milagro WIMP}. En este rango de masas la sección eficaz necesaria para conseguir dicha abundancia es prácticamente independiente del valor de la masa de la partícula WIMP,
\be
\langle \sigma v \rangle \backsimeq 2 \times 10^{-26}\, \text{cm}^3/\text{s} \backsim 1 \, \text{pb} \, .
\ee
Los detalles matemáticos y técnicos de este candidato a Materia Oscura se encuentran explicados en la Sec.~\ref{Sec:freezeout}.

\subsubsection{Materia Oscura tipo FIMP}

Complementariamente al caso WIMP, existe la Materia Oscura tipo FIMP\footnote{Nombre que deriva del ingles \textit{Feebly Interactive Massive Particle}.} la cual jamás llegó al equilibrio térmico con el resto de partículas del Modelo Estándar. En este escenario la Materia Oscura fue producida por diversos procesos durante la época de enfriamiento del Universo, después del Big Bang, siendo nula en el origen de los tiempos. Cuando la temperatura del Universo fue suficientemente baja, esta producción se congeló, dejando un remanente que ha llegado hasta nuestros días. Este mecanismo de producción recibe el nombre de \textit{freeze-in}\footnote{El mecanismo de producción fue propuesto en Ref.~\cite{Chung:1998rq}. Aunque en aquella época ni el mecanismo se conocía por dicho nombre, ni el candidato como FIMP.} y está detallado en la Sec.~\ref{Sec:freezein}.

La Materia Oscura FIMP no ha llegado a alcanzar la popularidad de la Materia Oscura tipo WIMP. Hay varios motivos para ello pero el principal es que debido a su baja intensidad de interacción es muy dificil buscar pruebas experimentales de su existencia.

\section{Detecci\'on de Materia Oscura}

Como hemos comentado en la Sec.~\ref{sec:evidences}, y resumido en Sec.~\ref{sec:res:evidencias}, tenemos muchas evidencias de la existencia de a Materia Oscura. No obstante, no se ha conseguido realizar ninguna observación directa de estas elusivas partículas\footnote{Existe una llamativa excepción: el experimento DAMA/Libra ha medido variaciones en la modulación solar que pueden ser interpretadas como Materia Oscura \cite{Bernabei:2008yi,Bernabei:2010mq}. No obstante, esta señal no está libre de controversia entre la comunidad científica ya que ningún otro experimento ha reportado absolutamente nada en el rango de masas en el que DAMA/Libra mide dicha señal.}. A pesar de esto, las técnicas de detección de Materia Oscura han avanzado mucho en los últimos años, poniendo cotas cada vez más restrictivas a la existencia de estas partículas aparentemente invisibles.
Dentro del gran abanico de experimentos de detección, estos pueden clasificarse en dos grandes grupos: la \textit{Detección Directa}\footnote{Del ingles \textit{Direct Detection.}} DD y la \textit{Deteccion Indirecta}\footnote{Del ingles \textit{Indirect Detection.}} ID.

\subsection{Detecci\'on Directa}

La idea de la Detección Directa (cuyos detalles técnicos se discuten en profundidad en la Sec.~\ref{Sec:DD}) fue propuesta por primera vez por Mark Goodman y Edward Witten \cite{Goodman:1984dc}. Como la Materia Oscura no presenta cargas eléctricas, es imposible detectarla mediante técnicas electromagnéticas. No obstante, la existencia de colisiones entre la DM y los núcleos atómicos abre una puerta para su observación directa. 

En general, esta clase de detecciones se realizan en experimentos ubicados bajo tierra. Ejemplos notables son Xenon1T \cite{PhysRevLett.121.111302} o LUX \cite{Akerib:2016vxi}, los cuales están compuestos por grandes cantidades de Xenón. La colisión de la Materia Oscura con los átomos de Xenón produciría una excitación de estos últimos, que finalmente se traduciría en la emisión de un fotón. Hasta el momento, no se ha realizado ninguna detección en dichos experimentos, lo cual pone fuertes límites sobre los modelos de Materia Oscura, haciendo que los escenarios más simples y \textit{naturales} estén prácticamente descartados.

\begin{figure}[htbp]
\centering
\includegraphics[width=130mm]{figures/direct_detection_bounds.pdf}
\caption[Estatus actual de los experimentos de detecci\'on directa.]{\it Límites actuales a la sección eficaz de interacción de Materia Oscura con nucleones. La región verde está excluida por los experimentos de Detección Directa con un 90\% de intervalo de confianza. Las dos zonas rojas muestran las regiones en las que DAMA/LIBRA afirma haber observado Materia Oscura. La zona amarilla representa el \textit{suelo  de neutrinos} \cite{Billard:2013qya}.}
 \label{fig:direct_detection_bounds_resumen}
\end{figure}

Uno puede hacerse una idea del panorama actual de estos experimentos mirando la Fig.~\ref{fig:direct_detection_bounds_resumen}. En ella, la zona verde muestra los valores de la sección eficaz de Detección Directa, como función de la masa de la Materia Oscura, que ya han sido descartados por los experimentos. Por otro lado, para hacernos una idea de magnitud de la zona ya eliminada, podemos mirar lo cerca que se encuentra de ella la región amarilla. Esta región muestra lo que se conoce como \textit{suelo de neutrinos}\footnote{En ingles conocido como \textit{neutrino floor}.} \cite{Billard:2013qya} y representa la sección eficaz para la que los experimentos de detección comenzarán a observar colisiones producidas por los neutrinos. Realizar exclusiones mediante experimentos de Detección Directa en esta región es complicado, puesto que la señal de ambos tipos de colisión es indistinta. Las dos regiones rojas muestran las observaciones de DAMA/LIBRA en zonas totalmente excluidas por el resto de experimentos.

\subsection{Detecci\'on Indirecta}

La observación directa de las colisiones de las partículas de Materia Oscura con los núcleos atómicos no es la única técnica para detectarla. Diferentes experimentos astronómicos llevan años intentando observar los posibles productos de las aniquilaciones de las partículas de Materia Oscura en los rayos cósmicos que nos llegan a la Tierra. Es posible distinguir entre tres tipos de flujos de partículas: fotones, neutrinos y partículas cargadas (como electrones, positrones, etc).

En general, de los diferentes flujos de partículas que llegan a la Tierra, los resultados más prometedores (en lo que a Materia Oscura se refiere) vienen de los fotones. Desde 2008 la colaboración Fermi-LAT analiza el flujo de fotones procedente de diferentes \textit{galaxias enanas} \cite{Fermi-LAT:2016uux,Ackermann:2015zua}. Hasta el momento el estudio se restringe a 15 ejemplares y por el momento los resultados no muestran ningún exceso en el flujo analizado que no pueda ser explicado por el Modelo Estándar de partículas. Esto pone cotas a modelos de nueva física en los cuales la Materia Oscura pueda aniquilarse a partículas que finalmente se desintegren en fotones, generalmente en el rango de masas $m_{\text{DM}} \in (0.5,500) $ GeV. No obstante, desde 2009 el mismo experimento ha estado reportando un exceso inexplicable de fotones procedente del centro galáctico\footnote{Popularmente conocido como \textit{Galactic Center $\gamma$-ray excess} (GCE) \cite{Goodenough:2009gk, Vitale:2009hr, Hooper:2010mq, Gordon:2013vta, Hooper:2011ti, Daylan:2014rsa, 2011PhLB..705..165B, Calore:2014xka, Abazajian:2014fta,Zhou:2014lva}.}. Aunque su origen aún es desconocido, este exceso, que se observa a una energía $\sim 3$ GeV, puede ser explicado por diferentes modelos de Materia Oscura.

Por otro lado, las señales procedentes de flujos de antipartículas cargadas acotan de una forma mucho menos restrictiva los modelos de Materia Oscura. El problema con esta clase de flujos es su propagación desde el punto en el que son generados hasta la Tierra (donde finalmente los detectamos). Hoy en día existen diversos modelos para ello, pero su precisión aún tiene que ser perfeccionada para que los límites impuestos por esta clase de flujos sean realmente restrictivos.

En la Sec.~\ref{Sec:ID} se ha realizado un análisis exhaustivo de la Detección Indirecta de Materia Oscura.

\section{Dimensiones Extra}

De entre las cuatro fuerzas fundamentales de la naturaleza, no cabe ninguna duda de que la gravedad es la más complicada de entender a nivel cuántico. A pesar de los muchos esfuerzos por parte de la comunidad científica, aún no tenemos una teoría cuántica para describirla.
Por otro lado, la gravedad es la más débil de las interacciones fundamentales. Tal es el caso, que de existir nueva física a la escala gravitatoria, el Modelo Estándar se enfrentaría a un serio problema: las correcciones a la masa del bosón de Higgs son muy sensibles a la escala de la nueva física. Teniendo en cuenta la diferencia entre la escala de Planck\footnote{La escala de la interacción gravitatoria.} y la escala electrodébil, de aparecer nueva física a la escala gravitatoria las correcciones a la masa del Higgs serían enormes, requiriendo cancelaciones ajustadas entre distintos órdenes de teoría de perturbaciones para explicar el valor medido. A este fenómeno se le conoce como \textit{problema de la jerarquía} (para un analisis más detallado del problema mirar la Sec.~\ref{sec:hierarchyproblem}). Entre las diversas propuestas que se han realizado para intentar resolver este problema se encuentran las dimensiones extra.

\subsection{Dimensiones Extra \textit{Grandes} (LED)}

El primer modelo de dimensiones extra que se propuso para dar solución al problema de la jerarquía fue \textit{Large Extra-Dimensions} (LED) \cite{ArkaniHamed:1998rs}. En este escenario se asume que las nuevas dimensiones tienen una forma similar a las tres espaciales ya conocidas, es decir, presentarían un aspecto plano. De acuerdo con el modelo LED, el tamaño de estas nuevas dimensiones sería finito o, en otras palabras, estarían compactificadas. Por otro lado, mientras que la gravedad se propaga libremente por el espacio 5-dimensional, el resto de campos del Modelo Estándar se encuentran confinados en unas hipersuperficies 4-dimensionales denominadas \textit{branas}. Este hecho hace que la gravedad se diluya a través de las dimensiones extra, haciendo que en la brana (donde nosotros vivimos confinados) su intensidad parezca anómalamente débil. De este modo, la escala de la gravitación, que para nosotros es $M_\text{P} = 1.22 \times 10^{19}$ GeV, en el espacio extra-dimensional completo sería $M_D$. Ambas escalas están relacionadas a través del radio de compactificación de las dimensiones extra ($r_c$):
\be
M_\text{P}^2 = M_{D}^{D-2} (2\pi r_c)^D.
\ee 

Para el caso particular de 5 dimensiones, el espacio-tiempo queda definido en este modelo por la métrica:
\be
ds^2 = \eta_{\mu \nu}dx^\mu dx^\nu + r_c^2dy^2,
\ee
Donde la dimensión extra está representada por $y$. Este parámetro puede escogerse de manera que $M_5 \backsim \text{TeV}$, resolviendo así el problema de la jerarquía.
No obstante, si imponemos esta condición, el modelo LED 5-dimensional está excluido totalmente a día de hoy: agregar una única dimensión extra en LED predice correcciones de la ley de la gravitación universal que podrían observarse en distancias parecidas al tamaño del Sistema Solar. No obstante, aunque el modelo esté excluido para una única dimensión extra, con dos o más dimensiones es posible resolver el problema de la jerarquía sin entrar en contradicciones con la ley de la gravitación universal.

\subsection{Dimensiones Extra Deformadas: Modelo de Randall-Sundrum}

A pesar de que los modelos LED presentan diversos problemas, pusieron la semilla para modelos futuros muy interesantes. El caso más popular es el modelo propuesto por Lisa Randall y Raman Sundrum a finales de los años 90, conocido como \textit{dimensiones extra deformadas} o \textit{modelo de Randall-Sundrum} (RS) \cite{Randall:1999ee}. En dicho modelo, las nuevas dimensiones presentan curvatura, a diferencia de LED, donde eran planas. En el modelo original de RS el espacio extra-dimensional está delimitado por dos branas. Todos los campos de materia viven atrapados en una de ellas (brana \textit{infrarroja} (IR), también llamada brana del TeV), mientras que la otra brana se encuentra vacía (brana \textit{ultravioleta} (UV) o de Planck). Por otro lado, la gravedad se propaga libremente por el espacio extra-dimensional (comúnmente conocido como \textit{bulk}). La geometría del modelo hace que los diferentes parámetros fundamentales con dimensión de masa sufran un proceso de deformación exponencial a lo largo del bulk, resolviendo así el problema de la jerarquía.

Concretamente, para el caso 5-dimensional (una única dimensión extra), la métrica que definiría este espacio tiempo vendría dada por
\be
ds^2 = e^{-2  kR|y|}\eta_{\mu \nu} dx^\mu dx^\nu - r_c^2 dy \, ,
\label{RS_metric_resumen}
\ee
Donde $k$ es la curvatura a lo largo de la dimensión extra y $r_c$ su radio de compactificación. El factor exponencial que multiplica la parte 4-dimensional de la métrica recibe el nombre de factor de deformación.
$M_5$ y $M_\text{P}$ quedarían entonces relacionados mediante los dos parámetros libres de la teoría:
\be
\bar{M_\text{P}}^2 = \frac{M_5}{k} \left( 1 - e^{-2 k \pi r_c} \right) \, .
\ee
Vemos que hay una clara diferencia con el modelo LED: en RS $M_5\backsimeq M_\text{P}$. Sin embargo, la modificación que sufren los parámetros medidos en la brana IR, debido a la presencia del factor de deformación, resuelve el problema de la jerarquía para $k\,r_c \backsim 10 $.

En RS la gravedad puede describirse a través del intercambio de gravitones no masivos 5-dimensionales, los cuales surgen de perturbaciones sobre la componente 4-dimensional de la métrica
\be
G^{(4)}_{\mu \nu} = e^{-2kr_c|y|} (\eta_{\mu \nu} + 2M_5^{-2/3} h_{\mu \nu}) \, .
\label{perturbacion_4dim}
\ee
La proyección de este campo 5-dimensional sobre las branas es equivalente a una torre de gravitones 4-dimensionales masivos, comúnmente conocidos como modos de Kaluza-Klein (KK). La escala efectiva de la interacción de estos gravitones 4-dimensionales con los campos confinados en la brana IR viene dada por
\be
\Lambda \equiv \bar{M_\text{P}} e^{-k \pi r_c} \, .
\ee
Por otro lado, cada gravitón de esta torre de partículas tiene una masa diferente que dependerá de los parámetros libres ($k,r_c$) del modelo y de su respectivo orden dentro de la torre. No obstante, establecida la masa del primer gravitón $m_1$, la masa del resto de gravitones queda totalmente fijada. La fenomenología de los modelos de RS puede ser descrita mediante los parámetros ($\Lambda,m_1$), en lugar de ($k,r_c$). Este hecho puede ser muy útil debido a su relación con observables fenomenológicos.

El modelo asume que la distancia entre las branas está fijada, pero no aporta ningún mecanismo para estabilizar este parámetro dinámicamente. La solución a este problema fue propuesta por Walter D. Goldberger y Mark B. Wise \cite{Goldberger:1999wh,Goldberger:1999uk}. Este mecanismo utiliza un nuevo campo escalar que se propaga libremente por el \textit{bulk}, sometido a unos potenciales localizados en las branas. 
Por otro lado, el nuevo campo escalar se mezcla con el ya presente en el \textit{bulk}, el graviescalar $G_{55}^{(5)}$ (el cual emerge de las perturbaciones sobre la parte 5-dimensional de la métrica). Al campo resultante de esta mezcla se le conoce como radión. Los mínimos de los potenciales en la brana IR y UV son diferentes, lo que genera un valor esperado de vacío para el radión. El tamaño de la quinta dimensión ($r_c$) está entonces relacionado con este valor esperado de vacio. La masa del radión no está determianda por los parámetros del modelo original, y representa un nuevo grado de libertad.

El modelo de RS ha gozado de gran popularidad desde que fue propuesto a finales de los 90's. La literatura sobre modelos de física más allá del Modelo Estándar desarrollados en este escenario es inmensa. En la Sec.~\ref{sc:warped} se ha realizado un análisis de los detalles técnicos del modelo.  

\subsection{Dimensiones extra tipo \textit{Clockwork/Linear Dilaton}}

Durante casi dos décadas lo modelos de RS fueron los únicos que resolvían el problema de la jerarquía mediante la introducción de dimensiones con curvatura. No obstante, en 2016 Gian Giudice y Matthew McCullough propusieron un nuevo modelo de dimensiones extra curvadas. Este nuevo modelo, propuesto en Ref.~\cite{Giudice:2016yja} y cuya fenomenología fue estudiada en Ref.~\cite{Giudice:2017fmj}, se conoce con el nombre de \textit{Clockwork/Linear Dilaton} (CW/LD).

Dicho modelo, que fue encontrado como límite continuo de los modelos \textit{Clockwork} discretos, puede caracterizarse a traves de la métrica:
\be
\label{eq:5dmetric_resumen}
ds^2 = e^{4/3 k r_c |y|} \left ( \eta_{\mu \nu} dx^{\mu}dx^{\nu} - r_c^2 \, dy^2 \right ) \, ,
\ee
donde $k$ y $r_c$ representan la curvatura y el radio de compactificación de la quinta dimensión, respectivamente. Para determinados valores de los parámetros libres, el modelo es capaz de resolver el problema de la jerarquía.

El modelo CW/LD guarda ciertas similitudes con RS. En ambos casos el espacio 5-dimensional está delimitado por las branas IR y UV. El caso mínimo implica tener todo el Modelos Estándar confinado en la brana IR, mientras que la gravedad se propaga libremente por el bulk 5-dimensional. Sin embargo, hay diferencias notables con RS. En primer lugar, la relación entre $M_5$ y $M_\text{P}$ en CW/LD viene dada por
\be
M_{\text{P}}^2 = \frac{M_5^3}{k} \left ( e^{2 \pi r_c}  - 1 \right ) \, ,
\ee 
pudiendo ser esta del orden del TeV (al igual que en el caso LED). Por otro lado, el acoplamiento de los modos de Kaluza-Klein de los gravitones a las partículas localizadas en la brana es diferente para cada gravitón:
\be
\dfrac{1}{\Lambda_{n}} =  \dfrac{1}{\sqrt{M_5^3 \pi r_c}}  \left ( 1 + \dfrac{k^2 r_c^2}{n^2} \right )^{-1/2} 
=  \dfrac{1}{\sqrt{M_5^3 \pi r_c}} \left ( 1 - \dfrac{k^2}{m_n^2} \right )^{1/2}  \,  .
\ee
Este hecho hace que describir la fenomenología en base a $\Lambda_n$ no sea tan útil como en RS. Otra diferencia notable es que hay una relación muy interesante entre el valor de la curvatura $k$ y la masa del primer gravitón $m_1$, haciendo que ambos parámetros sean prácticamente idénticos.

En el caso CW/LD, el modelo original ya incluye un campo escalar que estabiliza el tamaño de la quinta dimension, el campo de dilatación (\textit{dilaton}), $S = 2 k r_c |y|$, de la métrica. La existencia de unos potenciales en las branas IR y UV permite fijar la posición de las branas de un modo similar a como se hacía en RS.

\section{Metodolog\'ia Utilizada}

Antes de ponernos a hablar sobre los cuatro proyectos que conforman la presente Tesis, es necesario comentar las diferentes técnicas (tanto a nivel analítico como numérico) utilizadas en el desarrollo de los mismos. 

A nivel analítico, la complejidad de los problemas estudiados ha requerido un profundo conocimiento de la teoría cuántica de campos. Se han utilizado los desarrollos perturbativos de dicha teoría para obtener las diferentes probabilidades de interacción utilizadas posteriormente en los estudios fenomenológicos. Los modelos aquí estudiados asumen Materia Oscura tipo WIMP y FIMP. En ambos casos, la evolución de la abundancia de Materia Oscura a lo largo de la historia térmica del Universo requiere resolver la Ecuación de Boltzman, que determina la evolución de sistemas fuera del equilibrio térmico. Por otro lado, se ha trabajado con dos modelos de dimensiones extra:  Randall-Sundrum y Clockwork/Linear Dilatón. La fenomenología estudiada sobre estos modelos ha requerido un análisis exhaustivo de ambos escenarios.

Desde un punto de vista numérico, toda la fenomenología ha sido estudiada mediante lenguaje \textit{C++}, mientras que su representación a nivel gráfico ha sido obtenida utilizando \textit{python}. El análisis de la Detección Indirecta de Materia Oscura realizado en uno de los modelos estudiados ha requerido el uso de software más específico: \textit{micrOMEGAs}, \textit{SARAH}, \textit{gamlike}, \textit{pythia} y \textit{MadGraph}. Por otro lado, todo el estudio de la Ecuación de Boltzman en los cuatro modelos se ha realizado mediante métodos numéricos implementados en lenguaje \textit{C++}.

Finalmente, el enfoque fenomenológico que presenta esta Tesis ha implicado un contacto continuo con datos experimentales. El tratamiento de estos datos, así como las diferentes cotas de exclusión que han puesto sobre los diferentes modelos estudiados, ha requerido un uso de diversas técnicas estadísticas. Se han utilizado diferentes distribuciones de probabilidad (tales como la conocida $\chi^2$), técnicas de Monte Carlo, etc.

\section{Resultados y conclusiones de la Tesis}

En está sección, vamos a realizar un breve resumen de los proyectos que conforman esta Tesis. Todos ellos pueden encontrarse completos en la Parte \ref{sec:papers}.

\subsection{Estudio de la Detecci\'on Indirecta del Modelo de \textit{Portal de Neutrinos Est\'eriles}}

Uno de los grandes problemas abiertos en física de altas energías es la Materia Oscura, pero desde luego no es el único. Entre los diversos problemas que existen actualmente en el Modelo Estándar de partículas, uno de los más importantes es la masa de los neutrinos. El modelo predice una masa nula para ellos, no obstante, hace ya más de medio siglo se predijo un efecto denominado \textit{oscilaciones de neutrinos} \cite{Pontecorvo:1957cp}. Este curioso fenómeno, que fue confirmado experimentalmente en 1999 \cite{Fukuda:1998mi}, consiste en una oscilación en el sabor leptónico de los neutrinos. Las implicaciones de este hecho son muy profundas ya que únicamente puede suceder si al menos uno de los tres sabores de neutrinos es masivo\footnote{A pesar de que el fenómeno podría explicarse con un solo neutrino masivo, la observación del fenomeno tanto en neutrinos atmosfericos como solares requiere que al menos dos de los tres sabores de neutrinos sean masivos.}. No obstante, las cotas experimentales impuestas a la masa de estas partículas prácticamente invisibles son tan fuertes que su masa debe ser muy pequeña\footnote{El límite actual más fuerte viene dado por el experimento \textit{Karlsruhe Tritio Neutrino} (KATRIN) \cite{Aker:2019uuj}.}.
Este hecho potenció el desarrollo de modelos en los que la masa de los neutrinos era generada por mecanismos de tipo \textit{balancín}\footnote{Modelo \textit{seesaw} en inglés.} \cite{GellMann:1980vs,PhysRevLett.44.912,Yanagida:1979as,Glashow1111,MINKOWSKI1977421}. Hay diferentes versiones de estos modelos, en el \textit{tipo I}, por ejemplo, se asume la existencia de neutrinos dextrógiros muy masivos que justifican la pequeña masa de los neutrinos del Modelo Estándar. La mezcla de los neutrinos levógiros con los dextrogiros da como resultado los autoestados de masa, prediciendo neutrinos con masas muy grandes y muy pequeñas.

La posibilidad de que el problema de la Materia Oscura y de la masa de los neutrinos estén relacionados motivó el desarrollo del conocido como\footnote{El escenario más económico, la posibilidad de que los neutrinos estériles sean la Materia Oscura, fue propuesto en Ref.~\cite{Dodelson:1993je}. A día de hoy, esta posibilidad ha sido fuertemente estudiada y prácticamente descartada \cite{Adhikari:2016bei}.} \textit{portal de neutrinos estériles a Materia Oscura} \cite{Escudero:2016tzx,Macias:2015cna,Escudero:2016ksa}. Este modelo se ha estudiado por diversos autores, acotándolo utilizando la Detección Directa de Materia Oscura. No obstante, es un modelo muy interesante desde el punto de vista de la Detección Indirecta por varios motivos. Por un lado, la Detección Directa en este escenario no sucede al orden más bajo en teoría de perturbaciones de la teoría cuántica de campos. Este hecho hace que sus señales de Detección Directa sean bajas que en otros modelos, empeorando así los límites impuestos. Por otro lado, la conexión de los neutrinos estériles con los neutrinos activos hace que las aniquilaciones de Materia Oscura produzcan, como resultado de diversas desintegraciones, excesos de fotones y partículas cargadas. Todo esto lo convierte en el candidato perfecto para ser estudiado desde el punto de vista de la Detección Indirecta, tal como se ha llevado a cabo en la Ref.~\cite{Folgado:2018qlv}.

En este trabajo hemos analizado un modelo particular en el que, además de los neutrinos estériles, se asume la existencia de dos nuevos campos: uno escalar $\phi$ y otro fermionico $\Psi$. Estos campos son ambos singletes del Modelo Estándar, no obstante, están cargados respecto a un nuevo grupo de simetría, $G_{\text{dark}}$, de tal forma que la combinación $ \overline{\Psi} \phi$ es singlete de este nuevo grupo de simetría.

\begin{figure}[htbp]
\centering
\includegraphics[width=120mm]{figures/resultados_paper_1.pdf}
\caption[Resultados del primer art\'iculo.]{\it Límites sobre el \textit{portal de neutrinos estériles} en el espacio de masas. La región amarilla muestra los límites impuestos por los antiprotones mientras que la región azul son los límites impuestos por los fotones procedentes de las galaxias enanas. Los diferentes contornos muestran la zona en la que el modelo es capaz de reproducir el GCE. La línea discontinua azul muestra nuestra predicción sobre el límite de las galaxias enanas para los próximos 15 años.}
 \label{fig:resultados_paper_1}
\end{figure}

La más ligera de estas nuevas partículas \textit{oscuras} ($\phi$ y $\Psi$) es estable si todas las particulas del Modelo Estándar, así como los neutrinos esteriles, son singletes de $G_{\text{dark}}$, independientemente de la naturaleza de este grupo de simetría. Como consecuencia, debido a su estabilidad esta partícula es un buen candidato a Materia Oscura. Por simplicidad, asumimos que $G_{\text{dark}}$ es una simetría global a baja enería, en cualquier caso no esperamos cambios significantes en nuestro analisis fenomenológico si esta fuese local.

Los terminos más relevantes en el lagrangiano vienen dados por:
\bea
\mathcal{L} &=& \mu_H^2 H^\dagger H - \lambda_H (H^\dagger H)^2  -
\mu_\phi^2 \phi^\dagger \phi - \lambda_\phi (\phi^\dagger \phi)^2 - 
\lambda_{H\phi} (H^\dagger H) \, (\phi^\dagger \phi)   
\nonumber \\
&-&\left( \phi \overline{\Psi}(  \lambda_a +  \lambda_p \gamma_5) N 
 + Y \overline {L}_L H N_{R}  + {\rm h.c.}  \right)  \, . \nonumber \\
 \,
\eea

Los acoplamientos de Yukawa $Y$ entre los neutrinos dextrógiros $N_R$ y el doblete leptónico del Modelo Estándar genera las masas para los neutrinos activos después de la ruptura espontanea de la simetría, a traves del mecanismo \textit{balancín} de tipo I. Si bien se requieren al menos dos neutrinos estériles para generar las masas de neutrinos observadas en las oscilaciones, en nuestro análisis consideramos que solo una especie es más ligera que la Materia Oscura y, por lo tanto, relevante para la determinación de su abundancia y búsquedas indirectas. No obstante, los resultados son fáclmtente extendibles al caso en el que tenemos dos o más neutrinos estériles más ligeros que la Materia Oscura. Bajo el supuesto de que la Materia Oscura es descrita por $\Psi$ (el análisis es igualmente valido en el caso de que la Materia Oscura sea $\phi$) las masas del modelo cumplen la relación $m_N < m_\Psi < m_\phi$.

La Fig.~\ref{fig:resultados_paper_1} muestra los resultados finales de nuestro análisis. Fijando la masa del mediador escalar para obtener la abundancia de Materia Oscura mediante el mecanismo \textit{freeze-out} (es decir $\langle \sigma \, v \rangle \sim 2 \times 10^{-26} cm^3/s$), la figura muestra los diferentes limites impuestos por las búsquedas de fotones y antiprotones en el espacio de masas $(M_N,M_\Psi)$. Como ya hemos comentado, el experimento Fermi-LAT ha reportado un exceso de fotones inexplicable procedente del centro galáctico (GCE). El modelo estudiado predice un pequeño exceso de fotones que podría ser compatible con el GCE en ciertas zonas del espacio de parámetros. En nuestro analisis hemos asumidoque existen dos fuentes diferentes para el GCE: una astrofísica, responsable de la zona de alta energía del espectro de fotones, y otra procedente de las aniquilaciones de Materia Oscura, la cual explicaría la zona de baja energía del exceso,  
\be
\Phi = \Phi_{\text{astro}} + \Phi_{\text{DM}} \, .
\ee
Esta contribución astrofísica al flujo de fotones es siempre necesaria para reproducir el GCE, independientemente del modelo de Materia Oscura considerado.
La zona en la que puede realizarse el ajuste del exceso de fotones del centro galactico está delimitada por los diferentes contornos que se observan en la figura (en la leyenda está indicado el p-valor asociado a cada contorno). No obstante, este aumento de fotones predicho por el modelo tiene que ser compatible también con el resto de medidas realizadas sobre los diferentes flujos de fotones. En concreto, el mismo experimento realiza medidas sobre los fotones procedentes de 15 galaxias enanas\footnote{Galaxias compuesta por varios millones de estrellas. En contraposición tenemos las galaxias normales, compuestas por varios miles de millones.}, la región sombreada en azul muestra la zona del espacio de parámetros de la teoría en la cual los resultados obtenidos no son compatibles con dichas mediciones al 90 \% de intervalo de confianza.

Por otro lado, el modelo también predice un aumento del flujo de antiprotones. Este aumento se ha comparado con el flujo de antiprotones procedente del centro galáctico, el cual es medido en la actualidad por el experimento AMS-02.Los resultados obtenidos muestran que existen zonas en las cuales las predicciones del modelo no serían compatibles al 95 \% de intervalo de confianza con lo observado experimentalmente (zona sombreada en amarillo en la figura).
Por último, también se ha realizado un análisis del posible impacto de los resultados futuros el experimento Fermi-LAT. Basandonos en la mejora experimentada por la colaboración, hemos estimado que en 15 años se habrán detectado 45 galaxias enanas nuevas. Este hecho podría poner fuertes cotas al modelo estudiado (línea azul discontinua). Como comentario final, podemos decir que algunos modelos de Materia Oscura son capaces de explicar el exceso de fotones del centro galactico parcialmente\footnote{Hasta el momento todos los modelos necesitan asumir que parte del exceso es consecuencia a fenomenos astrofísicos.}. En concreto, el modelo aquí estudiado consigue reproducirlo con una precisión muy alta. No obstante, los resultados futuros del experimento Fermi-LAT podrían excluir casi por completo la región del espacio de parámetros en la cual el GCE puede ser explicado por el modelo.

\subsection{Materia Oscura Escalar Mediada por Gravedad en Dimensiones Extra Deformadas}

Todas las evidencias que tenemos hoy en día acerca de la existencia de la Materia Oscura están relacionadas con la interacción gravitatoria. Este hecho induce a pensar en la posibilidad de que las partículas de Materia Oscura únicamente interactúen gravitatoriamente. Esta idea tan natural ha sido explorada ya para los candidatos de tipo WIMP sin demasiado exito: la intensidad de la interacción gravitatoria es muy débil y hace imposible obtener la cantidad de abundancia de Materia Oscura que se observa en la actualidad (al menos en el escenario WIMP). No obstante, ¿que ocurre si pensamos en más de 4 dimensiones? Esta es la idea que inspiró la Ref.~\cite{Folgado:2019sgz}.

En dicho artículo tratamos de explorar si es posible obtener la abundancia de Materia Oscura actual, asumiendo que es de tipo WIMP escalar, únicamente mediante interacción gravitatoria y bajo el supuesto de un Universo 5-dimensional de tipo Randall-Sundrum. En el escenario descrito, la Materia Oscura y el Modelo Estándar viven confinados en la brana infrarroja. Ambos tipos de materia interactúan únicamente a través de la gravedad, cuya proyección sobre la brana IR es equivalente a una torre de gravitones 4-dimensionales masivos (torre de Kaluza-Klein).

El modelo queda descrito en base a cuatro parámetros físicos: la escala de la interacción de los gravitones 4-dimensionales con la materia, $\Lambda$; la masa del primer gravitón de la torre de KK, $m_{1}$; la masa del candidato a Materia Oscura, $m_{\text{DM}}$ y la masa del radión, $m_r$. Nuestro estudio muestra que cuando $m_r < m_\text{DM}$ y, en consecuencia, el canal de aniquilación a radiones esta abierto, el valor de $m_r$ es prácticamente irrelevante para la fenomenología. 
Respecto a la aniquilación de la Materia Oscura a partículas del Modelo Estandar a traves del intercambio de radiones virtuales, esta sección eficaz únicamente es relevante cerca de la resonancia $m_\text{DM} \backsim m_r/2$. Por lo tanto, en el estudio fenomenológico realizado hemos fijado la masa del radion y nos hemos centrado en el resto de parámetros libres del modelo.

El método seguido para el análisis del modelo ha sido la construcción de una malla bidimensional con diferentes valores de los parámetros $(m_{G_1},m_\text{DM})$. Para cada uno de los puntos de este mallado hemos buscado si existe algún valor de $\Lambda$ para el cual se obtiene la abundancia de Materia Oscura actual (es decir, para $\langle \sigma v \rangle \backsimeq \langle \sigma v \rangle_\text{fo} = 2 \times 10^{-26} \, \text{cm}^3/\text{s}$). De este modo, para cada punto del mallado los tres parámetros libres ($m_{1}$, $m_\text{DM}$, $\Lambda$) quedan totalmente definidos. Este análisis nos permite establecer diferentes límites teóricos y experimentales en el espacio de masas del modelo. 

\begin{figure}[t]
\centering
\includegraphics[width=150mm]{figures/resultados_paper_2.png}
\caption[Resultados del segundo art\'iculo.]{\it Región en el plano $(m_{\text{DM}}, m_{1})$ para la cual 
$\left\langle \sigma v \right\rangle = \left\langle \sigma_{\rm fo} v \right\rangle$. La gráfica de la izquierda muestra el caso sin radión, mientras que en la de la derecha se ha considerado $m_r = 100$ GeV. Las líneas discontinuas muestran los diferentes valores de $\Lambda$ en el plano ($m_\text{DM},m_{1}$) para los cuales se consigue la abundancia actual de Materia Oscura. La zona gris muestra la región en la cual es imposible conseguir la abundancia de Materia Oscura, independientemente del valor de $\Lambda$. Por otro lado, la región naranja nos indica los puntos en los que la abundancia se consigue gracias a los canales de interacción en los que interviene el radión. Respecto a los límites sobre el modelo: la zona de cuadraditos verde representa el límite de unitariedad; la zona de cuadraditos rosa representa la zona en la que la teoría efectiva deja de tener validez, es decir $\Lambda < m_{1}$; la zona roja representa los límites impuestos por el experimento Xenon1T sobre la sección eficaz de Detección Directa; la región azul es la zona eliminada por las búsquedas de resonancias en el LHC usando los datos de 36 fb$^{-1}$ at $\sqrt{s} = 13$ TeV. Finalmente, las líneas punteadas son las predicciones de exclusión para las fases \textit{Run-III} (con $\sim 300$ fb$^{-1}$) y \textit{High Luminosity} (con $\sim 3000$ fb$^{-1}$) del LHC.}
 \label{fig:resultados_paper_2}
\end{figure}

En la Fig.~\ref{fig:resultados_paper_2} pueden verse los resultados finales del análisis fenomenológico sobre el modelo. En la parte izquierda se ha explorado el caso sin radión, asumiendo que podría encontrarse algún método alternativo para estabilizar el radio de la quinta dimensión. Por otro lado, en la parte derecha se ha considerado que la masa del radión es $m_r = 100$ GeV (es importante recordar que la fenomenología no se ve afectada por el valor de esta masa). La zona sombreada en gris es la región en la que no es posible obtener la abundancia actual de Materia Oscura para ningún valor de $\Lambda$, mientras que la zona naranja representa la región del espacio de parámetros en la que la abundancia se consigue gracias a las contribuciones de los canales de interacción radiónicos. La zona sombreada con cuadraditos verdes se conoce como límite de unitariedad y representa el punto a partir del cual la sección eficaz de interacción es tan alta que la teoría de campos deja de tener sentido, esto sucede para\footnote{En el escenario WIMP las partículas de Materia Oscura tienen una velocidad relativa muy pequeña. Este hecho implica que $s \backsimeq m_{\text{DM}}^2 (4 + v^2_{\text{rel}}) $, donde $v_{\text{rel}} \ll 1 $ es la velocidad relativa de las partículas de Materia Oscura. Además, para conseguir la abundancia de Materia Oscura observada en la actualidad debe cumplirse $\sigma = \sigma_{\text{fo}}$. Como consecuencia, este límite se convierte en un límite sobre la masa de la Materia Oscura $m_{\text{DM}}^2 \lesssim 1/\sigma_{\text{fo}}$. Por lo tanto, enel plano de masas ($m_\text{DM}$, $m_1$) la zona excluida por unitariedad aparece como una linea vertical.} $\sigma > 1/s$. Además de este límite, existe otra restriccion teórica: si $\Lambda < m_{\text{DM}}, m_{1}$ la teoría efectiva que describe la interacción de estos campos cuánticos deja de tener sentido (ya que deberían estar integrados). Esto ocurre en la región de cuadraditos rosa.

Hasta el momento, hemos hablado de las diferentes restricciones al modelo por motivos teóricos, pero estos no son los únicos límites que pueden establecerse: los actuales experimentos de Detección Directa y las búsquedas de resonancias en los experimentos ATLAS y CMS del LHC pueden aportar mucha información a nuestro análisis. De este modo, las zonas sombreadas en rojo representan los puntos en los que la sección eficaz de Detección Directa está ya excluida por los actuales experimentos. Por otro lado, la zona azul es la excluida por las búsquedas de resonancias (gravitones 4-dimensionales en nuestro caso) en el LHC, se han utilizado los datos tomados a $\sqrt{s} = 13$ TeV con 36 fb$^{-1}$ en el canal $\gamma \gamma$. Las dos líneas punteadas muestran nuestra predicción sobre los límites futuros que serán impuestos por el LHC después de las futuras fases \textit{Run-3} (con $\sim 300$ fb$^{-1}$) y \textit{High Luminosity} (con $\sim 3000$ fb$^{-1}$), en el caso de que no se detecte ninguna resonancia.

El estudio realizado muestra que, en las regiones no excluidas del espacio de parámetros, la fenomenología está dominada por los canales de interacción relacionados con los gravitones. En dichas regiones, de acuerdo con nuestro análisis, los canales de interacción radiónicos siempre son subdominantes. Para ser más exactos, la abundancia se consigue gracias a la aniquilación de Materia Oscura directamente en gravitones.

Aunque ya se habían realizado análisis similares en Randall-Sundrum, este trabajo es el primero que tiene en cuenta los canales de aniquilación de Materia Oscura directamente a gravitones en regiones tan altas del espacio de masas (varios TeV). Así mismo, se ha estudiado un diagrama totalmente olvidado en la literatura hasta el momento: la aniquilación a gravitones sin mediador, procedente del desarrollo a segundo orden del lagrangiano de interacción. Aunque el impacto de este diagrama sobre la fenomenología no cambia drásticamente los resultados, debe ser añadido por consistencia ya que es del mismo orden que el resto de diagramas estudiados. Por otro lado, cabe destacar que este análisis únicamente se ha realizado para Materia Oscura escalar. No obstante, en la Ref.~\cite{Folgado:2020vjb} que está actualmente en trámites de publicación, se analizan los casos de Materia Oscura fermiónica y vectorial. En este estudio se ve que la Materia Oscura de tipo fermionico está claramente desfavorecida respecto a la escalar y vectorial ya que el canal dominante (la aniquilación directamente a gravitones) está más suprimido que en el resto de casos.

\subsection{Materia Oscura Mediada por Gravedad en Dimensiones Extra Tipo \textit{Clockwork/Linear Dilaton}}

Analizadas las implicaciones de la existencia de Materia Oscura tipo WIMP con interacciones puramente gravitatoria en el escenario de Randall-Sundrum, la pregunta de que ocurriría en el novedoso Clockwork/Linear Dilatón casi surge de forma natural. Esta idea inspiró la Ref.~\cite{Folgado:2019gie}. La estructura de este escenario es diferente a la que teníamos en RS: la torre de KK de gravitones masivos en este caso tiene una separación muy pequeña y variable. Este hecho dificulta en gran medida el análisis numérico de su fenomenología.

A nivel conceptual, la estrategia para abordar el modelo es idéntica a la empleada en el caso RS. La gran diferencia con el modelo anterior son los parámetros elegidos para estudiar la fenomenología. En CW/LD los acoplamientos de los gravitones 4-dimensionales masivos al resto de partículas dependen del orden del gravitón dentro de la torre. Por ello, es más útil caracterizar el modelo en función de $M_5$ directamente, en lugar de usar los acoplamientos efectivos $\Lambda_n$ de los gravitones 4-dimensionales. Por otro lado, la masa del primer gravitón coincide prácticamente con el valor de la curvatura a lo largo de la quinta dimensión $m_{1} = k$. Otra diferencia notable entre ambos escenarios es la estabilización del tamaño de la dimensión extra. En RS es necesario introducir un nuevo campos escalar en el \textit{bulk} con el fin de estabilizar dinamicamente $r_c$. En cambio, en CW/LD el dilatón presente en la métrica puede utilizarse para escribir los potenciales en la brana y estabilizar así el tamaño de la quinta dimensión. En este caso, la masa del radión (modo cero de la torre de dilatones 4-dimensionales) está fijada por los parámetros fundamentales del modelo (ya que deriva directamente de la métrica). No obstante, hay diferentes formas de realizar la estabilización usando el dilatón, el caso más simple es asumir que la tensión de las branas es infinita. Este escenario, recibe el nombre de límite rigido.

\begin{figure}[htbp]
\centering
\includegraphics[width=150mm]{figures/resultados_paper_3.png}
\caption[Resultados del tercer art\'iculo.]{\it Región en el plano $(m_{\rm DM}, k)$ para la cual $\left\langle \sigma v \right\rangle = \left\langle \sigma_{\rm fo} v \right\rangle$. Las gráficas superiores muestran los resultados para el caso de Materia Oscura escalar, la inferior izquierda el caso fermiónico y la inferior derecha el vectorial. La gráfica superior izquierda muestra las diferentes zonas de exclusión teniendo en cuenta únicamente la interacción con gravitones. Por otro lado, en la gráfica superior derecha se han considerado ambas, la interacción mediante gravitones y mediante dilatones, para el caso de Materia Oscura escalar. En los casos fermiónico y vectorial no se muestra el caso sin dilatones ya que la contribución de los mismos es despreciable y no varía los resultados. Las líneas discontínuas muestran los diferentes valores de $M_5$ en el plano ($m_\text{DM},k$) para los cuales se consigue la abundancia actual de Materia Oscura, mientras que la zona gris muestra la región en la cual es imposible conseguir dicha abundancia, independientemente del valor de $M_5$.
Respecto a los límites sobre el modelo: la zona de cuadraditos verde representa el límite de unitariedad ($m_{\rm DM} \gtrsim 1/\sqrt{\sigma_{\rm fo}}$); la región de cuadraditos rosa representa el área en la que la teoría efectiva deja de tener validez ($M_5 < k, m_\text{DM}$) y, finalmente, la región azul representa los límites impuestos por las búsquedas no-resonantes en el LHC usando los datos de 36 fb$^{-1}$ a $\sqrt{s} = 13$ TeV para el canal $\gamma \gamma$ \cite{Giudice:2017fmj}.}
 \label{fig:resultados_paper_3}
\end{figure}

La Fig.~\ref{fig:resultados_paper_3} muestra los diferentes límites obtenidos para este escenario. Análogamente al caso RS, $M_5$ se ha utilizado para fijar la abundancia actual de Materia Oscura para cada punto del espacio ($m_{\text{DM}},k$). Los diferentes límites estudiados son los mismos que en el caso anterior: la región de cuadraditos rosa muestra los límites de la teoría efectiva ($M_5 < k, m_\text{DM}$), la región de cuadraditos verdes el límite de unitariedad ($m_{\rm DM} \gtrsim 1/\sqrt{\sigma_{\rm fo}}$) y, finalmente, la zona sombreada en azul los límites impuestos por el LHC. En el caso de los límites experimentales, debido a la proximidad de las resonancias en la torre de gravitones, el límite más estricto impuesto por el LHC viene de las búsquedas en el espectro continuo de energías, en lugar de las búsquedas de resonancias. Estos límites han sido calculados usando los datos de 36 fb$^{-1}$ a $\sqrt{s} = 13$ TeV para el canal $\gamma \gamma$ \cite{Giudice:2017fmj}. Finalmente, cabe destacar que, en este caso, los límites impuestos por las búsquedas de Detección Directa de Materia Oscura corresponden a valores de ($m_\text{DM},k$) menores que los mostrados en la Figura. 

Otra diferencia notable con el caso RS es que aquí no solo hay que considerar el radión en la fenomenología, si no también toda la torre de KK de los dilatones. No obstante, en CW/LD el radión y los dilatones derivan directamente de la métrica del modelo, no es necesario un mecanismo externo para estabilizar el tamaño de la quinta dimensión. Este hecho hace que la masa de los mismos este intrínsecamente ligada a los parámetros fundamentales del modelo, sin agregar de este modo ningún grado nuevo de libertad al espacio de parámetros de la teoría.

En este trabajo se han analizado los tres posibles tipos de Materia Oscura: escalar, fermiónica y vectorial. Las dos figuras superiores corresponden al caso escalar sin tener en cuenta la torre de radión y dilatones (izquierda) y teniéndola en cuenta (derecha), respectivamente. Este es el único caso en el que los dilatones juegan un papel importante en la fenomenología del modelo y por ello merece la pena mostrar cuál es su impacto sobre los resultados finales. Las gráficas inferiores corresponden al caso fermiónico (izquierda) y al caso vectorial (derecha). Se puede ver claramente que el caso fermiónico está desfavorecido respecto a los otros dos. Este hecho se debe a que en el caso fermiónico el canal dominante, la aniquilación de Materia Oscura directamente a gravitones, sufre una supresión debido al momento angular total.

El análisis llevado a cabo en este trabajo representa el primer estudio fenomenológico del modelo CW/LD con presencia de Materia Oscura. Los resultados anteriores, al igual que en RS, son prometedores en el sentido de que toda la región no excluida podrá ser analizada en los próximos años por el LHC. Como comentario final sobre la Materia Oscura tipo WIMP púramente gravitatoria, podemos decir que en ambos escenarios es posible reproducir la abundancia actual en el rango $m_\text{DM} \in [1,10] \, \text{TeV}$. No obstante, los valores necesarios, tanto de $\Lambda$ en RS como de $M_5$ en CW/LD, para ello son excesivamente grandes como para resolver el problema de la jerarquía.

\subsection{Materia Oscura FIMP en Dimensiones Extra Deformadas}

Hasta el momento, todos los modelos analizados consideran partículas tipo WIMP. No obstante, la Materia Oscura tipo FIMP es muy interesante para el caso en el que la interacción es puramente gravitatoria. En el último proyecto incluido en esta Tesis hemos explorado la posibilidad de reproducir la abundancia de Materia Oscura actual utilizando partículas FIMP en un escenario tipo RS \cite{Bernal:2020fvw}. Este caso plantea complicaciones matemáticas y numéricas muy diferentes al caso WIMP. Entre estos problemas, el más importante es que la abundancia final predicha por el modelo depende en gran medida de las condiciones iniciales. Este hecho hace que, mientras que en el caso WIMP\footnote{Como consecuencia del \textit{milagro WIMP}.} la abundancia actual se reproduce para un valor constante de la sección eficaz de interacción ($\left\langle \sigma v \right\rangle = \left\langle \sigma_{\rm fo} v \right\rangle$), en el caso FIMP es necesario resolver siempre la ecuación diferencial que determina su evolución, la conocida como ecuación de Boltzmann.

\begin{figure}[htbp]
\centering
\includegraphics[width=115mm]{figures/resultados_paper_4.pdf}
\caption[Resultados del cuarto art\'iculo.]{\it Valores de la temperatura de reheating (lineas negras) para los cuales un determinado valor de la escala de interacción en la brana y la masa del primer graviton reproducen la abundancia de Materia Oscura actual para $m_\text{DM} = 1$ MeV y $m_r = m_1/10^3$. La zona azul representa la región excluida por las búsquedas de resonancias del LHC. La región roja muestra el límite de la teoría efectiva $m_1>\Lambda$. Finalmente, la región verde muestra la zona en la que el valor de la vida media del radión entra en conflicto con las observaciones de la Nucleosíntesis del Big Bang.}
 \label{fig:resultados_paper_4}
\end{figure}

Por otro lado, aquí la abundancia también tiene una fuerte dependencia con un nuevo parámetro: la temperatura máxima del Universo, conocida como temperatura de \textit{reheating} ($T_{\text{rh}}$). Debido a la complejidad del espacio de parámetros, el analisis en este escenario se ha llevado a cabo para un valor determinado de la masa de la Materia Oscura: $m_{\textit{DM}} = 1$ MeV, no obstante, los resultados son similares para otros valores $m_{\textit{DM}} $. En la Fig.~\ref{fig:resultados_paper_4} se muestran los valores necesarios de la temperatura de reheating para obtener la abundancia observada. La región azul sombreada muestra los límites experimentales impuestos por las búsquedas de resonancias en el canal $pp \rightarrow G_1 \rightarrow \gamma \, \gamma$ en el LHC (y las dos predicciones para las futuras etapas del experimento). Por otro lado, los límites teóricos en este escenario vienen determinados por la validez de la teoría efectiva (región roja) y la \textit{Nucleosíntesis del Big Bang}. Este último límite se traduce en una restricción sobre la vida media de los gravitones y del radión: si la $\tau>1$ s se podrían producir modificaciones en las observaciones sobre la Nucleosíntesis del Big Bang que deberían estar reflejadas en los datos experimentales actuales. En los modelos analizados anteriormente, este límte no aparecia ya que la vida media de los gravitones y radion/dilatones siempre era mayor que 1 segundo. 

A la vista de los resultados obtenidos, vemos que el caso FIMP está mucho menos excluido que el caso WIMP en el escenarios de RS y que la abundancia de Materia Oscura actual se consigue en una gran región muy amplia del espacio de parámetros. A pesar de ello, los valores obtenidos para los parámetros libres de la teoría están lejos de resolver el problema de la jerarquía. Por otro lado, los experimentos actuales aún no son capaces de explorar los parámetros típicos de los modelos FIMP. No obstante, el hecho de que los modelos de Materia Oscura tipo FIMP sean capaces de explicar la abundancia actual en un rango del espacio de parámetros tan amplio es una gran motivación para el futuro desarrollo de experimentos. Actualmente estamos trabajando en el estudio análogo para el caso CW/LD.

\subsection{Conclusi\'on}

%En esta Tesis hemos estudiado la fenomenología de diferentes modelos de Materia Oscura, centrándonos principalmente en los candidatos de tipo WIMP. En este escenario las partículas de Materia Oscura se encontraban en equilibrio termodinámico con el resto de partículas que componen el Modelo Estándar en el Universo primigenio. A causa de su expansión, el Universo sufrió un proceso de enfriamiento y las partículas de Materia Oscura terminaron por desacoplarse del plasma primigenio, dejando un remanente que ha llegado hasta nuestros días. Este proceso es denominado como \textit{freeze-out}.


%Entre los modelos estudiados en esta Tesis, se ha explorado la posibilidad de que el problema de la Materia Oscura pueda resolverse al mismo tiempo que el de la masa de los neutrinos mediante el Portal de Neutrinos Estériles. Por la estructura del modelo, este es un candidato perfecto para ser acotado usando la Detección Indirecta. Para ello, primero se ha estudiado la posibilidad de que el exceso de fotones del centro galáctico sea consecuencia de las aniquilaciones de Materia Oscura gracias a los neutrinos Estériles. Se ha visto que, efectivamente, el exceso puede ser reproducido para un pequeño rango de masas, el cual se encuentra actualmente en tensión con otras medidas experimentales: la detección de fotones procedentes de las galaxias enanas y de antiprotones procedentes del centro galáctico. Así mismo, se ha visto que a lo largo de los próximos años la mejora de las prestaciones del experimento Fermi-LAT hará, previsiblemente, que los datos recolectados acerca de las galaxias enanas sean incompatibles con la región del espacio de parámetros en la que es posible reproducir el exceso de fotones del centro galáctico.

%Por otro lado, se ha estudiado la posibilidad de que la Materia Oscura únicamente presente interacción gravitatoria. Esta idea se sustenta en el hecho de que todas las pruebas que tenemos de la existencia de la Materia Oscura están relacionadas únicamente con la interacción gravitatoria. En 4 dimensiones, como consecuencia de la debilidad de la interacción, es imposible obtener la cantidad exacta de Materia Oscura que existe actualmente en nuestro Universo. Por este motivo hemos estudiado la viabilidad de esta idea en 5 dimensiones. Efectivamente, se ha comprobado que en espacios 5-dimensionales se puede obtener la abundancia actual de Materia Oscura utilizando únicamente interacción gravitatoria. En este contexto se han analizado dos posibles modelos de dimensiones extra: el conocido modelo Randall-Sundrum y el novedoso \textit{Clockwork/Linear Dilatón}. Los resultados obtenidos en ambos casos son muy prometedores, la abundancia de Materia Oscura se obtiene en una amplia región del espacio de parámetros que puede ser acotada utilizando los resultados del LHC. En concreto, se ha estudiado el impacto de las búsquedas resonantes y no resonantes en los detectores ATLAS y CMS excluyendo así una amplia región del espacio de parámetros de las dos teorías. Así mismo, en el caso del modelo Randall-Sundrum se ha estudiado el posible impacto de las próximas fases del LHC, viendo que la exclusión prácticamente alcanzará zonas ya eliminadas por diferentes limitaciones teóricas.

%Por último, más allá del escenario WIMP, se ha estudiado otro candidato a Materia Oscura que se caracteriza por su débil interacción, la Materia Oscura tipo FIMP. En este escenario, la Materia Oscura interacciona tan débilmente con el resto de partículas que jamás llegó a estar en equilibrio en el Universo primigenio. La abundancia de Materia Oscura medida actualmente sería consecuencia de un proceso totalmente diferente al del caso WIMP, el denominado \textit{freeze-in}. Como consecuencia de su débil interacción, la Materia Oscura tipo FIMP es un candidato perfecto si únicamente asumimos interacción gravitatoria. En este contexto se ha estudiado la posibilidad de obtener la abundancia de Materia Oscura en el escenario de Randall-Sundrum 5-dimensional. Nuestro análisis muestra que la región del espacio de parámetros de la teoría en la cual es posible reproducir la abundancia actual de Materia Oscura es enorme. Las diferentes cotas experimentales y teóricas limitan mucho menos el espacio de parámetros que en el caso WIMP. Así mismo, las previsiones sobre los futuros límites impuestos por el LHC apenas restringen la región permitida. De este modo, el candidato FIMP es más prometedor que el candidato WIMP en el escenario de Randall-Sundrum y la inaccesibilidad del LHC a ciertas regiones permitidas del espacio de parámetros representan una motivación para nuevos experimentos de física de altas energías.

Nuestro escaso conocimiento acerca de la naturaleza de la Materia Oscura hace que el conjunto de modelos que pueden explicar las evidencias actuales sea enorme. Esta Tesis ha contribuido a explorar parte de estos modelos y acotar un poco más lo que sabemos de ella, estudiando la fenomenología de diferentes candidatos. En general, los resultados obtenidos hacen que esperemos con ansia los resultados de los experimentos futuros, tanto en materia de Detección Indirecta, como en búsquedas del LHC. La relevancia de estos futuros datos es tal que en los próximos años la existencia de los candidatos de tipo WIMP puede verse corroborada o seriamente comprometida. Por otro lado, la débil interacción de los candidatos de tipo FIMP hace que su futuro experimental sea bastante más incierto. Como comentario final, es cierto que los modelos aquí estudiados representan una ínfima parte de todo el abanico de posibilidades existentes en la actualidad para explicar este escurridizo tipo de materia. No obstante, espero que hayan arrojado algo de luz sobre tan oscuro misterio.

%Nuestro escaso conocimiento acerca de la naturaleza de la Materia Oscura hace que el conjunto de modelos que pueden explicar las evidencias actuales sea enorme. Esta Tesis ha contribuido a explorar parte de estos modelos y acotar un poco más lo que sabemos de ella, estudiando la fenomenología de diferentes candidatos. En general, los resultados obtenidos hacen que tengamos un ojo puesto en los experimentos futuros, tanto en materia de Detección Indirecta, como en búsquedas del LHC. La relevancia de estos futuros datos es tal que en los próximos años la existencia de los candidatos de tipo WIMP y FIMP puede verse corroborada o seriamente comprometida. Como comentario final, es cierto que los modelos aquí estudiados representan una ínfima parte de todo el abanico de posibilidades existentes en la actualidad para explicar este escurridizo tipo de materia. No obstante, espero que hayan arrojado algo de luz sobre tan oscuro misterio.


==> Chapters/Resumen_Tesis/Resumen_Tesis_auxiliar.tex <==
\inputencoding{latin1}
\include{Umlaute}       % ISO-8859-1 encoding
\inputencoding{utf8} % back to UTF-8


\chapter{Resumen de la Tesis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Motivación Histórica}

Desde tiempos inmemoriales, uno de los más profundos deseos del ser humano ha sido descubrir la composición última de la materia que nos rodea. Ya los primeros escritos griegos hablan sobre la modelización de la naturaleza en base a cuatro elementos fundamentales; a saber, agua, tierra, fuego y viento. El paso de los siglos afinó mucho más esta prematura descripción. En el siglo XVII, se sintetizó por primera vez un elemento químico\footnote{En 1669 el alquimista Hennig Brand sintetizó por accidente fósforo, bautizándolo con este nombre por el brillo que desprendía.}, y tan solo dos siglos después (1869), ya existía una tabla periódica de los elementos, un claro reflejo de nuestro anhelo por encontrar orden en el caos.

El elevado número de elementos descubiertos en el siglo XX motivó la búsqueda de una estructura mucho más fundamental, aún totalmente desconocida. Fue Niels Bohr quien dió forma a esta idea, al sentar las bases de la teoría atómica actual \cite{Bohr:1913:CAMa,Bohr:1913:CAMb,Bohr:1913:CAMc}, apoyándose en los modelos atómicos propuestos previamente por Joseph John Thomson y Ernest Rutherford. Su elegante modelo explicaba toda forma de matéria utilizando únicamente tres tipos de partículas: neutrones y protones, que componían el núcleo de los diferentes elementos atómicos, y electrones, los cuales orbitaban alrededor de dichos núcleos con energías cuantizadas. Los átomos quedaban descritos pues como pequeños sistemas planetarios, solo que las fuerzas implicadas en su estabilidad eran totalmente diferentes a la gravitatoria.

\begin{figure}[htbp]
\centering
\includegraphics[width=80mm]{figures/Standard_Model_of_Elementary_Particles.pdf}
\caption[Modelo Estándar de las interacciones fundamentales]{\it Modelo Estándar de las interacciones fundamentales: las partículas moradas, verdes y rojas representan, respectivamente, los quarks, leptones y bosones de gauge. Por otro lado, la amarilla representa el Bosón de Higgs. Imagen tomada de Ref.~\cite{citaSM}.}
 \label{fig:modelo_estandar}
\end{figure}

A lo largo del siglo XX el desarrollo de la mecánica cuántica cambió totalmente la forma de entender el mundo microscópico. A la fuerza gravitatoria y electromagnetica se le sumaron dos nuevas interacciones: débil y fuerte. Por otro lado, los protones y neutrones, que en el modelo de Bohr eran constituyentes fundamentales de la materia, pasaron a ser partículas compuestas por quarks, mientras una nueva plétora de partículas eran descubiertas gracias a los rayos cósmicos y a la construcción de nuevos experimentos y detectores. El resultado último de toda la revolución cuántica fue el Modelo Estándar de la física de partículas \cite{PhysRevLett.19.1264,GLASHOW1961579,Salam:1968rm,PhysRevLett.13.321,PhysRev.145.1156,PhysRevLett.13.508,PhysRevLett.13.585,PhysRev.155.1554,PhysRev.139.B1006,PhysRevD.2.1285,FRITZSCH1973365}, esquematizado en la Fig.~\ref{fig:modelo_estandar}. El modelo describe la naturaleza a nivel microscópico utilizando un total de doce partículas elementales, o campos, y cuatro tipos de interacción. Los éxitos del Modelo Estándar fueron totalmente rotundos, con él se han realizado las predicciones más precisas de la historia de la ciencia. No obstante, tiene ciertas limitaciones, como el hecho de que es incapaz de describir la gravedad cuántica. En el Capitulo \ref{sec:SM} se ha realizado una descripción detallada del modelo, profundizando en sus predicciones y fallos.

Hoy, casi medio siglo después de que fuese propuesto, sabemos que el Modelo Estandar únicamente es capaz de explicar el $5\%$ del contenido del Universo, el $95\%$ restante continua envuelto en un halo de misterio. Observaciones astrofísicas y cosmológicas indican que el $26\%$ del Universo está compuesto por un nuevo tipo de materia cosmológicamente estable que no emite luz, y que no puede identificarse con ninguna de las partículas del Modelo Estándar. \nuria{Esta curiosa característica inspiró su nombre, \textit{Materia Oscura}}. El resto del Universo es aún más enigmático si cabe. Actualmente se cree que está compuesto por algún tipo de energía que explicaría la expansión acelerada del Universo, pero esto es otra historia muy diferente a la de la Materia Oscura y queda lejos de los objetivos del trabajo aquí realizado.

La motivación de esta Tesis es intentar arrojar algo de luz sobre ese gran porcentaje de materia que nuestra ciencia actual no ha sido capaz de explicar, haciéndola un poco menos oscura de lo que su nombre indica.


\section{El Modelo Estándar de las Interacciones Fundamentales: La Piedra Angular de la Física de Altas Energías} 
\label{sec:modelo_estandar}

En esta sección vamos a realizar un breve resumen de los conceptos más importantes del Modelo Estándar (en el Capitulo \ref{sec:SM} se han explicado todos los detalles técnicos del mismo). El Modelo Estándar de la física de partículas\footnote{Típicamente abreviado como SM, del inglés Standard Model.} es una teoría cuántica de campos con simetría gauge de los grupos unitarios $SU(3)_C \times SU(2)_L \times U(1)_Y$. El modelo describe con gran precisión tres de las cuatro interacciones fundamentales que existen en la naturaleza: débil, electromagnética y fuerte. La complejidad de la estructura de la interacción gravitatoria hace que sea muy complicado describirla como una teoría de campos gauge, actualmente se trabaja activamente en el tema\footnote{Algunos autores defienden que quizá el origen de la interacción gravitatoria sea totalmente diferente al resto de fuerzas fundamentales. La gravedad emergente (propuesta por Andrei Sakharov en 1967, el artículo original en inglés puede encontrarse en Ref.~\cite{Sakharov_1991}), por ejemplo, sugiere que dicha interacción no es más que el residuo de una serie de grados de libertad aún desconocidos, tal como la mecánica de fluidos, que deriva de la mecánica estadística.}. El resto de las interacciones fundamentales quedan descritas con gran precisión por el modelo mediante el intercambio de diferentes campos de spin 1, que constituyen el sector gauge de la teoría. Mientras que el grupo $SU(3)_C$  se asocia a la interacción fuerte, los grupos $SU(2)_L \times U(1)_Y$ describen la interacción electrodébil\footnote{Las interacciones electromagnéticas y débiles fueron unificadas en los años 70 por Sheldon Lee Glashow, Abdus Salam y Steven Weinberg.}

Mientras que las partículas de spin $1$, o bosones, describen las interacciones del modelo, los constituyentes fundamentales de la materia son los fermiones, partículas de spin $1/2$: quarks y leptones. Curiosamente, la naturaleza replica los fermiones en 3 familias casi idénticas, únicamente diferenciadas por las masas de sus constituyentes: 
\bea
\label{familia_1_CS}
\nth{1} \, \text{Family}: L_{1} \equiv \left( \begin{array}{c}
\nu_e  \\
e^{-}  \end{array} \right)_{L} \, ; \, e_1 \equiv e^{-}_{_R} \, ; \, 
Q_1 \equiv \left( \begin{array}{c}
u  \\
d  \end{array} \right)_{L} \, ; \, U_1 \equiv u_R \, ; \, D_1 \equiv d_R \, , \nonumber \\
\label{familia_2_CS}
\nth{2} \, \text{Family}: L_{2}\equiv\left( \begin{array}{c}
\nu_{\mu}  \\
\mu^{-}  \end{array} \right)_{L} \, ; \, e_2 \equiv \mu^{-}_{_R} \, ; \,
Q_2 \equiv\left( \begin{array}{c}
c  \\
s  \end{array} \right)_{L} \, ; \, U_2 \equiv c_R \, ; \, D_2 \equiv s_R \, , \nonumber \\
\label{familia_3_CS}
\nth{3} \, \text{Family}: L_{3}\equiv\left( \begin{array}{c}
\nu_{\tau}  \\
\tau^{-}  \end{array} \right)_{L} \, ; \, e_3 \equiv \tau^{-}_{_R} \, ; \, 
Q_3 \equiv\left( \begin{array}{c}
t  \\
b  \end{array} \right)_{L} \, ; \, U_3 \equiv t_R \, ; \, D_3 \equiv b_R \, . \nonumber
\eea
\miguel{Por otro lado, el modelo trata de forma diferente a partículas con quiralidad dextrógira y levógira, agrupando las primeras en singletes y las segundas en dobletes de $SU(2)_L$}. De este modo, los quarks y leptones levógiros vienen representados por $Q_i$ (compuesto por los quarks tipo \textit{up} y tipo \textit{down}, con cargas eléctricas $+2/3$ y $-1/3$ de la carga fundamental del electrón, respectivamente) y $L_i$ (compuesto por los leptones cargados y los neutrinos, con cargas eléctricas $-1$ y $0$, respectivamente). Por otro lado, los quarks dextrógiros están representados por los singletes $U_i$ y $D_i$, mientras que los leptones cargados dextrógiros vienen dados por $e_i$.
Los neutrinos dextrógiros no están incluidos en el modelo original, aunque hay muchas líneas de investigación abiertas en la actualidad sobre la posibilidad de su existencia.

Aparte de todo lo comentado, el modelo incluye un campo de spin 0, el campo de Higgs. Los bosones gauge de la teoría débil, es decir $Z$ y $W^\pm)$, tienen masa. Este hecho parecía incompatible con la construcción de un modelo basado en simetrías ya que la invariancia gauge prohíbe términos de masa para los bosones gauge. Por ello, fue necesario desarrollar un mecanismo que dotase de masa estas partículas. La solución a este problema llegó de la mano de Robert Brout, Francois Englert, Gerald Guralnik, Carl Richard Hagen, Peter Higgs y Tom Kibble (en estricto orden alfabético), constituyendo lo que popularmente se conoce como \textit{mecanismo de Higgs} \cite{PhysRevLett.13.321,PhysRev.145.1156,PhysRevLett.13.585,PhysRev.155.1554}.

La idea del mecanismo de Higgs se basa en la \textit{ruptura espontánea de la simetría}\footnote{Del inglés \textit{Spontaneous Symmetry Breaking}.} (SSB) y consiste en agregar a la teoría un campo complejo escalar doblete de $SU(2)_L$:
\be
\Phi = \left( \begin{array}{c}
\Phi^+  \\
\Phi^0  \end{array} \right) = 
\left( \begin{array}{c}
\Phi^+  \\
\dfrac{1}{\sqrt{2}}(v + \phi_1 + i\phi_2)  \end{array} \right) \, .
\ee
Este peculiar campo presenta lo que se conoce como \textit{valor esperado de vacío}\footnote{Del inglés de \textit{Vacuum Expectation Value}.} (VEV) no nulo en su componente neutra, produciendo de este modo una ruptura de la simetría electrodébil (que no es una simetría exacta del vacío) y dando como resultado la simetría electromagnética\footnote{La abreviación QED viene de \textit{Quantum Electrodynamics} \cite{10.1143/PTP.1.27,10.1143/ptp/2.3.101,10.1143/ptp/3.2.101,PhysRev.74.224,PhysRev.74.1439,Feynman:1948ur,Feynman:1949zx}, nombre que recibe la teoría gauge que describe la interacción electromagnética.},
\be
SU(2)_L\times U(1)_Y \longrightarrow U(1)_{QED}.
\ee

\miguel{Durante la SSB, tanto la parte cargada del doblete como la parte imaginaria de la componente neutra son absorbidos como grados de libertad longitudinales por los bosones gauge de la teoría, los cuales pasan a comportarse como bosones masivos.} Por otro lado, la parte real del campo cargado, $\phi_1$, se queda presente en el espectro de partículas del Modelo Estándar como una partícula de spin 0, el popular \textit{bosón de Higgs}. Detectado en 2012 por los experimentos ATLAS \cite{Aad_2012} y CMS del LHC \cite{Chatrchyan_2012}, confirmando el modelo.

Las representaciones de los fermiones del Modelo Estándar bajo el grupo $SU(2)_L\times U(1)_Y$ no presentan simetría quiral, necesaria para que los correspondientes términos de masa puedan aparecer en el lagrangiano del modelo. No obstante, el mecanismo de Higgs soluciona este problema ya que bajo el grupo $U(1)_{\text{QED}}$ si que presentan dicha simetría. En consecuencia, después de la SSB, el VEV del campo de Higgs permite la formación de los términos de masa para estas partículas.

Para una exposición detallada y completa del Modelo Estándar en español ver Ref.~\cite{gelmini2014el}.

\section{La Necesidad de la Materia Oscura}

Como ya hemos comentado, el Modelo Estandar de partículas solo puede explicar un porcentaje pequeño de la materia que nos rodea, conocida como \textit{bariónica}\footnote{Nombre que recibe la materia descrita por el Modelo Estándar.}. El resto de materia que puebla el Universo recibe el nombre de Materia Oscura. A pesar de que este exótico tipo de materia es un activo campo de estudio en la actualidad, los primeros indicadores de su existencia son ya casi centenarios \cite{Zwicky:1933gu}. No obstante, las primeras pruebas sólidas se las debemos a los trabajos de Vera Cooper Rubin, Kent Ford y Ken Freeman, llevados a cabo allá por los años 60 \cite{1970ApJ...159..379R,1970ApJ...160..811F}.

\subsection{Evidencias de la Existencia de Materia Oscura}
\label{sec:res:evidencias}

La evidencia más clara que tenemos a día de hoy de la existencia de la Materia Oscura son las curvas de rotación de las galaxias. El contenido en masa de una galaxia puede medirse en base a su luminosidad, mediante técnicas astrofísicas. De este modo, tenemos una clara idea de cuanta materia bariónica hay en una determinada galaxia y como está distribuida dentro de ella. Conocida la masa de la galaxia, la velocidad de rotación de un objeto situado a una distancia $R$ del centro de la misma puede determinarse a partir de las leyes de Kepler\footnote{$v = \sqrt{MG/R}$, donde $M$ es la masa contenida en la esfera de radio $R$ y $G$ la constante de gravitación universal.}. De acuerdo con esto, la distribución de materia bariónica observada nos indica que la velocidad de rotación debería disminuir conforme nos acercamos al borde galáctico. Sin embargo, medidas directas sobre la velocidad de rotación indican lo contrario: en la mayoría de los casos esta velocidad de rotación permanece constante.

Las curvas de rotación de las galaxias son la evidencia más famosa de la existencia de este exótico tipo de materia, pero no la única. La teoría de la Relatividad General predice que el campo gravitatorio producido por un gran cúmulo de materia es capaz de desviar los rayos de luz, el conocido como efecto \textit{lente gravitatoria}. De este modo, puede utilizarse la luz procedente de galaxias lejanas para, mediante ciertos estudios sobre la trayectoria de los haces de luz, determinar la cantidad de materia que hay en los cúmulos de galaxias situados en su trayectoria. Este análisis confirma la presencia de Materia Oscura en la mayoría de cúmulos de galaxias estudiados.

Aparte de las evidencias astrofísicas, hay muchas otras evidencias cosmológicas que confirman la existencia de la Materia Oscura. En la Sec.~\ref{sec:evidences} se ha realizado una breve descripción de todas ellas.

\subsection{Características Fundamentales}

A pesar de las evidencias de su existencia, a día de hoy aún no se ha realizado ninguna observación directa de la Materia Oscura. No obstante, podemos inferir mucho acerca de su naturaleza:
\begin{itemize}
\item La Materia Oscura debe ser no bariónica: algunos candidatos bariónicos han sido propuestos a lo largo de los años, como es el caso de los MACHOs\footnote{Del inglés \textit{Massive Compact Halo Objects}.} \cite{1986ApJ...304....1P}. No obstante, los límites sobre esta clase de modelos son tan fuertes en la actualidad que están prácticamente descartados en su totalidad.
\item Debe ser \textit{fría} o \textit{cálida}: según la distancia recorrida, como consecuencia de movimientos aleatorios, por las partículas de Materia Oscura en el Universo primigenio, podemos catalogarla en tres grandes grupos: \textit{calinte}, \textit{cálida} y \textit{fría}. Si la distancia recorrida es mayor, igual o menor que el tamaño de una protogalaxia \miguel{(unos 100 años luz)}, la Materia Oscura será caliente, cálida o fría, respectivamente. En la actualidad se han realizado numerosas simulaciones numéricas de la evolución del Universo con diferentes tipos de materia. Si la Materia Oscura fuese caliente, de acuerdo con estas simulaciones, el Universo tendría un aspecto muy diferente al que conocemos hoy en día \cite{primack2001happened}.
\item Debe colisionar muy débilmente consigo misma: el motivo de esto es que recientes observaciones astrofísicas, tales como las realizadas sobre el conocido como \textit{cúmulo bala}\footnote{Este curioso cúmulo es el resultado de dos cúmulos actualmente en colisión. En él se observa un efecto muy exótico, el centro de masas del cúmulo resultante se encuentra desplazado. Esta característica solo puede ser explicada mediante la existencia de grandes cantidades de Materia Oscura en su composición. La alternativa requeriría una modificación de las leyes más fundamentales de la dinámica relativista.}, imponen restricciones a la autointeracción de la Materia Oscura \cite{Dave_2001,Feng_2009,Agrawal_2017,Randall_2008,Kahlhoefer_2013}:
\be
\sigma/m \lesssim 10^{-24} \, \text{cm}^2/\text{GeV} .
\ee
\item Débilmente interactiva con la materia bariónica: \miguel{aparte de la interacción gravitatoria, la única interacción posible que podría llegar a tener la Materia Oscura es la débil. Respecto a lo que al electromagnetismo se refiere, las diversas implicaciones que supone la existencia de Materia Oscura cargada han sido profundamente estudiadas en la literatura \cite{DERUJULA1990173}, descartando prácticamente esta opción por motivos experimentales\footnote{En la actualidad las técnicas de detección de partículas cargadas son tan avanzadas que de existir la Materia Oscura eléctricamente cargada, esta ya debería haber sido observada.} \cite{Taoso:2007qk}.
Por otro lado, de existir la Materia Oscura fuertemente interactiva\footnote{Fuertemente en el sentido de interacción a través de la interacción fuerte.}, ésta dejaría huella incluso en el flujo de calor terrestre \cite{Mack:2007xj}. Las fuertes implicaciones de este tipo de candidatos hacen que esten excluidos casi en su totalidad.}
\item Debe ser estable: la Materia Oscura que observamos hoy en día en el Universo es prácticamente un fósil térmico: es el remanente de la que la que componía el Universo primigenio. La única forma de que ese remanente haya sobrevivido hasta nuestros días es que la Materia Oscura sea estable o, en su defecto, que su vida media sea mayor que la edad del Universo.
\end{itemize}

En la Sec.~\ref{sec:Properties} se ha realizado un estudio mucho más profundo de todas estas propiedades.

\subsection{Candidatos Estudiados}

Hasta el momento hemos hablado de las diferentes evidencias y características de la Materia Oscura. Pero ¿cuál es su naturaleza? En el escenario científico actual se han propuesto muchos candidatos a Materia Oscura, desde todo tipo de partículas con interacciones parecidas a las que ya conocemos, hasta candidatos altamente exóticos como agujeros negros primigenios \cite{10.1093/mnras/168.2.399,1975ApJ...201....1C,10.1093/mnras/152.1.75}. Todo esto ha sido detallado en la Sec.~\ref{sec:candidates}. En este resumen únicamente hablaremos sobre los dos candidatos estudiados en esta Tesis: las partículas WIMP \cite{PhysRevLett.39.165} y las FIMP \cite{Hall:2009bx}.

\subsubsection{Materia Oscura tipo WIMP}

Las partículas WIMP\footnote{Su nombre deriva del inglés \textit{Weakly Interactive Massive Particles}, es decir, partículas masivas débilmente interactivas.} son partículas con masas típicamente desde el GeV hasta varios TeV. Este candidato se basa en la suposición de que las partículas de Materia Oscura se encontraban en equilibrio térmico con el resto de partículas del Modelo Estándar en el Universo primigenio. La abundancia que observamos en la actualidad sería pues el resultado de un proceso denominado \textit{freeze-out}.

Para entender bien el concepto de \textit{freeze-out}, debemos remontarnos a los primeros instantes del Universo, justo después del Big Bang. En aquella época, los átomos no existían, las diferentes partículas que poblaban el Universo se encontraban en un equilibrio continuo de aniquilación/producción, formando un plasma de altísima temperatura. Poco a poco, el Universo fue expandiéndose, enfriando dicho plasma. El enfriamiento del Universo provocó que algunos de los procesos que mantenían este equilibrio dejasen de tener lugar, desacoplando de este modo las diferentes especies de partículas de este \textit{caldo} primigenio.

Cuando la temperatura del Universo fue demasiado baja como para que la creación de partículas de Materia Oscura fuese posible, está se desacopló del \textit{caldo} primigenio. Como consecuencia, la abundancia de estas partículas comenzó a disminuir, hasta que fue tan pequeña que la probabilidad de que dos partículas de Materia Oscura se encontrasen y se aniquilasen se volvió prácticamente nula. A dicha temperatura, conocida como temperatura de \textit{freeze-out}, la abundancia de Materia Oscura superviviente se convirtió en un leve remanente, un mero fósil térmico, que ha llegado hasta nuestros días.

Este candidato a Materia Oscura ha gozado de gran acogida por los físicos teóricos desde que fuese propuesto alla por los años 70. El motivo de tal popularidad es que en el rango de masas mencionado, curiosamente, para reproducir la abundancia de Materia Oscura actual, se necesita que la interacción entre ésta y las partículas del Modelo Estándar sea justo del orden de la interacción electrodébil. Hecho, cuanto menos sorprendente, que se conoce como \textit{Milagro WIMP}. En este rango de masas la sección eficaz necesaria para conseguir dicha abundancia es prácticamente independiente del valor de la masa de la partícula WIMP,
\be
\langle \sigma v \rangle \backsimeq 2 \times 10^{-26}\, \text{cm}^3/\text{s} \backsim 1 \, \text{pb} \, .
\ee
Los detalles matemáticos y técnicos de este candidato a Materia Oscura se encuentran explicados en la Sec.~\ref{Sec:freezeout}.

\subsubsection{Materia Oscura tipo FIMP}

Complementariamente al caso WIMP, existe la Materia Oscura tipo FIMP\footnote{Nombre que deriva del ingles \textit{Feebly Interactive Massive Particle}.} la cual jamás llegó al equilibrio térmico con el resto de partículas del Modelo Estándar. En este escenario la Materia Oscura fue producida por diversos procesos durante la época de enfriamiento del Universo, después del Big Bang, siendo nula en el origen de los tiempos. Cuando la temperatura del Universo fue suficientemente baja, esta producción se congeló, dejando un remanente que ha llegado hasta nuestros días. Este mecanismo de producción recibe el nombre de \textit{freeze-in}\footnote{El mecanismo de producción fue propuesto en Ref.~\cite{Chung:1998rq}. Aunque en aquella época ni el mecanismo se conocía por dicho nombre, ni el candidato como FIMP.} y está detallado en la Sec.~\ref{Sec:freezein}.

\miguel{La Materia Oscura FIMP no ha llegado a alcanzar la popularidad de la Materia Oscura tipo WIMP. Hay varios motivos para ello pero el principal es que debido a su baja intensidad de interacción es muy dificil buscar pruebas experimentales de su existencia.}

\section{Detección de Materia Oscura}

Como hemos comentado en la Sec.~\ref{sec:evidences}, y resumido en Sec.~\ref{sec:res:evidencias}, tenemos muchas evidencias de la existencia de a Materia Oscura. No obstante, no se ha conseguido realizar ninguna observación directa de estas elusivas partículas\footnote{Existe una llamativa excepción: el experimento DAMA/Libra ha medido variaciones en la modulación solar que pueden ser interpretadas como Materia Oscura \cite{Bernabei:2008yi,Bernabei:2010mq}. No obstante, esta señal no está libre de controversia entre la comunidad científica ya que ningún otro experimento ha reportado absolutamente nada en el rango de masas en el que DAMA/Libra mide dicha señal.}. A pesar de esto, las técnicas de detección de Materia Oscura han avanzado mucho en los últimos años, poniendo cotas cada vez más restrictivas a la existencia de estas partículas aparentemente invisibles.
Dentro del gran abanico de experimentos de detección, estos pueden clasificarse en dos grandes grupos: la \textit{Detección Directa}\footnote{Del ingles \textit{Direct Detection.}} DD y la \textit{Deteccion Indirecta}\footnote{Del ingles \textit{Indirect Detection.}} ID.

\subsection{Detección Directa}

La idea de la Detección Directa (cuyos detalles técnicos se discuten en profundidad en la Sec.~\ref{Sec:DD}) fue propuesta por primera vez por Mark Goodman y Edward Witten \cite{Goodman:1984dc}. Como la Materia Oscura no presenta cargas eléctricas, es imposible detectarla mediante técnicas electromagnéticas. No obstante, la existencia de colisiones entre la DM y los núcleos atómicos abre una puerta para su observación directa. 

En general, esta clase de detecciones se realizan en experimentos ubicados bajo tierra. Ejemplos notables son Xenon1T \cite{PhysRevLett.121.111302} o LUX \cite{Akerib:2016vxi}, los cuales están compuestos por grandes cantidades de Xenón. La colisión de la Materia Oscura con los átomos de Xenón produciría una excitación de estos últimos, que finalmente se traduciría en la emisión de un fotón. Hasta el momento, no se ha realizado ninguna detección en dichos experimentos, lo cual pone fuertes límites sobre los modelos de Materia Oscura, haciendo que los escenarios más simples y \textit{naturales} estén prácticamente descartados.

\begin{figure}[htbp]
\centering
\includegraphics[width=130mm]{figures/direct_detection_bounds.pdf}
\caption[Estatus actual de los experimentos de detección directa.]{\it Límites actuales a la sección eficaz de interacción de Materia Oscura con nucleones. La región verde está excluida por los experimentos de Detección Directa con un 90\% de intervalo de confianza. Las dos zonas rojas muestran las regiones en las que DAMA/LIBRA afirma haber observado Materia Oscura. La zona amarilla representa el \textit{suelo  de neutrinos} \cite{Billard:2013qya}.}
 \label{fig:direct_detection_bounds_resumen}
\end{figure}

Uno puede hacerse una idea del panorama actual de estos experimentos mirando la Fig.~\ref{fig:direct_detection_bounds_resumen}. En ella, la zona verde muestra los valores de la sección eficaz de Detección Directa, como función de la masa de la Materia Oscura, que ya han sido descartados por los experimentos. Por otro lado, para hacernos una idea de magnitud de la zona ya eliminada, podemos mirar lo cerca que se encuentra de ella la región amarilla. Esta región muestra lo que se conoce como \textit{suelo de neutrinos}\footnote{En ingles conocido como \textit{neutrino floor}.} \cite{Billard:2013qya} y representa \miguel{la sección eficaz} para la que los experimentos de detección comenzarán a observar colisiones producidas por los neutrinos. Realizar exclusiones mediante experimentos de Detección Directa en esta región es complicado, puesto que la señal de ambos tipos de colisión es indistinta. Las dos regiones rojas muestran las observaciones de DAMA/LIBRA en zonas totalmente excluidas por el resto de experimentos.

\subsection{Detección Indirecta}

La observación directa de las colisiones de las partículas de Materia Oscura con los núcleos atómicos no es la única técnica para detectarla. Diferentes experimentos astronómicos llevan años intentando observar los posibles productos de las aniquilaciones de las partículas de Materia Oscura en los rayos cósmicos que nos llegan a la Tierra. Es posible distinguir entre tres tipos de flujos de partículas: fotones, neutrinos y partículas cargadas (como electrones, positrones, etc).

En general, de los diferentes flujos de partículas que llegan a la Tierra, los resultados más prometedores (en lo que a Materia Oscura se refiere) vienen de los fotones. Desde 2008 la colaboración Fermi-LAT analiza el flujo de fotones procedente de diferentes \textit{galaxias enanas} \cite{Fermi-LAT:2016uux,Ackermann:2015zua}. Hasta el momento el estudio se restringe a 15 ejemplares y por el momento los resultados no muestran ningún exceso en el flujo analizado que no pueda ser explicado por el Modelo Estándar de partículas. Esto pone cotas a modelos de nueva física en los cuales la Materia Oscura pueda aniquilarse a partículas que finalmente se desintegren en fotones, generalmente en el rango de masas $m_{\text{DM}} \in (0.5,500) $ GeV. No obstante, desde 2009 el mismo experimento ha estado reportando un exceso inexplicable de fotones procedente del centro galáctico\footnote{Popularmente conocido como \textit{Galactic Center $\gamma$-ray excess} (GCE) \cite{Goodenough:2009gk, Vitale:2009hr, Hooper:2010mq, Gordon:2013vta, Hooper:2011ti, Daylan:2014rsa, 2011PhLB..705..165B, Calore:2014xka, Abazajian:2014fta,Zhou:2014lva}.}. Aunque su origen aún es desconocido, este exceso, que se observa a una energía $\sim 3$ GeV, puede ser explicado por diferentes modelos de Materia Oscura.

Por otro lado, las señales procedentes de flujos de antipartículas cargadas acotan de una forma mucho menos restrictiva los modelos de Materia Oscura. El problema con esta clase de flujos es su propagación desde el punto en el que son generados hasta la Tierra (donde finalmente los detectamos). Hoy en día existen diversos modelos para ello, pero su precisión aún tiene que ser perfeccionada para que los límites impuestos por esta clase de flujos sean realmente restrictivos.

En la Sec.~\ref{Sec:ID} se ha realizado un análisis exhaustivo de la Detección Indirecta de Materia Oscura.

\section{Dimensiones Extra}

De entre las cuatro fuerzas fundamentales de la naturaleza, no cabe ninguna duda de que la gravedad es la más complicada de entender a nivel cuántico. A pesar de los muchos esfuerzos por parte de la comunidad científica, aún no tenemos una teoría cuántica para describirla.
Por otro lado, la gravedad es la más débil de las interacciones fundamentales. Tal es el caso, que de existir nueva física a la escala gravitatoria, el Modelo Estándar se enfrentaría a un serio problema: las correcciones a la masa del bosón de Higgs son muy sensibles a la escala de la nueva física. Teniendo en cuenta la diferencia entre la escala de Planck\footnote{La escala de la interacción gravitatoria.} y la escala electrodébil, de aparecer nueva física a la escala gravitatoria las correcciones a la masa del Higgs serían enormes, requiriendo cancelaciones ajustadas entre distintos órdenes de teoría de perturbaciones para explicar el valor medido. A este fenómeno se le conoce como \textit{problema de la jerarquía} (para un analisis más detallado del problema mirar la Sec.~\ref{sec:hierarchyproblem}). Entre las diversas propuestas que se han realizado para intentar resolver este problema se encuentran las dimensiones extra.

\subsection{Dimensiones Extra \textit{Grandes} (LED)}

El primer modelo de dimensiones extra que se propuso para dar solución al problema de la jerarquía fue \textit{Large Extra-Dimensions} (LED) \cite{ArkaniHamed:1998rs}. En este escenario se asume que las nuevas dimensiones tienen una forma similar a las tres espaciales ya conocidas, es decir, presentarían un aspecto plano. De acuerdo con el modelo LED, el tamaño de estas nuevas dimensiones sería finito o, en otras palabras, estarían compactificadas. Por otro lado, mientras que la gravedad se propaga libremente por el espacio 5-dimensional, el resto de campos del Modelo Estándar se encuentran confinados en unas hipersuperficies 4-dimensionales denominadas \textit{branas}. Este hecho hace que la gravedad se diluya a través de las dimensiones extra, haciendo que en la brana (donde nosotros vivimos confinados) su intensidad parezca anómalamente débil. De este modo, la escala de la gravitación, que para nosotros es $M_\text{P} = 1.22 \times 10^{19}$ GeV, en el espacio extra-dimensional completo sería $M_D$. \miguel{Ambas escalas están relacionadas a través del radio de compactificación de las dimensiones extra ($r_c$):
\be
M_\text{P}^2 = M_{D}^{D-2} (2\pi r_c)^D.
\ee 
}

Para el caso particular de 5 dimensiones, el espacio-tiempo queda definido en este modelo por la métrica:
\be
ds^2 = \eta_{\mu \nu}dx^\mu dx^\nu + r_c^2dy^2,
\ee
Donde la dimensión extra está representada por $y$. Este parámetro puede escogerse de manera que $M_5 \backsim \text{TeV}$, resolviendo así el problema de la jerarquía.
No obstante, si imponemos esta condición, el modelo LED 5-dimensional está excluido totalmente a día de hoy: agregar una única dimensión extra en LED predice correcciones de la ley de la gravitación universal que podrían observarse en distancias parecidas al tamaño del Sistema Solar. \miguel{No obstante, aunque el modelo esté excluido para una única dimensión extra, con dos o más dimensiones es posible resolver el problema de la jerarquía sin entrar en contradicciones con la ley de la gravitación universal.}

\subsection{Dimensiones Extra Deformadas: Modelo de Randall-Sundrum}

A pesar de que los modelos LED presentan diversos problemas, pusieron la semilla para modelos futuros muy interesantes. El caso más popular es el modelo propuesto por Lisa Randall y Raman Sundrum a finales de los años 90, conocido como \textit{dimensiones extra deformadas} o \textit{modelo de Randall-Sundrum} (RS) \cite{Randall:1999ee}. En dicho modelo, las nuevas dimensiones presentan curvatura, a diferencia de LED, donde eran planas. En el modelo original de RS el espacio extra-dimensional está delimitado por dos branas. Todos los campos de materia viven atrapados en una de ellas (brana \textit{infrarroja} (IR), también llamada brana del TeV), mientras que la otra brana se encuentra vacía (brana \textit{ultravioleta} (UV) o de Planck). Por otro lado, la gravedad se propaga libremente por el espacio extra-dimensional (comúnmente conocido como \textit{bulk}). La geometría del modelo hace que los diferentes parámetros fundamentales con dimensión de masa sufran un proceso de deformación exponencial a lo largo del bulk, resolviendo así el problema de la jerarquía.

Concretamente, para el caso 5-dimensional (una única dimensión extra), la métrica que definiría este espacio tiempo vendría dada por
\be
ds^2 = e^{-2  kR|y|}\eta_{\mu \nu} dx^\mu dx^\nu - r_c^2 dy \, ,
\label{RS_metric_resumen}
\ee
Donde $k$ es la curvatura a lo largo de la dimensión extra y $r_c$ su radio de compactificación. El factor exponencial que multiplica la parte 4-dimensional de la métrica recibe el nombre de factor de deformación.
$M_5$ y $M_\text{P}$ quedarían entonces relacionados mediante los dos parámetros libres de la teoría:
\be
\bar{M_\text{P}}^2 = \frac{M_5}{k} \left( 1 - e^{-2 k \pi r_c} \right) \, .
\ee
Vemos que hay una clara diferencia con el modelo LED: en RS $M_5\backsimeq M_\text{P}$. Sin embargo, la modificación que sufren los parámetros medidos en la brana IR, debido a la presencia del factor de deformación, resuelve el problema de la jerarquía para $k\,r_c \backsim 10 $.

\miguel{En RS la gravedad puede describirse a través del intercambio de gravitones no masivos 5-dimensionales, los cuales surgen de perturbaciones sobre la componente 4-dimensional de la métrica
\be
G^{(4)}_{\mu \nu} = e^{-2kr_c|y|} (\eta_{\mu \nu} + 2M_5^{-2/3} h_{\mu \nu}) \, .
\label{perturbacion_4dim}
\ee
No obstante, la proyección de este campo 5-dimensional sobre las branas es equivalente a una torre de gravitones 4-dimensionales masivos, comúnmente conocidos como modos de Kaluza-Klein (KK). La escala efectiva de la interacción de estos gravitones 4-dimensionales con los campos confinados en la brana IR viene dada por
\be
\Lambda \equiv \bar{M_\text{P}} e^{-k \pi r_c} \, .
\ee
Por otro lado, cada gravitón de esta torre de partículas tiene una masa diferente que dependerá de los parámetros libres ($k,r_c$) del modelo y de su respectivo orden dentro de la torre. No obstante, establecida la masa del primer gravitón $m_1$, la masa del resto de gravitones queda totalmente fijada. La fenomenología de los modelos de RS puede ser descrita mediante los parámetros ($\Lambda,m_1$), en lugar de ($k,r_c$). Este hecho puede ser muy útil debido a su relación con observables fenomenológicos.}

\miguel{El modelo asume que la distancia entre las branas está fijada, pero no aporta ningún mecanismo para estabilizar este parámetro dinámicamente. La solución a este problema fue propuesta por Walter D. Goldberger y Mark B. Wise \cite{Goldberger:1999wh,Goldberger:1999uk}. Este mecanismo utiliza un nuevo campo escalar que se propaga libremente por el \textit{bulk}, sometido a unos potenciales localizados en las branas. 
Por otro lado, el nuevo campo escalar se mezcla con el ya presente en el \textit{bulk}, el graviescalar $G_{55}^{(5)}$ (el cual emerge de las perturbaciones sobre la parte 5-dimensional de la métrica). Al campo resultante de esta mezcla se le conoce como radión. La masa de este nuevo campo no está determianda por el modelo y representa un nuevo grado de libertad.}

\miguel{El modelo asume que la distancia entre las branas está fijada, pero no aporta ningún mecanismo para estabilizar este parámetro dinámicamente. La solución a este problema fue propuesta por Walter D. Goldberger y Mark B. Wise \cite{Goldberger:1999wh,Goldberger:1999uk}. Este mecanismo utiliza un nuevo campo escalar que se propaga libremente por el \textit{bulk}, \nuria{sometido a} unos potenciales localizados en las branas. 
Por otro lado, el nuevo campo escalar se mezcla con el ya presente en el \textit{bulk}, el graviescalar $G_{55}^{(5)}$ (el cual emerge de las perturbaciones sobre la parte 5-dimensional de la métrica). Al campo resultante de esta mezcla se le conoce como radión. \nuria{Los mínimos de los potenciales en la brana IR y UV son diferentes, lo que genera un valor esperado de vacío para (este nuevo campo escalar) el radi�n. El tamaño de la quinta dimensión ($r_c$) está entonces relacionado con este valor esperado de vacio.La masa del radi�n no está determianda por los par�metros del modelo original, y representa un nuevo grado de libertad.}

El modelo de RS ha gozado de gran popularidad desde que fue propuesto a finales de los 90's. La literatura sobre modelos de física más allá del Modelo Estándar desarrollados en este escenario es inmensa. En la Sec.~\ref{sc:warped} se ha realizado un análisis de los detalles técnicos del modelo.  

\subsection{Dimensiones extra tipo \textit{Clockwork/Linear Dilaton}}

\miguel{Durante casi dos decadas lo modelos de RS fueron los únicos que resolvian el problema de la jerarquía mediante la introducción de dimensiones con curvatura. No obstante, en 2016 Gian Giudice y Matthew McCullough propusieron un nuevo modelo de dimensiones extra curvadas. Este nuevo modelo, propuesto en Ref.~\cite{Giudice:2016yja} y cuya fenomenología fue estudiada en Ref.~\cite{Giudice:2017fmj}, se conoce con el nombre de \textit{Clockwork/Linear Dilaton} (CW/LD).}

\miguel{Este modelo, que fue encontrado como límite continuo de los modelos \textit{Clockwork} discretos, puede caracterizarse a traves de la métrica:
\be
\label{eq:5dmetric_resumen}
ds^2 = e^{4/3 k r_c |y|} \left ( \eta_{\mu \nu} dx^{\mu}dx^{\nu} - r_c^2 \, dy^2 \right ) \, ,
\ee
donde $k$ y $r_c$ representan la curvatura y el radio de compactificación de la quinta dimensión, respectivamente. Para determinados valores de los parámetros libres, el modelo es capaz de resolver el problema de la jerarquía.}

El modelo CW/LD guarda ciertas similitudes con RS. En ambos casos el espacio 5-dimensional está delimitado por las branas IR y UV. El caso mínimo implica tener todo el Modelos Estándar confinado en la brana IR, mientras que la gravedad se propaga libremente por el bulk 5-dimensional. Sin embargo, hay diferencias notables con RS. En primer lugar, la relación entre $M_5$ y $M_\text{P}$ en CW/LD viene dada por
\be
M_{\text{P}}^2 = \frac{M_5^3}{k} \left ( e^{2 \pi r_c}  - 1 \right ) \, ,
\ee 
pudiendo ser esta del orden del TeV (al igual que en el caso LED). Por otro lado, el acoplamiento de \miguel{los gravitones de KK} a las partículas localizadas en la brana es diferente para cada gravitón:
\be
\dfrac{1}{\Lambda_{n}} =  \dfrac{1}{\sqrt{M_5^3 \pi r_c}}  \left ( 1 + \dfrac{k^2 r_c^2}{n^2} \right )^{-1/2} 
=  \dfrac{1}{\sqrt{M_5^3 \pi r_c}} \left ( 1 - \dfrac{k^2}{m_n^2} \right )^{1/2}  \,  .
\ee
Este hecho hace que describir la fenomenología en base a $\Lambda_n$ no sea tan útil como en RS. Otra diferencia notable es que hay una relación muy interesante entre el valor de la curvatura $k$ y la masa del primer gravitón $m_1$, haciendo que ambos parámetros sean prácticamente idénticos.

\miguel{En el caso CW/LD, el tamaño de la quinta dimension puede estabilizarse sin necesidad de introducir ningún nuevo campo. La forma del modelo genera unos potenciales en las branas IR y UV a traves del campo de dilatación (\textit{dilaton}), $S = 2 k r_c |y|$, de la métrica. Esto permite fijar la posición de las branas de un modo similar a como se hacía en RS.}

\section{Metodología Utilizada}

Antes de ponernos a hablar sobre los cuatro proyectos que conforman la presente Tesis, es necesario comentar las diferentes técnicas (tanto a nivel analítico como numérico) utilizadas en el desarrollo de los mismos. 

A nivel analítico, la complejidad de los problemas estudiados ha requerido un profundo conocimiento de la teoría cuántica de campos. Se han utilizado los desarrollos perturbativos de dicha teoría para obtener las diferentes probabilidades de interacción utilizadas posteriormente en los estudios fenomenológicos. Los modelos aquí estudiados asumen Materia Oscura tipo WIMP y FIMP. En ambos casos, la evolución de la abundancia de Materia Oscura a lo largo de la historia térmica del Universo requiere resolver la Ecuación de Boltzman, que determina la evolución de sistemas fuera del equilibrio térmico. Por otro lado, se ha trabajado con dos modelos de dimensiones extra:  Randall-Sundrum y Clockwork/Linear Dilatón. La fenomenología estudiada sobre estos modelos ha requerido un análisis exhaustivo de ambos escenarios.

Desde un punto de vista numérico, toda la fenomenología ha sido estudiada mediante lenguaje \textit{C++}, mientras que su representación a nivel gráfico ha sido obtenida utilizando \textit{python}. El análisis de la Detección Indirecta de Materia Oscura realizado en uno de los modelos estudiados ha requerido el uso de software más específico: \textit{micrOMEGAs}, \textit{SARAH}, \textit{gamlike}, \textit{pythia} y \textit{MadGraph}. Por otro lado, todo el estudio de la Ecuación de Boltzman en los cuatro modelos se ha realizado mediante métodos numéricos implementados en lenguaje \textit{C++}.

Finalmente, el enfoque fenomenológico que presenta esta Tesis ha implicado un contacto continuo con datos experimentales. El tratamiento de estos datos, así como las diferentes cotas de exclusión que han puesto sobre los diferentes modelos estudiados, ha requerido un uso de diversas técnicas estadísticas. Se han utilizado diferentes distribuciones de probabilidad (tales como la conocida $\chi^2$), técnicas de Monte Carlo, etc.

\section{Resultados y conclusiones de la Tesis}

En está sección, vamos a realizar un breve resumen de los proyectos que conforman esta Tesis. Todos ellos pueden encontrarse completos en la Parte \ref{sec:papers}.

\subsection{Estudio de la Detección Indirecta del Modelo de \textit{Portal de Neutrinos Estériles}}

Uno de los grandes problemas abiertos en física de altas energías es la Materia Oscura, pero desde luego no es el único. Entre los diversos problemas que existen actualmente en el Modelo Estándar de partículas, uno de los más importantes es la masa de los neutrinos. El modelo predice una masa nula para ellos, no obstante, hace ya más de medio siglo se predijo un efecto denominado \textit{oscilaciones de neutrinos} \cite{Pontecorvo:1957cp}. Este curioso fenómeno, que fue confirmado experimentalmente en 1999 \cite{Fukuda:1998mi}, consiste en una oscilación en el sabor leptónico de los neutrinos. Las implicaciones de este hecho son muy profundas ya que únicamente puede suceder si al menos uno de los tres sabores de neutrinos es masivo\footnote{\miguel{A pesar de que el fenómeno podría explicarse con un solo neutrino masivo, la observación del fenomeno tanto en neutrinos atmosfericos como solares requiere que al menos dos de los tres sabores de neutrinos sean masivos.}}. No obstante, las cotas experimentales impuestas a la masa de estas partículas prácticamente invisibles son tan fuertes que su masa debe ser muy pequeña\footnote{El límite actual más fuerte viene dado por el experimento \textit{Karlsruhe Tritio Neutrino} (KATRIN) \cite{Aker:2019uuj}.}.
Este hecho potenció el desarrollo de modelos en los que la masa de los neutrinos era generada por mecanismos de tipo \textit{balancín}\footnote{Modelo \textit{seesaw} en inglés.} \cite{GellMann:1980vs,PhysRevLett.44.912,Yanagida:1979as,Glashow1111,MINKOWSKI1977421}. Hay diferentes versiones de estos modelos, en el \textit{tipo I}, por ejemplo, se asume la existencia de neutrinos dextrógiros muy masivos que justifican la pequeña masa de los neutrinos del Modelo Estándar. La mezcla de los neutrinos levógiros con los dextrogiros da como resultado los autoestados de masa, prediciendo neutrinos con masas muy grandes y muy pequeñas.

La posibilidad de que el problema de la Materia Oscura y de la masa de los neutrinos estén relacionados motivó el desarrollo del conocido como\footnote{El escenario más económico, la posibilidad de que los neutrinos estériles sean la Materia Oscura, fue propuesto en Ref.~\cite{Dodelson:1993je}. A día de hoy, esta posibilidad ha sido fuertemente estudiada y prácticamente descartada \cite{Adhikari:2016bei}.} \textit{portal de neutrinos estériles a Materia Oscura} \cite{Escudero:2016tzx,Macias:2015cna,Escudero:2016ksa}. Este modelo se ha estudiado por diversos autores, acotándolo utilizando la Detección Directa de Materia Oscura. No obstante, es un modelo muy interesante desde el punto de vista de la Detección Indirecta por varios motivos. Por un lado, la Detección Directa en este escenario no sucede al orden más bajo en teoría de perturbaciones de la teoría cuántica de campos. Este hecho hace que sus señales de Detección Directa sean bajas que en otros modelos, empeorando así los límites impuestos. Por otro lado, la conexión de los neutrinos estériles con los neutrinos activos hace que las aniquilaciones de Materia Oscura produzcan, como resultado de diversas desintegraciones, excesos de fotones y partículas cargadas. Todo esto lo convierte en el candidato perfecto para ser estudiado desde el punto de vista de la Detección Indirecta, tal como se ha llevado a cabo en la Ref.~\cite{Folgado:2018qlv}.

En este trabajo hemos analizado un modelo particular en el que, además de los neutrinos estériles, se asume la existencia de dos nuevos campos: uno escalar $\phi$ y otro fermionico $\Psi$. Estos campos son ambos singletes del Modelo Estándar, no obstante, están cargados respecto a un nuevo grupo de simetría, $G_{\text{dark}}$, de tal forma que la combinación $ \overline{\Psi} \phi$ es singlete de este nuevo grupo de simetría.

\begin{figure}[htbp]
\centering
\includegraphics[width=120mm]{figures/resultados_paper_1.pdf}
\caption[Resultados del primer articulo.]{\it Límites sobre el \textit{portal de neutrinos estériles} en el espacio de masas. La región amarilla muestra los límites impuestos por los antiprotones mientras que la región azul son los límites impuestos por los fotones procedentes de las galaxias enanas. Los diferentes contornos muestran la zona en la que el modelo es capaz de reproducir el GCE. La línea discontinua azul muestra nuestra predicción sobre el límite de las galaxias enanas para los próximos 15 años.}
 \label{fig:resultados_paper_1}
\end{figure}

La más ligera de estas nuevas partículas \textit{oscuras} ($\phi$ y $\Psi$) es estable si todas las particulas del Modelo Estándar, así como los neutrinos esteriles, son singletes de $G_{\text{dark}}$, independientemente de la naturaleza de este grupo de simetría. Como consecuencia, debido a su estabilidad esta partícula es un buen candidato a Materia Oscura. Por simplicidad, asumimos que $G_{\text{dark}}$ es una simetría global a baja enería, en cualquier caso no esperamos cambios significantes en nuestro analisis fenomenológico si esta fuese local.

Los terminos más relevantes en el lagrangiano vienen dados por:
\bea
\mathcal{L} &=& \mu_H^2 H^\dagger H - \lambda_H (H^\dagger H)^2  -
\mu_\phi^2 \phi^\dagger \phi - \lambda_\phi (\phi^\dagger \phi)^2 - 
\lambda_{H\phi} (H^\dagger H) \, (\phi^\dagger \phi)   
\nonumber \\
&-&\left( \phi \overline{\Psi}(  \lambda_a +  \lambda_p \gamma_5) N 
 + Y \overline {L}_L H N_{R}  + {\rm h.c.}  \right)  \, .
\eea

Los acoplamientos de Yukawa $Y$ entre los neutrinos dextrógiros $N_R$ y el doblete leptónico del Modelo Estándar genera las masas para los neutrinos activos después de la ruptura espontanea de la simetría, a traves del mecanismo \textit{balancín} de tipo I. Si bien se requieren al menos dos neutrinos estériles para generar las masas de neutrinos observadas en las oscilaciones, en nuestro análisis consideramos que solo una especie es más ligera que la Materia Oscura y, por lo tanto, relevante para la determinación de su abundancia y búsquedas indirectas. No obstante, los resultados son fáclmtente extendibles al caso en el que tenemos dos o más neutrinos estériles más ligeros que la Materia Oscura. Bajo el supuesto de que la Materia Oscura es descrita por $\Psi$ (el análisis es igualmente valido en el caso de que la Materia Oscura sea $\phi$) las masas del modelo cumplen la relación $m_N < m_\Psi < m_\phi$.

La Fig.~\ref{fig:resultados_paper_1} muestra los resultados finales de nuestro análisis. Fijando la masa del mediador escalar para obtener la abundancia de Materia Oscura mediante el mecanismo \textit{freeze-out} (es decir $\langle \sigma \, v \rangle \sim 2 \times 10^{-26} cm^3/s$), la figura muestra los diferentes limites impuestos por las búsquedas de fotones y antiprotones en el espacio de masas $(M_N,M_\Psi)$. Como ya hemos comentado, el experimento Fermi-LAT ha reportado un exceso de fotones inexplicable procedente del centro galáctico (GCE). El modelo estudiado predice un pequeño exceso de fotones que podría ser compatible con el GCE en ciertas zonas del espacio de parámetros. En nuestro analisis hemos asumidoque existen dos fuentes diferentes para el GCE: una astrofísica, responsable de la zona de alta energía del espectro de fotones, y otra procedente de las aniquilaciones de Materia Oscura, la cual explicaría la zona de baja energía del exceso,  
\be
\Phi = \Phi_{\text{astro}} + \Phi_{\text{DM}} \, .
\ee
Esta contribución astrofísica al flujo de fotones es siempre necesaria para reproducir el GCE, independientemente del modelo de Materia Oscura considerado.
La zona en la que puede realizarse el ajuste del exceso de fotones del centro galactico está delimitada por los diferentes contornos que se observan en la figura (en la leyenda está indicado el p-valor asociado a cada contorno). No obstante, este aumento de fotones predicho por el modelo tiene que ser compatible también con el resto de medidas realizadas sobre los diferentes flujos de fotones. En concreto, el mismo experimento realiza medidas sobre los fotones procedentes de 15 galaxias enanas\footnote{Galaxias compuesta por varios millones de estrellas. En contraposición tenemos las galaxias normales, compuestas por varios miles de millones.}, la región sombreada en azul muestra la zona del espacio de parámetros de la teoría en la cual los resultados obtenidos no son compatibles con dichas mediciones al 90 \% de intervalo de confianza.

Por otro lado, el modelo también predice un aumento del flujo de antiprotones. Este aumento se ha comparado con el flujo de antiprotones procedente del centro galáctico, el cual es medido en la actualidad por el experimento AMS-02.Los resultados obtenidos muestran que existen zonas en las cuales las predicciones del modelo no serían compatibles al 95 \% de intervalo de confianza con lo observado experimentalmente (zona sombreada en amarillo en la figura).
Por último, también se ha realizado un análisis del posible impacto de los resultados futuros el experimento Fermi-LAT. Basandonos en la mejora experimentada por la colaboración, hemos estimado que en 15 años se habrán detectado 45 galaxias enanas nuevas. Este hecho podría poner fuertes cotas al modelo estudiado (línea azul discontinua). Como comentario final, podemos decir que algunos modelos de Materia Oscura son capaces de explicar el exceso de fotones del centro galactico parcialmente\footnote{Hasta el momento todos los modelos necesitan asumir que parte del exceso es consecuencia a fenomenos astrofísicos.}. En concreto, el modelo aquí estudiado consigue reproducirlo con una precisión muy alta. No obstante, los resultados futuros del experimento Fermi-LAT podrían excluir casi por completo la región del espacio de parámetros en la cual el GCE puede ser explicado por el modelo.

\subsection{Materia Oscura Escalar Mediada por Gravedad en Dimensiones Extra Deformadas}

Todas las evidencias que tenemos hoy en día acerca de la existencia de la Materia Oscura están relacionadas con la interacción gravitatoria. Este hecho induce a pensar en la posibilidad de que las partículas de Materia Oscura únicamente interactúen gravitatoriamente. Esta idea tan natural ha sido explorada ya para los candidatos de tipo WIMP sin demasiado exito: la intensidad de la interacción gravitatoria es muy débil y hace imposible obtener la cantidad de abundancia de Materia Oscura que se observa en la actualidad (al menos en el escenario WIMP). No obstante, ¿que ocurre si pensamos en más de 4 dimensiones? Esta es la idea que inspiró la Ref.~\cite{Folgado:2019sgz}.

En dicho artículo tratamos de explorar si es posible obtener la abundancia de Materia Oscura actual, asumiendo que es de tipo WIMP escalar, únicamente mediante interacción gravitatoria y bajo el supuesto de un Universo 5-dimensional de tipo Randall-Sundrum. En el escenario descrito, la Materia Oscura y el Modelo Estándar viven confinados en la brana infrarroja. Ambos tipos de materia interactúan únicamente a través de la gravedad, cuya proyección sobre la brana IR es equivalente a una torre de gravitones 4-dimensionales masivos (torre de Kaluza-Klein).

El modelo queda descrito en base a cuatro parámetros físicos: la escala de la interacción de los gravitones 4-dimensionales con la materia, $\Lambda$; la masa del primer gravitón de la torre de KK, $m_{1}$; la masa del candidato a Materia Oscura, $m_{\text{DM}}$ y la masa del radión, $m_r$. Nuestro estudio muestra que cuando $m_r < m_\text{DM}$ y, en consecuencia, el canal de aniquilación a radiones esta abierto, el valor de $m_r$ es prácticamente irrelevante para la fenomenología. 
Respecto a la aniquilación de la Materia Oscura a partículas del Modelo Estandar a traves del intercambio de radiones virtuales, esta sección eficaz únicamente es relevante cerca de la resonancia $m_\text{DM} \backsim m_r/2$. Por lo tanto, en el estudio fenomenológico realizado hemos fijado la masa del radion y nos hemos centrado en el resto de parámetros libres del modelo.

El método seguido para el análisis del modelo ha sido la construcción de una malla bidimensional con diferentes valores de los parámetros $(m_{G_1},m_\text{DM})$. Para cada uno de los puntos de este mallado hemos buscado si existe algún valor de $\Lambda$ para el cual se obtiene la abundancia de Materia Oscura actual (es decir, para $\langle \sigma v \rangle \backsimeq \langle \sigma v \rangle_\text{fo} = 2 \times 10^{-26} \, \text{cm}^3/\text{s}$). De este modo, para cada punto del mallado los tres parámetros libres ($m_{1}$, $m_\text{DM}$, $\Lambda$) quedan totalmente definidos. Este análisis nos permite establecer diferentes límites teóricos y experimentales en el espacio de masas del modelo. 

\begin{figure}[t]
\centering
\includegraphics[width=150mm]{figures/resultados_paper_2.png}
\caption[Resultados del segundo articulo.]{\it Región en el plano $(m_{\text{DM}}, m_{1})$ para la cual 
$\left\langle \sigma v \right\rangle = \left\langle \sigma_{\rm fo} v \right\rangle$. La gráfica de la izquierda muestra el caso sin radión, mientras que en la de la derecha se ha considerado $m_r = 100$ GeV. Las líneas discontinuas muestran los diferentes valores de $\Lambda$ en el plano ($m_\text{DM},m_{1}$) para los cuales se consigue la abundancia actual de Materia Oscura. La zona gris muestra la región en la cual es imposible conseguir la abundancia de Materia Oscura, independientemente del valor de $\Lambda$. Por otro lado, la región naranja nos indica los puntos en los que la abundancia se consigue gracias a los canales de interacción en los que interviene el radión. Respecto a los límites sobre el modelo: la zona de cuadraditos verde representa el límite de unitariedad; la zona de cuadraditos rosa representa la zona en la que la teoría efectiva deja de tener validez, es decir $\Lambda < m_{1}$; la zona roja representa los límites impuestos por el experimento Xenon1T sobre la sección eficaz de Detección Directa; la región azul es la zona eliminada por las búsquedas de resonancias en el LHC usando los datos de 36 fb$^{-1}$ at $\sqrt{s} = 13$ TeV. Finalmente, las líneas punteadas son las predicciones de exclusión para las fases \textit{Run-III} (con $\sim 300$ fb$^{-1}$) y \textit{High Luminosity} (con $\sim 3000$ fb$^{-1}$) del LHC.}
 \label{fig:resultados_paper_2}
\end{figure}

En la Fig.~\ref{fig:resultados_paper_2} pueden verse los resultados finales del análisis fenomenológico sobre el modelo. En la parte izquierda se ha explorado el caso sin radión, asumiendo que podría encontrarse algún método alternativo para estabilizar el radio de la quinta dimensión. Por otro lado, en la parte derecha se ha considerado que la masa del radión es $m_r = 100$ GeV (es importante recordar que la fenomenología no se ve afectada por el valor de esta masa). La zona sombreada en gris es la región en la que no es posible obtener la abundancia actual de Materia Oscura para ningún valor de $\Lambda$, mientras que la zona naranja representa la región del espacio de parámetros en la que la abundancia se consigue gracias a las contribuciones de los canales de interacción radiónicos. La zona sombreada con cuadraditos verdes se conoce como límite de unitariedad y representa el punto a partir del cual la sección eficaz de interacción es tan alta que la teoría de campos deja de tener sentido, esto sucede para\footnote{\miguel{En el escenario WIMP las partículas de Materia Oscura tienen una velocidad relativa muy pequeña. Este hecho implica que $s \backsimeq m_{\text{DM}}^2 (4 + v^2_{\text{rel}}) $, donde $v_{\text{rel}}$ es la velocidad relativa de las partículas de Materia Oscura, se asume que es pequeña. Ademas, debemos recordar que para conseguir la abundancia de Materia Oscura observada en la actualidad debe cumplirse $\sigma = \sigma_{\text{fo}}$. Como consecuencia, este límite se convierte en un límite sobre la masa de la Materia Oscura $m_{\text{DM}}^2 \lesssim 1/\sigma_{\text{fo}}$. Por lo tanto, enel plano de masas ($m_\text{DM}$, $m_1$) la zona excluida por unitariedad aparece como una linea vertical.}} $\sigma > 1/s$. Además de este límite, existe otra restriccion teórica: si $\Lambda < m_{\text{DM}}, m_{1}$ la teoría efectiva que describe la interacción de estos campos cuánticos deja de tener sentido (ya que deberían estar integrados). Esto ocurre en la región de cuadraditos rosa.

Hasta el momento, hemos hablado de las diferentes restricciones al modelo por motivos teóricos, pero estos no son los únicos límites que pueden establecerse: los actuales experimentos de Detección Directa y las búsquedas de resonancias en los experimentos ATLAS y CMS del LHC pueden aportar mucha información a nuestro análisis. De este modo, las zonas sombreadas en rojo representan los puntos en los que la sección eficaz de Detección Directa está ya excluida por los actuales experimentos. Por otro lado, la zona azul es la excluida por las búsquedas de resonancias (gravitones 4-dimensionales en nuestro caso) en el LHC, se han utilizado los datos tomados a $\sqrt{s} = 13$ TeV con 36 fb$^{-1}$ en el canal $\gamma \gamma$. Las dos líneas punteadas muestran nuestra predicción sobre los límites futuros que serán impuestos por el LHC después de las futuras fases \textit{Run-3} (con $\sim 300$ fb$^{-1}$) y \textit{High Luminosity} (con $\sim 3000$ fb$^{-1}$), en el caso de que no se detecte ninguna resonancia.

El estudio realizado muestra que, en las regiones no excluidas del espacio de parámetros, la fenomenología está dominada por los canales de interacción relacionados con los gravitones. En dichas regiones, de acuerdo con nuestro análisis, los canales de interacción radiónicos siempre son subdominantes. Para ser más exactos, la abundancia se consigue gracias a la aniquilación de Materia Oscura directamente en gravitones.

Aunque ya se habían realizado análisis similares en Randall-Sundrum, este trabajo es el primero que tiene en cuenta los canales de aniquilación de Materia Oscura directamente a gravitones en regiones tan altas del espacio de masas (varios TeV). Así mismo, se ha estudiado un diagrama totalmente olvidado en la literatura hasta el momento: la aniquilación a gravitones sin mediador, procedente del desarrollo a segundo orden del lagrangiano de interacción. Aunque el impacto de este diagrama sobre la fenomenología no cambia drásticamente los resultados, debe ser añadido por consistencia ya que es del mismo orden que el resto de diagramas estudiados. Por otro lado, cabe destacar que este análisis únicamente se ha realizado para Materia Oscura escalar. No obstante, en la Ref.~\cite{Folgado:2020vjb} que está actualmente en trámites de publicación, se analizan los casos de Materia Oscura fermiónica y vectorial. En este estudio se ve que la Materia Oscura de tipo fermionico está claramente desfavorecida respecto a la escalar y vectorial ya que el canal dominante (la aniquilación directamente a gravitones) está más suprimido que en el resto de casos.

\subsection{Materia Oscura Mediada por Gravedad en Dimensiones Extra Tipo \textit{Clockwork/Linear Dilatón}}

Analizadas las implicaciones de la existencia de Materia Oscura tipo WIMP con interacciones puramente gravitatoria en el escenario de Randall-Sundrum, la pregunta de que ocurriría en el novedoso Clockwork/Linear Dilatón casi surge de forma natural. Esta idea inspiró la Ref.~\cite{Folgado:2019gie}. La estructura de este escenario es diferente a la que teníamos en RS: la torre de KK de gravitones masivos en este caso tiene una separación muy pequeña y variable. Este hecho dificulta en gran medida el análisis numérico de su fenomenología.

A nivel conceptual, la estrategia para abordar el modelo es idéntica a la empleada en el caso RS. La gran diferencia con el modelo anterior son los parámetros elegidos para estudiar la fenomenología. En CW/LD los acoplamientos de los gravitones 4-dimensionales masivos al resto de partículas dependen del orden del gravitón dentro de la torre. Por ello, es más útil caracterizar el modelo en función de $M_5$ directamente, en lugar de usar los acoplamientos efectivos $\Lambda_n$ de los gravitones 4-dimensionales. Por otro lado, la masa del primer gravitón coincide prácticamente con el valor de la curvatura a lo largo de la quinta dimensión $m_{1} = k$. Otra diferencia notable entre ambos escenarios es la estabilización del tamaño de la dimensión extra. En RS es necesario introducir un nuevo campos escalar en el \textit{bulk} con el fin de estabilizar dinamicamente $r_c$. En cambio, en CW/LD el dilatón presente en la métrica puede utilizarse para escribir los potenciales en la brana y estabilizar así el tamaño de la quinta dimensión. En este caso, la masa del radión (modo cero de la torre de dilatones 4-dimensionales) está fijada por los parámetros fundamentales del modelo (ya que deriva directamente de la métrica). No obstante, hay diferentes formas de realizar la estabilización usando el dilatón, el caso más simple es asumir que la tensión de las branas es infinita. Este escenario, recibe el nombre de límite rigido.

\begin{figure}[htbp]
\centering
\includegraphics[width=150mm]{figures/resultados_paper_3.png}
\caption[Resultados del tercer articulo.]{\it Región en el plano $(m_{\rm DM}, k)$ para la cual $\left\langle \sigma v \right\rangle = \left\langle \sigma_{\rm fo} v \right\rangle$. Las gráficas superiores muestran los resultados para el caso de Materia Oscura escalar, la inferior izquierda el caso fermiónico y la inferior derecha el vectorial. La gráfica superior izquierda muestra las diferentes zonas de exclusión teniendo en cuenta únicamente la interacción con gravitones. Por otro lado, en la gráfica superior derecha se han considerado ambas, la interacción mediante gravitones y mediante dilatones, para el caso de Materia Oscura escalar. En los casos fermiónico y vectorial no se muestra el caso sin dilatones ya que la contribución de los mismos es despreciable y no varía los resultados. Las líneas discontínuas muestran los diferentes valores de $M_5$ en el plano ($m_\text{DM},k$) para los cuales se consigue la abundancia actual de Materia Oscura, mientras que la zona gris muestra la región en la cual es imposible conseguir dicha abundancia, independientemente del valor de $M_5$.
Respecto a los límites sobre el modelo: la zona de cuadraditos verde representa el límite de unitariedad ($m_{\rm DM} \gtrsim 1/\sqrt{\sigma_{\rm fo}}$); la región de cuadraditos rosa representa el área en la que la teoría efectiva deja de tener validez ($M_5 < k, m_\text{DM}$) y, finalmente, la región azul representa los límites impuestos por las búsquedas no-resonantes en el LHC usando los datos de 36 fb$^{-1}$ a $\sqrt{s} = 13$ TeV para el canal $\gamma \gamma$ \cite{Giudice:2017fmj}.}
 \label{fig:resultados_paper_3}
\end{figure}

La Fig.~\ref{fig:resultados_paper_3} muestra los diferentes límites obtenidos para este escenario. Análogamente al caso RS, $M_5$ se ha utilizado para fijar la abundancia actual de Materia Oscura para cada punto del espacio ($m_{\text{DM}},k$). Los diferentes límites estudiados son los mismos que en el caso anterior: la región de cuadraditos rosa muestra los límites de la teoría efectiva ($M_5 < k, m_\text{DM}$), la región de cuadraditos verdes el límite de unitariedad ($m_{\rm DM} \gtrsim 1/\sqrt{\sigma_{\rm fo}}$) y, finalmente, la zona sombreada en azul los límites impuestos por el LHC. En el caso de los límites experimentales, debido a la proximidad de las resonancias en la torre de gravitones, el límite más estricto impuesto por el LHC viene de las búsquedas en el espectro continuo de energías, en lugar de las búsquedas de resonancias. Estos límites han sido calculados usando los datos de 36 fb$^{-1}$ a $\sqrt{s} = 13$ TeV para el canal $\gamma \gamma$ \cite{Giudice:2017fmj}. Finalmente, cabe destacar que, en este caso, los límites impuestos por las búsquedas de Detección Directa de Materia Oscura corresponden a valores de ($m_\text{DM},k$) menores que los mostrados en la Figura. 

Otra diferencia notable con el caso RS es que aquí no solo hay que considerar el radión en la fenomenología, si no también toda la torre de KK de los dilatones. No obstante, en CW/LD el radión y los dilatones derivan directamente de la métrica del modelo, no es necesario un mecanismo externo para estabilizar el tamaño de la quinta dimensión. Este hecho hace que la masa de los mismos este intrínsecamente ligada a los parámetros fundamentales del modelo, sin agregar de este modo ningún grado nuevo de libertad al espacio de parámetros de la teoría.

En este trabajo se han analizado los tres posibles tipos de Materia Oscura: escalar, fermiónica y vectorial. Las dos figuras superiores corresponden al caso escalar sin tener en cuenta la torre de radión y dilatones (izquierda) y teniéndola en cuenta (derecha), respectivamente. Este es el único caso en el que los dilatones juegan un papel importante en la fenomenología del modelo y por ello merece la pena mostrar cuál es su impacto sobre los resultados finales. Las gráficas inferiores corresponden al caso fermiónico (izquierda) y al caso vectorial (derecha). Se puede ver claramente que el caso fermiónico está desfavorecido respecto a los otros dos. Este hecho se debe a que en el caso fermiónico el canal dominante, la aniquilación de Materia Oscura directamente a gravitones, sufre una supresión debido al momento angular total.

El análisis llevado a cabo en este trabajo representa el primer estudio fenomenológico del modelo CW/LD con presencia de Materia Oscura. Los resultados anteriores, al igual que en RS, son prometedores en el sentido de que toda la región no excluida podrá ser analizada en los próximos años por el LHC. Como comentario final sobre la Materia Oscura tipo WIMP púramente gravitatoria, podemos decir que en ambos escenarios es posible reproducir la abundancia actual en el rango $m_\text{DM} \in [1,10] \, \text{TeV}$. No obstante, los valores necesarios, tanto de $\Lambda$ en RS como de $M_5$ en CW/LD, para ello son excesivamente grandes como para resolver el problema de la jerarquía.

\subsection{Materia Oscura FIMP en Dimensiones Extra Deformadas}

Hasta el momento, todos los modelos analizados consideran partículas tipo WIMP. No obstante, la Materia Oscura tipo FIMP es muy interesante para el caso en el que la interacción es puramente gravitatoria. En el último proyecto incluido en esta Tesis hemos explorado la posibilidad de reproducir la abundancia de Materia Oscura actual utilizando partículas FIMP en un escenario tipo RS \cite{Bernal:2020fvw}. Este caso plantea complicaciones matemáticas y numéricas muy diferentes al caso WIMP. Entre estos problemas, el más importante es que la abundancia final predicha por el modelo depende en gran medida de las condiciones iniciales. Este hecho hace que, mientras que en el caso WIMP\footnote{Como consecuencia del \textit{milagro WIMP}.} la abundancia actual se reproduce para un valor constante de la sección eficaz de interacción ($\left\langle \sigma v \right\rangle = \left\langle \sigma_{\rm fo} v \right\rangle$), en el caso FIMP es necesario resolver siempre la ecuación diferencial que determina su evolución, la conocida como ecuación de Boltzmann.

\begin{figure}[htbp]
\centering
\includegraphics[width=110mm]{figures/resultados_paper_4.pdf}
\caption[Resultados del cuarto articulo.]{\it Valores de la temperatura de reheating (lineas negras) para los cuales un determinado valor de la escala de interacción en la brana y la masa del primer graviton reproducen la abundancia de Materia Oscura actual para $m_\text{DM} = 1$ MeV y $m_r = m_1/10^3$. La zona azul representa la región excluida por las búsquedas de resonancias del LHC. La región roja muestra el límite de la teoría efectiva $m_1>\Lambda$. Finalmente, la región verde muestra la zona en la que el valor de la vida media del radión entra en conflicto con las observaciones de la Nucleosíntesis del Big Bang.}
 \label{fig:resultados_paper_4}
\end{figure}

Por otro lado, aquí la abundancia también tiene una fuerte dependencia con un nuevo parámetro: la temperatura máxima del Universo, conocida como temperatura de \textit{reheating} ($T_{\text{rh}}$). Debido a la complejidad del espacio de parámetros, el analisis en este escenario se ha llevado a cabo para un valor determinado de la masa de la Materia Oscura: $m_{\textit{DM}} = 1$ MeV, no obstante, los resultados son similares para otros valores $m_{\textit{DM}} $. En la Fig.~\ref{fig:resultados_paper_4} se muestran los valores necesarios de la temperatura de reheating para obtener la abundancia observada. La región azul sombreada muestra los límites experimentales impuestos por las búsquedas de resonancias en el canal $pp \rightarrow G_1 \rightarrow \gamma \, \gamma$ en el LHC (y las dos predicciones para las futuras etapas del experimento). Por otro lado, los límites teóricos en este escenario vienen determinados por la validez de la teoría efectiva (región roja) y la \textit{Nucleosíntesis del Big Bang}. Este último límite se traduce en una restricción sobre la vida media de los gravitones y del radión: si la $\tau>1$ s se podrían producir modificaciones en las observaciones sobre la Nucleosíntesis del Big Bang que deberían estar reflejadas en los datos experimentales actuales. En los modelos analizados anteriormente, este límte no aparecia ya que la vida media de los gravitones y radion/dilatones siempre era mayor que 1 segundo. 

A la vista de los resultados obtenidos, vemos que el caso FIMP está mucho menos excluido que el caso WIMP en el escenarios de RS y que la abundancia de Materia Oscura actual se consigue en una gran región muy amplia del espacio de parámetros. A pesar de ello, los valores obtenidos para los parámetros libres de la teoría están lejos de resolver el problema de la jerarquía. Por otro lado, los experimentos actuales aún no son capaces de explorar los parámetros típicos de los modelos FIMP. No obstante, el hecho de que los modelos de Materia Oscura tipo FIMP sean capaces de explicar la abundancia actual en un rango del espacio de parámetros tan amplio es una gran motivación para el futuro desarrollo de experimentos. Actualmente estamos trabajando en el estudio análogo para el caso CW/LD.

\subsection{Conclusión}

%En esta Tesis hemos estudiado la fenomenología de diferentes modelos de Materia Oscura, centrándonos principalmente en los candidatos de tipo WIMP. En este escenario las partículas de Materia Oscura se encontraban en equilibrio termodinámico con el resto de partículas que componen el Modelo Estándar en el Universo primigenio. A causa de su expansión, el Universo sufrió un proceso de enfriamiento y las partículas de Materia Oscura terminaron por desacoplarse del plasma primigenio, dejando un remanente que ha llegado hasta nuestros días. Este proceso es denominado como \textit{freeze-out}.


%Entre los modelos estudiados en esta Tesis, se ha explorado la posibilidad de que el problema de la Materia Oscura pueda resolverse al mismo tiempo que el de la masa de los neutrinos mediante el Portal de Neutrinos Estériles. Por la estructura del modelo, este es un candidato perfecto para ser acotado usando la Detección Indirecta. Para ello, primero se ha estudiado la posibilidad de que el exceso de fotones del centro galáctico sea consecuencia de las aniquilaciones de Materia Oscura gracias a los neutrinos Estériles. Se ha visto que, efectivamente, el exceso puede ser reproducido para un pequeño rango de masas, el cual se encuentra actualmente en tensión con otras medidas experimentales: la detección de fotones procedentes de las galaxias enanas y de antiprotones procedentes del centro galáctico. Así mismo, se ha visto que a lo largo de los próximos años la mejora de las prestaciones del experimento Fermi-LAT hará, previsiblemente, que los datos recolectados acerca de las galaxias enanas sean incompatibles con la región del espacio de parámetros en la que es posible reproducir el exceso de fotones del centro galáctico.

%Por otro lado, se ha estudiado la posibilidad de que la Materia Oscura únicamente presente interacción gravitatoria. Esta idea se sustenta en el hecho de que todas las pruebas que tenemos de la existencia de la Materia Oscura están relacionadas únicamente con la interacción gravitatoria. En 4 dimensiones, como consecuencia de la debilidad de la interacción, es imposible obtener la cantidad exacta de Materia Oscura que existe actualmente en nuestro Universo. Por este motivo hemos estudiado la viabilidad de esta idea en 5 dimensiones. Efectivamente, se ha comprobado que en espacios 5-dimensionales se puede obtener la abundancia actual de Materia Oscura utilizando únicamente interacción gravitatoria. En este contexto se han analizado dos posibles modelos de dimensiones extra: el conocido modelo Randall-Sundrum y el novedoso \textit{Clockwork/Linear Dilatón}. Los resultados obtenidos en ambos casos son muy prometedores, la abundancia de Materia Oscura se obtiene en una amplia región del espacio de parámetros que puede ser acotada utilizando los resultados del LHC. En concreto, se ha estudiado el impacto de las búsquedas resonantes y no resonantes en los detectores ATLAS y CMS excluyendo así una amplia región del espacio de parámetros de las dos teorías. Así mismo, en el caso del modelo Randall-Sundrum se ha estudiado el posible impacto de las próximas fases del LHC, viendo que la exclusión prácticamente alcanzará zonas ya eliminadas por diferentes limitaciones teóricas.

%Por último, más allá del escenario WIMP, se ha estudiado otro candidato a Materia Oscura que se caracteriza por su débil interacción, la Materia Oscura tipo FIMP. En este escenario, la Materia Oscura interacciona tan débilmente con el resto de partículas que jamás llegó a estar en equilibrio en el Universo primigenio. La abundancia de Materia Oscura medida actualmente sería consecuencia de un proceso totalmente diferente al del caso WIMP, el denominado \textit{freeze-in}. Como consecuencia de su débil interacción, la Materia Oscura tipo FIMP es un candidato perfecto si únicamente asumimos interacción gravitatoria. En este contexto se ha estudiado la posibilidad de obtener la abundancia de Materia Oscura en el escenario de Randall-Sundrum 5-dimensional. Nuestro análisis muestra que la región del espacio de parámetros de la teoría en la cual es posible reproducir la abundancia actual de Materia Oscura es enorme. Las diferentes cotas experimentales y teóricas limitan mucho menos el espacio de parámetros que en el caso WIMP. Así mismo, las previsiones sobre los futuros límites impuestos por el LHC apenas restringen la región permitida. De este modo, el candidato FIMP es más prometedor que el candidato WIMP en el escenario de Randall-Sundrum y la inaccesibilidad del LHC a ciertas regiones permitidas del espacio de parámetros representan una motivación para nuevos experimentos de física de altas energías.

Nuestro escaso conocimiento acerca de la naturaleza de la Materia Oscura hace que el conjunto de modelos que pueden explicar las evidencias actuales sea enorme. Esta Tesis ha contribuido a explorar parte de estos modelos y acotar un poco más lo que sabemos de ella, estudiando la fenomenología de diferentes candidatos. En general, los resultados obtenidos hacen que esperemos con ansia los resultados de los experimentos futuros, tanto en materia de Detección Indirecta, como en búsquedas del LHC. La relevancia de estos futuros datos es tal que en los próximos años la existencia de los candidatos de tipo WIMP y FIMP puede verse corroborada o seriamente comprometida. Por otro lado, la débil interacción de los candidatos de tipo FIMP hace que su futuro experimental sea bastante más incierto. Como comentario final, es cierto que los modelos aquí estudiados representan una ínfima parte de todo el abanico de posibilidades existentes en la actualidad para explicar este escurridizo tipo de materia. No obstante, espero que hayan arrojado algo de luz sobre tan oscuro misterio.

%Nuestro escaso conocimiento acerca de la naturaleza de la Materia Oscura hace que el conjunto de modelos que pueden explicar las evidencias actuales sea enorme. Esta Tesis ha contribuido a explorar parte de estos modelos y acotar un poco más lo que sabemos de ella, estudiando la fenomenología de diferentes candidatos. En general, los resultados obtenidos hacen que tengamos un ojo puesto en los experimentos futuros, tanto en materia de Detección Indirecta, como en búsquedas del LHC. La relevancia de estos futuros datos es tal que en los próximos años la existencia de los candidatos de tipo WIMP y FIMP puede verse corroborada o seriamente comprometida. Como comentario final, es cierto que los modelos aquí estudiados representan una ínfima parte de todo el abanico de posibilidades existentes en la actualidad para explicar este escurridizo tipo de materia. No obstante, espero que hayan arrojado algo de luz sobre tan oscuro misterio.


==> Chapters/Resumen_Tesis/Resumen_Tesis_corregido_nuria.tex <==
\inputencoding{latin1}
\include{Umlaute}       % ISO-8859-1 encoding
\inputencoding{utf8} % back to UTF-8


\chapter{Resumen de la Tesis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{MotivaciÃ³n HistÃ³rica}

Desde tiempos inmemoriales, uno de los mÃ¡s profundos deseos del ser humano ha sido descubrir la composiciÃ³n Ãºltima de la materia que nos rodea. Ya los primeros escritos griegos hablan sobre la modelizaciÃ³n de la naturaleza en base a cuatro elementos fundamentales; a saber, agua, tierra, fuego y viento. El paso de los siglos afinÃ³ mucho mÃ¡s esta prematura descripciÃ³n. En el siglo XVII, se sintetizÃ³ por primera vez un elemento quÃ­mico\footnote{En 1669 el alquimista Hennig Brand sintetizÃ³ por accidente fÃ³sforo, bautizÃ¡ndolo con este nombre por el brillo que desprendÃ­a.}, y tan solo dos siglos despuÃ©s (1869), ya existÃ­a una tabla periÃ³dica de los elementos, un claro reflejo de nuestro anhelo por encontrar orden en el caos.

El elevado nÃºmero de elementos descubiertos en el siglo XX motivÃ³ la bÃºsqueda de una estructura mucho mÃ¡s fundamental, aÃºn totalmente desconocida. Fue Niels Bohr quien diÃ³ forma a esta idea, \nuria{al sentar las bases de la teorÃ­a atÃ³mica actual \cite{Bohr:1913:CAMa,Bohr:1913:CAMb,Bohr:1913:CAMc}, apoy\'andose en los modelos atÃ³micos propuestos previamente por Joseph John Thomson y Ernest Rutherford.} Su elegante modelo explicaba toda forma de materia utilizando Ãºnicamente tres tipos de partÃ­culas: neutrones y protones, que componÃ­an el nÃºcleo de los diferentes elementos atÃ³micos, y electrones, los cuales orbitaban alrededor de dichos nÃºcleos \nuria{con energías cuantizadas}. Los Ã¡tomos quedaban descritos pues como pequeÃ±os sistemas planetarios, solo que las fuerzas implicadas en su estabilidad eran totalmente diferentes a la gravitatoria.

\begin{figure}[htbp]
\centering
\includegraphics[width=80mm]{figures/Standard_Model_of_Elementary_Particles.pdf}
\caption[Modelo EstÃ¡ndar de las interacciones fundamentales]{\it Modelo EstÃ¡ndar de las interacciones fundamentales: las partÃ­culas moradas, verdes y rojas representan, respectivamente, los quarks, leptones y bosones de gauge. Por otro lado, la amarilla representa el BosÃ³n de Higgs. Imagen tomada de Ref.~\cite{citaSM}.}
 \label{fig:modelo_estandar}
\end{figure}

\miguel{A lo largo del siglo XX el desarrollo de la mecÃ¡nica cuÃ¡ntica cambiÃ³ totalmente la forma de entender el mundo microscÃ³pico. A la fuerza gravitatoria y electromagnetica se le sumaron dos nuevas interacciones: dÃ©bil y fuerte. Por otro lado, los protones y neutrones, que en el modelo de Bohr eran constituyentes fundamentales de la materia, pasaron a ser partÃ­culas compuestas por quarks,} \nuria{mientras una nueva plétora de partículas eran descubiertas gracias a los rayos cósmicos y a la construcción de nuevos experimentos y detectores}. El resultado Ãºltimo de toda la revoluciÃ³n cuÃ¡ntica fue el Modelo EstÃ¡ndar de la fÃ­sica de partÃ­culas \cite{PhysRevLett.19.1264,GLASHOW1961579,Salam:1968rm,PhysRevLett.13.321,PhysRev.145.1156,PhysRevLett.13.508,PhysRevLett.13.585,PhysRev.155.1554,PhysRev.139.B1006,PhysRevD.2.1285,FRITZSCH1973365}, esquematizado en la Fig.~\ref{fig:modelo_estandar}. El modelo describe la naturaleza a nivel microscÃ³pico utilizando un total de doce partÃ­culas elementales, o campos, y cuatro tipos de interacciÃ³n. Los Ã©xitos del Modelo EstÃ¡ndar fueron totalmente rotundos, con Ã©l se han realizado las predicciones mÃ¡s precisas de la historia de la ciencia. No obstante, tiene ciertas limitaciones, como el hecho de que es incapaz de describir la gravedad cuÃ¡ntica. En el Capitulo \ref{sec:SM} se ha realizado una exposiciÃ³n detallada del modelo, profundizando en sus predicciones y fallos.

\nuria{la materia oscura no es que no siga las reglas de la materia barionica, es que no emite luz, puedes decir que "un nuevo tipo de materia cosmológicamente estable que no emite luz, y que no puede identificarse con ninguna de las partículas del Modelo Estándar "(lleva acento en español)}
\miguel{Hoy, casi medio siglo despuÃ©s de que fuese propuesto, sabemos que el Modelo Estandar Ãºnicamente es capaz de explicar el $5\%$ del contenido del Universo, el $95\%$ restante continua envuelto en un halo de misterio}. Observaciones astrofÃ­sicas y cosmolÃ³gicas indican que el $26\%$ del Universo estÃ¡ compuesto por un nuevo tipo de materia que no sigue las mismas reglas que la materia bariÃ³nica\footnote{Nombre que recibe la materia descrita por el Modelo EstÃ¡ndar.}, comÃºnmente denominada \textit{Materia Oscura}. El resto del Universo es aÃºn mÃ¡s enigmÃ¡tico si cabe. Actualmente se cree que estÃ¡ compuesto por algÃºn tipo de energÃ­a que explicarÃ­a la expansiÃ³n acelerada del Universo, pero esto es otra historia muy diferente a la de la Materia Oscura y queda lejos de los objetivos del trabajo aquÃ­ realizado.

La motivaciÃ³n de esta Tesis es intentar arrojar algo de luz sobre ese gran porcentaje de materia que nuestra ciencia actual no ha sido capaz de explicar, haciÃ©ndola un poco menos oscura de lo que su nombre indica.


\section{El Modelo EstÃ¡ndar de las Interacciones Fundamentales: La Piedra Angular de la FÃ­sica de Altas EnergÃ­as} 
\label{sec:modelo_estandar}

En esta secciÃ³n vamos a realizar un breve resumen de los conceptos mÃ¡s importantes del Modelo EstÃ¡ndar (en el Capitulo \ref{sec:SM} se han explicado todos los detalles tÃ©cnicos del mismo). El Modelo EstÃ¡ndar de la fÃ­sica de partÃ­culas\footnote{TÃ­picamente abreviado como SM, del inglÃ©s Standard Model.} es una teorÃ­a cuÃ¡ntica de campos con simetrÃ­a gauge de los grupos unitarios $SU(3)_C \times SU(2)_L \times U(1)_Y$. El modelo describe con gran precisiÃ³n tres de las cuatro interacciones fundamentales que existen en la naturaleza: dÃ©bil, electromagnÃ©tica y fuerte. La complejidad de la estructura de la interacciÃ³n gravitatoria hace que sea muy complicado describirla como una teorÃ­a de campos gauge, actualmente se trabaja activamente en el tema\footnote{Algunos autores defienden que quizÃ¡ el origen de la interacciÃ³n gravitatoria sea totalmente diferente al resto de fuerzas fundamentales. La gravedad emergente (propuesta por Andrei Sakharov en 1967, el artÃ­culo original en inglÃ©s puede encontrarse en Ref.~\cite{Sakharov_1991}), por ejemplo, sugiere que dicha interacciÃ³n no es mÃ¡s que el residuo de una serie de grados de libertad aÃºn desconocidos, tal como la mecÃ¡nica de fluidos, que deriva de la mecÃ¡nica estadÃ­stica.}. El resto de las interacciones fundamentales quedan descritas con gran precisiÃ³n por el modelo mediante el intercambio de diferentes campos de spin 1, que constituyen el sector gauge de la teorÃ­a. Mientras que el grupo $SU(3)_C$  se asocia a la interacciÃ³n fuerte, los grupos $SU(2)_L \times U(1)_Y$ describen la interacciÃ³n electrodÃ©bil\footnote{Las interacciones electromagnÃ©ticas y dÃ©biles fueron unificadas en los aÃ±os 70 por Sheldon Lee Glashow, Abdus Salam y Steven Weinberg.}


Las partÃ­culas de spin $1$, o bosones, describen las interacciones del modelo,  en tanto que  los constituyentes fundamentales de la materia son los fermiones, partÃ­culas de spin $1/2$: quarks y leptones. Curiosamente, la naturaleza replica los fermiones en 3 familias casi idÃ©nticas, Ãºnicamente diferenciadas por las masas de sus constituyentes: 
\bea
\label{familia_1_CS}
\nth{1} \, \text{Family}: L_{1} \equiv \left( \begin{array}{c}
\nu_e  \\
e^{-}  \end{array} \right)_{L} \, ; \, e_1 \equiv e^{-}_{_R} \, ; \, 
Q_1 \equiv \left( \begin{array}{c}
u  \\
d  \end{array} \right)_{L} \, ; \, U_1 \equiv u_R \, ; \, D_1 \equiv d_R \, , \nonumber \\
\label{familia_2_CS}
\nth{2} \, \text{Family}: L_{2}\equiv\left( \begin{array}{c}
\nu_{\mu}  \\
\mu^{-}  \end{array} \right)_{L} \, ; \, e_2 \equiv \mu^{-}_{_R} \, ; \,
Q_2 \equiv\left( \begin{array}{c}
c  \\
s  \end{array} \right)_{L} \, ; \, U_2 \equiv c_R \, ; \, D_2 \equiv s_R \, , \nonumber \\
\label{familia_3_CS}
\nth{3} \, \text{Family}: L_{3}\equiv\left( \begin{array}{c}
\nu_{\tau}  \\
\tau^{-}  \end{array} \right)_{L} \, ; \, e_3 \equiv \tau^{-}_{_R} \, ; \, 
Q_3 \equiv\left( \begin{array}{c}
t  \\
b  \end{array} \right)_{L} \, ; \, U_3 \equiv t_R \, ; \, D_3 \equiv b_R \, . \nonumber
\eea
\miguel{Por otro lado, el modelo trata de forma diferente a partÃ­culas con quiralidad dextrÃ³gira y levÃ³gira, agrupando las primeras en singletes y las segundas en dobletes de $SU(2)_L$}. De este modo, los quarks y leptones levÃ³giros vienen representados por $Q_i$ (compuesto por los quarks tipo \textit{up} y tipo \textit{down}, con cargas elÃ©ctricas $+2/3$ y $-1/3$ de la carga fundamental del electrÃ³n, respectivamente) y $L_i$ (compuesto por los leptones cargados y los neutrinos, con cargas elÃ©ctricas $-1$ y $0$, respectivamente). Por otro lado, los quarks dextrÃ³giros estÃ¡n representados por los singletes $U_i$ y $D_i$, mientras que los leptones cargados dextrÃ³giros vienen dados por $e_i$.
Los neutrinos dextrÃ³giros no estÃ¡n incluidos en el modelo original, aunque hay muchas lÃ­neas de investigaciÃ³n abiertas en la actualidad sobre la posibilidad de su existencia.

Aparte de todo lo comentado, el modelo incluye un campo de spin 0, el campo de Higgs. Los bosones gauge de la teorÃ­a dÃ©bil, es decir $Z$ y $W^\pm$, tienen masa. Este hecho parecÃ­a incompatible con la construcciÃ³n de un modelo basado en simetrÃ­as ya que la invariancia gauge prohÃ­be tÃ©rminos de masa para los bosones gauge. Por ello, fue necesario desarrollar un mecanismo que dotase de masa a estas partÃ­culas. La soluciÃ³n a este problema llegÃ³ de la mano de Robert Brout, Francois Englert, Gerald Guralnik, Carl Richard Hagen, Peter Higgs y Tom Kibble (en estricto orden alfabÃ©tico) \cite{PhysRevLett.13.321,PhysRev.145.1156,PhysRevLett.13.585,PhysRev.155.1554}.

La idea de \nuria{este mecanismo} quitar:(de Higgs) se basa en la \textit{ruptura espontÃ¡nea de la simetrÃ­a}\footnote{Del inglÃ©s \textit{Spontaneous Symmetry Breaking}.} (SSB) y consiste en agregar a la teorÃ­a un campo complejo escalar doblete de $SU(2)_L$:
\be
\Phi = \left( \begin{array}{c}
\Phi^+  \\
\Phi^0  \end{array} \right) = 
\left( \begin{array}{c}
\Phi^+  \\
\dfrac{1}{\sqrt{2}}(v + \phi_1 + i\phi_2)  \end{array} \right) \, .
\ee
Este peculiar campo presenta lo que se conoce como \textit{valor esperado de vacÃ­o}\footnote{Del inglÃ©s de \textit{Vacuum Expectation Value}.} (VEV) no nulo en su componente neutra, produciendo de este modo una ruptura de la simetrÃ­a electrodÃ©bil (que no es una simetrÃ­a exacta del vacÃ­o) y dando como resultado la simetrÃ­a electromagnÃ©tica\footnote{La abreviaciÃ³n QED viene de \textit{Quantum Electrodynamics} \cite{10.1143/PTP.1.27,10.1143/ptp/2.3.101,10.1143/ptp/3.2.101,PhysRev.74.224,PhysRev.74.1439,Feynman:1948ur,Feynman:1949zx}, nombre que recibe la teorÃ­a gauge que describe la interacciÃ³n electromagnÃ©tica.},
\be
SU(2)_L\times U(1)_Y \longrightarrow U(1)_{QED}.
\ee

\miguel{Durante la SSB, tanto la parte cargada del doblete como la parte imaginaria de la componente neutra son absorbidos como grados de libertad longitudinales por los bosones gauge de la teorÃ­a, los cuales pasan a comportarse como bosones masivos.} Por otro lado, la parte real del campo cargado, $\phi_1$, se queda presente en el espectro de partÃ­culas del Modelo EstÃ¡ndar como una partÃ­cula de spin 0, el popular \textit{bosÃ³n de Higgs}, que fue detectado en 2012 por los experimentos ATLAS \cite{Aad_2012} y CMS del LHC \cite{Chatrchyan_2012}, confirmando el modelo.

\nuria{Las representaciones de los fermiones del Modelo Estándar bajo el grupo $SU(2)_L\times U(1)_Y$ no presentan simetría quiral, necesaria para que los correspondientes  tÃ©rminos de masa puedan aparecer en el lagrangiano del modelo.}
 (El grupo $SU(2)_L\times U(1)_Y$ no presenta simetrÃ­a quiral, necesaria para escribir los tÃ©rminos de masa de los fermiones en el lagrangiano del modelo.) No obstante, el mecanismo de Higgs soluciona este problema ya que \nuria{ bajo el grupo $U(1)_{\text{QED}}$ si que presentan dicha simetrÃ­a}. En consecuencia, despuÃ©s de la SSB, el VEV del campo de Higgs permite la formaciÃ³n de los tÃ©rminos de masa para estas partÃ­culas.

Para una exposiciÃ³n detallada y completa del Modelo EstÃ¡ndar en espaÃ±ol ver Ref.~\cite{gelmini2014el}.

\section{La Necesidad de la Materia Oscura}

\nuria{estos párrafos estan repetidos, sobra 1}
\miguel{Como ya hemos comentado, el Modelo Estandar de partÃ­culas solo puede explicar un porcentaje pequeÃ±o de la materia que nos rodea, conocida como \textit{bariÃ³nica}. El resto de materia que puebla el Universo recibe el nombre de Materia Oscura\footnote{Su nombre se debe a que no emite ni refleja ningÃºn tipo de luz.}}. A pesar de que este exÃ³tico tipo de materia es un (fuerte) \nuria{activo} campo de estudio en la actualidad, los primeros indicadores de su existencia son ya casi centenarios \cite{Zwicky:1933gu}. No obstante, las primeras pruebas sÃ³lidas se las debemos a los trabajos de Vera Cooper Rubin, Kent Ford y Ken Freeman, llevados a cabo allÃ¡ por los aÃ±os 60 \cite{1970ApJ...159..379R,1970ApJ...160..811F}.

A pesar de los grandes exitos cosechados por el Modelo EstÃ¡ndar, hoy sabemos que no es, ni mucho menos, el final de la fÃ­sica de partÃ­culas. La que aparentemente era la conclusiÃ³n de la fÃ­sica de altas energÃ­as, Ãºnicamente es capaz de explicar un porcentaje muy pequeÃ±o de la materia del Universo, el resto sigue siendo un misterio. Las observaciones astrofÃ­sicas y cosmolÃ³gicas mÃ¡s recientes \cite{Aghanim:2018eyx} nos indican que el $26\%$ del contenido de energÃ­a del Universo es un nuevo tipo de materia, conocida como Materia Oscura\footnote{Su nombre se debe a que no emite ni refleja ningÃºn tipo de luz.}. A pesar de que este exÃ³tico tipo de materia es un fuerte campo de estudio en la actualidad, los primeros indicadores de su existencia son ya casi centenarios \cite{Zwicky:1933gu}. No obstante, las primeras pruebas sÃ³lidas se las debemos a los trabajos de Vera Cooper Rubin, Kent Ford y Ken Freeman, llevados a cabo allÃ¡ por los aÃ±os 60 \cite{1970ApJ...159..379R,1970ApJ...160..811F}.

\subsection{Evidencias de la Existencia de Materia Oscura}
\label{sec:res:evidencias}

La evidencia mÃ¡s clara que tenemos a dÃ­a de hoy de la existencia de la Materia Oscura son las curvas de rotaciÃ³n de las galaxias. El contenido en masa de una galaxia puede medirse en base a su luminosidad, mediante tÃ©cnicas astrofÃ­sicas. De este modo, tenemos una clara idea de cuanta materia bariÃ³nica hay en una determinada galaxia y como estÃ¡ distribuida dentro de ella. Conocida la masa de la galaxia, la velocidad de rotaciÃ³n de un objeto situado a una distancia $R$ del centro de la misma puede determinarse a partir de las leyes de Kepler\footnote{$v = \sqrt{MG/R}$, donde $M$ es la masa contenida en la esfera de radio $R$ y $G$ la constante de gravitaciÃ³n universal.}. De acuerdo con esto, la distribuciÃ³n de materia bariÃ³nica observada nos indica que la velocidad de rotaciÃ³n deberÃ­a disminuir conforme nos acercamos al borde galÃ¡ctico. Sin embargo, medidas directas sobre la velocidad de rotaciÃ³n indican lo contrario: en la mayorÃ­a de los casos esta velocidad de rotaciÃ³n permanece constante.

Las curvas de rotaciÃ³n de las galaxias son la evidencia mÃ¡s famosa de la existencia de este exÃ³tico tipo de materia, pero no la Ãºnica. La teorÃ­a de la Relatividad General predice que el campo gravitatorio producido por un gran cÃºmulo de materia es capaz de desviar los rayos de luz, el conocido como efecto \textit{lente gravitatoria}. De este modo, puede utilizarse la luz procedente de galaxias lejanas para, mediante ciertos estudios sobre la trayectoria de los haces de luz, determinar la cantidad de materia que hay en los cÃºmulos de galaxias situados en su trayectoria. Este anÃ¡lisis confirma la presencia de Materia Oscura en la mayorÃ­a de cÃºmulos de galaxias estudiados.

Aparte de las evidencias astrofÃ­sicas, hay tambi\'en  evidencias cosmolÃ³gicas que confirman la existencia de la Materia Oscura. En la Sec.~\ref{sec:evidences} se ha realizado una breve descripciÃ³n de todas ellas.

\subsection{CaracterÃ­sticas Fundamentales}

A pesar de las evidencias de su existencia, a dÃ­a de hoy aÃºn no se ha realizado ninguna observaciÃ³n directa de la Materia Oscura. No obstante, podemos inferir mucho acerca de su naturaleza:
\begin{itemize}
\item La Materia Oscura debe ser no bariÃ³nica: algunos candidatos bariÃ³nicos han sido propuestos a lo largo de los aÃ±os, como es el caso de los MACHOs\footnote{Del inglÃ©s \textit{Massive Compact Halo Objects}.} \cite{1986ApJ...304....1P}. No obstante, los lÃ­mites sobre esta clase de modelos son tan fuertes en la actualidad que estÃ¡n prÃ¡cticamente descartados en su totalidad.
\item Debe ser \textit{frÃ­a} o \textit{cÃ¡lida}: segÃºn la distancia recorrida, como consecuencia de movimientos aleatorios, por las partÃ­culas de Materia Oscura en el Universo primigenio, podemos catalogarla en tres grandes grupos: \textit{calinte}, \textit{cÃ¡lida} y \textit{frÃ­a}. Si la distancia recorrida es mayor, igual o menor que el tamaÃ±o de una protogalaxia \miguel{(unos 100 aÃ±os luz)}, la Materia Oscura serÃ¡ caliente, cÃ¡lida o frÃ­a, respectivamente. En la actualidad se han realizado numerosas simulaciones numÃ©ricas de la evoluciÃ³n del Universo con diferentes tipos de materia. Si la Materia Oscura fuese caliente, de acuerdo con estas simulaciones, el Universo tendrÃ­a un aspecto muy diferente al que conocemos hoy en dÃ­a \cite{primack2001happened}.
\item Debe colisionar muy dÃ©bilmente consigo misma: el motivo de esto es que recientes observaciones astrofÃ­sicas, tales como las realizadas sobre el conocido como \textit{cÃºmulo bala}\footnote{Este curioso cÃºmulo es el resultado de dos cÃºmulos actualmente en colisiÃ³n. En Ã©l se observa un efecto muy exÃ³tico, el centro de masas del cÃºmulo resultante se encuentra desplazado. Esta caracterÃ­stica solo puede ser explicada mediante la existencia de grandes cantidades de Materia Oscura en su composiciÃ³n. La alternativa requerirÃ­a una modificaciÃ³n de las leyes mÃ¡s fundamentales de la dinÃ¡mica relativista.}, imponen restricciones a la autointeracciÃ³n de la Materia Oscura \cite{Dave_2001,Feng_2009,Agrawal_2017,Randall_2008,Kahlhoefer_2013}:
\be
\sigma/m \lesssim 10^{-24} \, \text{cm}^2/\text{GeV} .
\ee
\item DÃ©bilmente interactiva con la materia bariÃ³nica: \miguel{aparte de la interacciÃ³n gravitatoria, la Ãºnica interacciÃ³n posible que podrÃ­a llegar a tener la Materia Oscura es la dÃ©bil. Respecto a lo que al electromagnetismo se refiere, las diversas implicaciones que supone la existencia de Materia Oscura cargada han sido profundamente estudiadas en la literatura \cite{DERUJULA1990173}, descartando prÃ¡cticamente esta opciÃ³n por motivos experimentales\footnote{En la actualidad las tÃ©cnicas de detecciÃ³n de partÃ­culas cargadas son tan avanzadas que de existir la Materia Oscura elÃ©ctricamente cargada, esta ya deberÃ­a haber sido observada.} \cite{Taoso:2007qk}.
Por otro lado, de existir la Materia Oscura fuertemente interactiva\footnote{Fuertemente en el sentido de interacciÃ³n a travÃ©s de la interacciÃ³n fuerte.}, Ã©sta dejarÃ­a huella incluso en el flujo de calor terrestre \cite{Mack:2007xj}. Las fuertes implicaciones de este tipo de candidatos hacen que esten excluidos casi en su totalidad.}
\item Debe ser estable: la Materia Oscura que observamos hoy en dÃ­a en el Universo es prÃ¡cticamente un fÃ³sil tÃ©rmico: es el remanente de la que la que componÃ­a el Universo primigenio. La Ãºnica forma de que ese remanente haya sobrevivido hasta nuestros dÃ­as es que la Materia Oscura sea estable o, en su defecto, que su vida media sea mayor que la edad del Universo.
\end{itemize}

En la Sec.~\ref{sec:Properties} se ha realizado un estudio mucho mÃ¡s profundo de todas estas propiedades.

\subsection{Candidatos Estudiados}

Hasta el momento hemos hablado de las diferentes evidencias y caracterÃ­sticas de la Materia Oscura. Pero Â¿cuÃ¡l es su naturaleza? En el escenario cientÃ­fico actual se han propuesto muchos candidatos a Materia Oscura, desde todo tipo de partÃ­culas con interacciones parecidas a las que ya conocemos, hasta candidatos altamente exÃ³ticos como agujeros negros primigenios \cite{10.1093/mnras/168.2.399,1975ApJ...201....1C,10.1093/mnras/152.1.75}. Todo esto ha sido detallado en la Sec.~\ref{sec:candidates}. En este resumen Ãºnicamente hablaremos sobre los dos candidatos estudiados en esta Tesis: las partÃ­culas WIMP \cite{PhysRevLett.39.165} y las FIMP \cite{Hall:2009bx}.

\subsubsection{Materia Oscura tipo WIMP}

Las partÃ­culas WIMP\footnote{Su nombre deriva del inglÃ©s \textit{Weakly Interactive Massive Particles}, es decir, partÃ­culas masivas dÃ©bilmente interactivas.} son partÃ­culas con masas tÃ­picamente desde el GeV hasta varios TeV. Este candidato se basa en la suposiciÃ³n de que las partÃ­culas de Materia Oscura se encontraban en equilibrio tÃ©rmico con el resto de partÃ­culas del Modelo EstÃ¡ndar en el Universo primigenio. La abundancia que observamos en la actualidad serÃ­a pues el resultado de un proceso denominado \textit{freeze-out}.

Para entender bien el concepto de \textit{freeze-out}, debemos remontarnos a los primeros instantes del Universo, justo despuÃ©s del Big Bang. En aquella Ã©poca, los Ã¡tomos no existÃ­an, las diferentes partÃ­culas que poblaban el Universo se encontraban en un equilibrio continuo de aniquilaciÃ³n/producciÃ³n, formando un plasma de altÃ­sima temperatura. Poco a poco, el Universo fue expandiÃ©ndose, enfriando dicho plasma. El enfriamiento del Universo provocÃ³ que algunos de los procesos que mantenÃ­an este equilibrio dejasen de tener lugar, desacoplando de este modo las diferentes especies de partÃ­culas de este \textit{caldo} primigenio.

Cuando la temperatura del Universo fue demasiado baja como para que la creaciÃ³n de partÃ­culas de Materia Oscura fuese posible, estÃ¡ se desacoplÃ³ del \textit{caldo} primigenio. Como consecuencia, la abundancia de estas partÃ­culas comenzÃ³ a disminuir, hasta que fue tan pequeÃ±a que la probabilidad de que dos partÃ­culas de Materia Oscura se encontrasen y se aniquilasen se volviÃ³ prÃ¡cticamente nula. A dicha temperatura, conocida como temperatura de \textit{freeze-out}, la abundancia de Materia Oscura superviviente se convirtiÃ³ en un leve remanente, un mero fÃ³sil tÃ©rmico, que ha llegado hasta nuestros dÃ­as.

Este candidato a Materia Oscura ha gozado de gran acogida por los fÃ­sicos teÃ³ricos desde que fuese propuesto alla por los aÃ±os 70. El motivo de tal popularidad es que en el rango de masas mencionado, curiosamente, para reproducir la abundancia de Materia Oscura actual, se necesita que la interacciÃ³n entre Ã©sta y las partÃ­culas del Modelo EstÃ¡ndar sea justo del orden de la interacciÃ³n electrodÃ©bil. Hecho, cuanto menos sorprendente, que se conoce como \textit{Milagro WIMP}. En este rango de masas la secciÃ³n eficaz necesaria para conseguir dicha abundancia es prÃ¡cticamente independiente del valor de la masa de la partÃ­cula WIMP,
\be
\langle \sigma v \rangle \backsimeq 2 \times 10^{-26}\, \text{cm}^3/\text{s} \backsim 1 \, \text{pb} \, .
\ee
Los detalles matemÃ¡ticos y tÃ©cnicos de este candidato a Materia Oscura se encuentran explicados en la Sec.~\ref{Sec:freezeout}.

\subsubsection{Materia Oscura tipo FIMP}

Complementariamente al caso WIMP, existe la Materia Oscura tipo FIMP\footnote{Nombre que deriva del ingles \textit{Feebly Interactive Massive Particle}.} la cual jamÃ¡s llegÃ³ al equilibrio tÃ©rmico con el resto de partÃ­culas del Modelo EstÃ¡ndar. En este escenario la Materia Oscura fue producida por diversos procesos durante la Ã©poca de enfriamiento del Universo, despuÃ©s del Big Bang, siendo nula en el origen de los tiempos. Cuando la temperatura del Universo fue suficientemente baja, esta producciÃ³n se congelÃ³, dejando un remanente que ha llegado hasta nuestros dÃ­as. Este mecanismo de producciÃ³n recibe el nombre de \textit{freeze-in}\footnote{El mecanismo de producciÃ³n fue propuesto en Ref.~\cite{Chung:1998rq}. Aunque en aquella Ã©poca ni el mecanismo se conocÃ­a por dicho nombre, ni el candidato como FIMP.} y estÃ¡ detallado en la Sec.~\ref{Sec:freezein}.

\miguel{La Materia Oscura FIMP no ha llegado a alcanzar la popularidad de la Materia Oscura tipo WIMP. Hay varios motivos para ello pero el principal es que debido a su baja intensidad de interacciÃ³n es muy dificil buscar pruebas experimentales de su existencia.}

\section{DetecciÃ³n de Materia Oscura}

Como hemos comentado en la Sec.~\ref{sec:evidences}, y resumido en Sec.~\ref{sec:res:evidencias}, tenemos muchas evidencias de la existencia de a Materia Oscura. No obstante, no se ha conseguido realizar ninguna observaciÃ³n directa de estas elusivas partÃ­culas\footnote{Existe una llamativa excepciÃ³n: el experimento DAMA/Libra ha medido variaciones en la modulaciÃ³n solar que pueden ser interpretadas como Materia Oscura \cite{Bernabei:2008yi,Bernabei:2010mq}. No obstante, esta seÃ±al no estÃ¡ libre de controversia entre la comunidad cientÃ­fica ya que ningÃºn otro experimento ha reportado absolutamente nada en el rango de masas en el que DAMA/Libra mide dicha seÃ±al.}. A pesar de esto, las tÃ©cnicas de detecciÃ³n de Materia Oscura han avanzado mucho en los Ãºltimos aÃ±os, poniendo cotas cada vez mÃ¡s restrictivas a la existencia de estas partÃ­culas aparentemente invisibles.
Dentro del gran abanico de experimentos de detecciÃ³n, estos pueden clasificarse en dos grandes grupos: la \textit{DetecciÃ³n Directa}\footnote{Del ingles \textit{Direct Detection.}} DD y la \textit{Deteccion Indirecta}\footnote{Del ingles \textit{Indirect Detection.}} ID.

\subsection{DetecciÃ³n Directa}

La idea de la DetecciÃ³n Directa (cuyos detalles tÃ©cnicos se discuten en profundidad en la Sec.~\ref{Sec:DD}) fue propuesta por primera vez por Mark Goodman y Edward Witten \cite{Goodman:1984dc}. Como la Materia Oscura no presenta cargas elÃ©ctricas, es imposible detectarla mediante tÃ©cnicas electromagnÃ©ticas. No obstante, la existencia de colisiones entre la DM y los nÃºcleos atÃ³micos abre una puerta para su observaciÃ³n directa. 

En general, esta clase de detecciones se realizan en experimentos ubicados bajo tierra. Ejemplos notables son Xenon1T \cite{PhysRevLett.121.111302} o LUX \cite{Akerib:2016vxi}, los cuales estÃ¡n compuestos por grandes cantidades de XenÃ³n. La colisiÃ³n de la Materia Oscura con los Ã¡tomos de XenÃ³n producirÃ­a una excitaciÃ³n de estos Ãºltimos, que finalmente se traducirÃ­a en la emisiÃ³n de un fotÃ³n. Hasta el momento, no se ha realizado ninguna detecciÃ³n en dichos experimentos, lo cual pone fuertes lÃ­mites sobre los modelos de Materia Oscura, haciendo que los escenarios mÃ¡s simples y \textit{naturales} estÃ©n prÃ¡cticamente descartados.

\begin{figure}[htbp]
\centering
\includegraphics[width=130mm]{figures/direct_detection_bounds.pdf}
\caption[Estatus actual de los experimentos de detecciÃ³n directa.]{\it LÃ­mites actuales a la secciÃ³n eficaz de interacciÃ³n de Materia Oscura con nucleones. La regiÃ³n verde estÃ¡ excluida por los experimentos de DetecciÃ³n Directa con un 90\% de intervalo de confianza. Las dos zonas rojas muestran las regiones en las que DAMA/LIBRA afirma haber observado Materia Oscura. La zona amarilla representa el \textit{suelo  de neutrinos} \cite{Billard:2013qya}.}
 \label{fig:direct_detection_bounds_resumen}
\end{figure}

Uno puede hacerse una idea del panorama actual de estos experimentos mirando la Fig.~\ref{fig:direct_detection_bounds_resumen}. En ella, la zona verde muestra los valores de la secciÃ³n eficaz de DetecciÃ³n Directa, como funciÃ³n de la masa de la Materia Oscura, que ya han sido descartados por los experimentos. Por otro lado, para hacernos una idea de magnitud de la zona ya eliminada, podemos mirar lo cerca que se encuentra de ella la regiÃ³n amarilla. Esta regiÃ³n muestra lo que se conoce como \textit{suelo de neutrinos}\footnote{En ingles conocido como \textit{neutrino floor}.} \cite{Billard:2013qya} y representa \miguel{la secciÃ³n eficaz} para la que los experimentos de detecciÃ³n comenzarÃ¡n a observar colisiones producidas por los neutrinos. Realizar exclusiones mediante experimentos de DetecciÃ³n Directa en esta regiÃ³n es complicado, puesto que la seÃ±al de ambos tipos de colisiÃ³n es indistinta. Las dos regiones rojas muestran las observaciones de DAMA/LIBRA en zonas totalmente excluidas por el resto de experimentos.

\subsection{DetecciÃ³n Indirecta}

La observaciÃ³n directa de las colisiones de las partÃ­culas de Materia Oscura con los nÃºcleos atÃ³micos no es la Ãºnica tÃ©cnica para detectarla. Diferentes experimentos astronÃ³micos llevan aÃ±os intentando observar los posibles productos de las aniquilaciones de las partÃ­culas de Materia Oscura en los rayos cÃ³smicos que nos llegan a la Tierra. Es posible distinguir entre tres tipos de flujos de partÃ­culas: fotones, neutrinos y partÃ­culas cargadas (como electrones, positrones, etc).

En general, de los diferentes flujos de partÃ­culas que llegan a la Tierra, los resultados mÃ¡s prometedores (en lo que a Materia Oscura se refiere) vienen de los fotones. Desde 2008 la colaboraciÃ³n Fermi-LAT analiza el flujo de fotones procedente de diferentes \textit{galaxias enanas} \cite{Fermi-LAT:2016uux,Ackermann:2015zua}. Hasta el momento el estudio se restringe a 15 ejemplares y por el momento los resultados no muestran ningÃºn exceso en el flujo analizado que no pueda ser explicado por el Modelo EstÃ¡ndar de partÃ­culas. Esto pone cotas a modelos de nueva fÃ­sica en los cuales la Materia Oscura pueda aniquilarse a partÃ­culas que finalmente se desintegren en fotones, generalmente en el rango de masas $m_{\text{DM}} \in (0.5,500) $ GeV. No obstante, desde 2009 el mismo experimento ha estado reportando un exceso inexplicable de fotones procedente del centro galÃ¡ctico\footnote{Popularmente conocido como \textit{Galactic Center $\gamma$-ray excess} (GCE) \cite{Goodenough:2009gk, Vitale:2009hr, Hooper:2010mq, Gordon:2013vta, Hooper:2011ti, Daylan:2014rsa, 2011PhLB..705..165B, Calore:2014xka, Abazajian:2014fta,Zhou:2014lva}.}. Aunque su origen aÃºn es desconocido, este exceso, que se observa a una energÃ­a $\sim 3$ GeV, puede ser explicado por diferentes modelos de Materia Oscura.

Por otro lado, las seÃ±ales procedentes de flujos de antipartÃ­culas cargadas acotan de una forma mucho menos restrictiva los modelos de Materia Oscura. El problema con esta clase de flujos es su propagaciÃ³n desde el punto en el que son generados hasta la Tierra (donde finalmente los detectamos). Hoy en dÃ­a existen diversos modelos para ello, pero su precisiÃ³n aÃºn tiene que ser perfeccionada para que los lÃ­mites impuestos por esta clase de flujos sean realmente restrictivos.

En la Sec.~\ref{Sec:ID} se ha realizado un anÃ¡lisis exhaustivo de la DetecciÃ³n Indirecta de Materia Oscura.

\section{Dimensiones Extra}

\miguel{De entre las cuatro fuerzas fundamentales de la naturaleza, no cabe ninguna duda de que la gravedad es la mÃ¡s complicada de entender a nivel cuÃ¡ntico. A pesar de los muchos esfuerzos por parte de la comunidad cientÃ­fica, aÃºn no tenemos una teorÃ­a cuÃ¡ntica para describirla.
Por otro lado, la gravedad es la mÃ¡s dÃ©bil de las interacciones fundamentales. Tal es el caso, que de existir nueva fÃ­sica a la escala gravitatoria, el Modelo EstÃ¡ndar se enfrentarÃ­a a un serio problema}: las correcciones a la masa del bosÃ³n de Higgs son muy sensibles a la escala de la nueva fÃ­sica. Teniendo en cuenta la diferencia entre la escala de Planck\footnote{La escala de la interacciÃ³n gravitatoria.} y la escala electrodÃ©bil, de aparecer nueva fÃ­sica a la escala gravitatoria las correcciones a la masa del Higgs serÃ­an enormes, (entrando en serias inconsistencias matemÃ¡ticas) \nuria{requiriendo cancelaciones ajustadas entre distintos órdenes de teoría de perturbaciones para explicar el valor medido}. A este fenÃ³meno se le conoce como \textit{problema de la jerarquÃ­a} (para un analisis mÃ¡s detallado del problema mirar la Sec.~\ref{sec:hierarchyproblem}). Entre las diversas propuestas que se han realizado para intentar resolver este problema se encuentran las dimensiones extra.

\subsection{Dimensiones Extra \textit{Grandes} (LED)}

El primer modelo de dimensiones extra que se propuso para dar soluciÃ³n al problema de la jerarquÃ­a fue \textit{Large Extra-Dimensions} (LED) \cite{ArkaniHamed:1998rs}. En este escenario se asume que las nuevas dimensiones tienen una forma similar a las tres espaciales ya conocidas, es decir, presentarÃ­an un aspecto plano. De acuerdo con el modelo LED, el tamaÃ±o de estas nuevas dimensiones serÃ­a finito o, en otras palabras, estarÃ­an compactificadas. Por otro lado, mientras que la gravedad se propaga libremente por el espacio 5-dimensional, el resto de campos del Modelo EstÃ¡ndar se encuentran confinados en unas hipersuperficies 4-dimensionales denominadas \textit{branas}. Este hecho hace que la gravedad se diluya a travÃ©s de las dimensiones extra, haciendo que en la brana (donde nosotros vivimos confinados) su intensidad parezca anÃ³malamente dÃ©bil. De este modo, la escala de la gravitaciÃ³n, que para nosotros es $M_\text{P} = 1.22 \times 10^{19}$ GeV, en el espacio extra-dimensional completo serÃ­a $M_D$. \miguel{Ambas escalas estÃ¡n relacionadas a travÃ©s del radio de compactificaciÃ³n de las dimensiones extra ($r_c$):
\be
M_\text{P}^2 = M_{D}^{D-2} (2\pi r_c)^D.
\ee 
}

Para el caso particular de 5 dimensiones, el espacio-tiempo queda definido en este modelo por la mÃ©trica:
\be
ds^2 = \eta_{\mu \nu}dx^\mu dx^\nu + r_c^2dy^2,
\ee
Donde la dimensiÃ³n extra estÃ¡ representada por $y$. Este parÃ¡metro puede escogerse de manera que $M_5 \backsim \text{TeV}$, resolviendo asÃ­ el problema de la jerarquÃ­a.
No obstante, si imponemos esta condiciÃ³n, el modelo LED 5-dimensional estÃ¡ excluido totalmente a dÃ­a de hoy: agregar una Ãºnica dimensiÃ³n extra en LED predice correcciones de la ley de la gravitaciÃ³n universal que podrÃ­an observarse en distancias parecidas al tamaÃ±o del Sistema Solar. \miguel{No obstante, aunque el modelo estÃ© excluido para una Ãºnica dimensiÃ³n extra, con dos o mÃ¡s dimensiones es posible resolver el problema de la jerarquÃ­a sin entrar en contradicciones con la ley de la gravitaciÃ³n universal.}

\subsection{Dimensiones Extra Deformadas: Modelo de Randall-Sundrum}

A pesar de que los modelos LED presentan diversos problemas, pusieron la semilla para modelos futuros muy interesantes. El caso mÃ¡s popular es el modelo propuesto por Lisa Randall y Raman Sundrum a finales de los aÃ±os 90, conocido como \textit{dimensiones extra deformadas} o \textit{modelo de Randall-Sundrum} (RS) \cite{Randall:1999ee}. En dicho modelo, las nuevas dimensiones presentan curvatura, a diferencia de LED, donde eran planas. En el modelo original de RS el espacio extra-dimensional estÃ¡ delimitado por dos branas. Todos los campos de materia viven atrapados en una de ellas (brana \textit{infrarroja} (IR), tambiÃ©n llamada brana del TeV), mientras que la otra brana se encuentra vacÃ­a (brana \textit{ultravioleta} (UV) o de Planck). Por otro lado, la gravedad se propaga libremente por el espacio extra-dimensional (comÃºnmente conocido como \textit{bulk}). La geometrÃ­a del modelo hace que los diferentes parÃ¡metros fundamentales con dimensiÃ³n de masa sufran un proceso de deformaciÃ³n exponencial a lo largo del bulk, resolviendo asÃ­ el problema de la jerarquÃ­a.

Concretamente, para el caso 5-dimensional (una Ãºnica dimensiÃ³n extra), la mÃ©trica que definirÃ­a este espacio tiempo vendrÃ­a dada por
\be
ds^2 = e^{-2  kR|y|}\eta_{\mu \nu} dx^\mu dx^\nu - r_c^2 dy \, ,
\label{RS_metric_resumen}
\ee
Donde $k$ es la curvatura a lo largo de la dimensiÃ³n extra y $r_c$ su radio de compactificaciÃ³n. El factor exponencial que multiplica la parte 4-dimensional de la mÃ©trica recibe el nombre de factor de deformaciÃ³n.
$M_5$ y $M_\text{P}$ quedarÃ­an entonces relacionados mediante los dos parÃ¡metros libres de la teorÃ­a:
\be
\bar{M_\text{P}}^2 = \frac{M_5}{k} \left( 1 - e^{-2 k \pi r_c} \right) \, .
\ee
Vemos que hay una clara diferencia con el modelo LED: en RS $M_5\backsimeq M_\text{P}$. Sin embargo, la modificaciÃ³n que sufren los parÃ¡metros medidos en la brana IR, debido a la presencia del factor de deformaciÃ³n, resuelve el problema de la jerarquÃ­a para $k\,r_c \backsim 10 $.

\miguel{En RS la gravedad puede describirse a travÃ©s del intercambio de gravitones no masivos 5-dimensionales, los cuales surgen de perturbaciones sobre la componente 4-dimensional de la mÃ©trica
\be
G^{(4)}_{\mu \nu} = e^{-2kr_c|y|} (\eta_{\mu \nu} + 2M_5^{-2/3} h_{\mu \nu}) \, .
\label{perturbacion_4dim}
\ee
La proyecciÃ³n de este campo 5-dimensional sobre las branas es equivalente a una torre de gravitones 4-dimensionales masivos, comÃºnmente conocidos como modos de Kaluza-Klein (KK). La escala efectiva de la interacciÃ³n de estos gravitones 4-dimensionales con los campos confinados en la brana IR viene dada por
\be
\Lambda \equiv \bar{M_\text{P}} e^{-k \pi r_c} \, .
\ee
Por otro lado, cada gravitÃ³n de esta torre de partÃ­culas tiene una masa diferente que dependerÃ¡ de los parÃ¡metros libres ($k,r_c$) del modelo y de su respectivo orden dentro de la torre. No obstante, establecida la masa del primer gravitÃ³n $m_1$, la masa del resto de gravitones queda totalmente fijada. La fenomenologÃ­a de los modelos de RS puede ser descrita mediante los parÃ¡metros ($\Lambda,m_1$), en lugar de ($k,r_c$). Este hecho puede ser muy Ãºtil debido a su relaciÃ³n con observables fenomenolÃ³gicos.}

\miguel{El modelo asume que la distancia entre las branas estÃ¡ fijada, pero no aporta ningÃºn mecanismo para estabilizar este parÃ¡metro dinÃ¡micamente. La soluciÃ³n a este problema fue propuesta por Walter D. Goldberger y Mark B. Wise \cite{Goldberger:1999wh,Goldberger:1999uk}. Este mecanismo utiliza un nuevo campo escalar que se propaga libremente por el \textit{bulk}, \nuria{sometido a} unos potenciales localizados en las branas. 
Por otro lado, el nuevo campo escalar se mezcla con el ya presente en el \textit{bulk}, el graviescalar $G_{55}^{(5)}$ (el cual emerge de las perturbaciones sobre la parte 5-dimensional de la mÃ©trica). Al campo resultante de esta mezcla se le conoce como radiÃ³n. \nuria{Los mÃ­nimos de los potenciales en la brana IR y UV son diferentes, lo que genera un valor esperado de vacÃ­o para (este nuevo campo escalar) el radión. El tamaÃ±o de la quinta dimensiÃ³n ($r_c$) estÃ¡ entonces relacionado con este valor esperado de vacio.La masa del radión no estÃ¡ determianda por los parámetros del modelo original, y representa un nuevo grado de libertad.}

El modelo de RS ha gozado de gran popularidad desde que fue propuesto a finales de los 90's. La literatura sobre modelos de fÃ­sica mÃ¡s allÃ¡ del Modelo EstÃ¡ndar desarrollados en este escenario es inmensa. En la Sec.~\ref{sc:warped} se ha realizado un anÃ¡lisis de los detalles tÃ©cnicos del modelo.  

\subsection{Dimensiones extra tipo \textit{Clockwork/Linear Dilaton}}

\miguel{Durante casi dos décadas lo modelos de RS fueron los Ãºnicos que resolvían el problema de la jerarquÃ­a mediante la introducciÃ³n de dimensiones con curvatura. No obstante, en 2016 Gian Giudice y Matthew McCullough propusieron un nuevo modelo de dimensiones extra curvadas. Este nuevo modelo, propuesto en Ref.~\cite{Giudice:2016yja} y cuya fenomenologÃ­a fue estudiada en Ref.~\cite{Giudice:2017fmj}, se conoce con el nombre de \textit{Clockwork/Linear Dilaton} (CW/LD).}

\miguel{Dicho modelo, que fue encontrado como lÃ­mite continuo de los modelos \textit{Clockwork} discretos, puede caracterizarse a traves de la mÃ©trica:
\be
\label{eq:5dmetric_resumen}
ds^2 = e^{4/3 k r_c |y|} \left ( \eta_{\mu \nu} dx^{\mu}dx^{\nu} - r_c^2 \, dy^2 \right ) \, ,
\ee
donde $k$ y $r_c$ representan la curvatura y el radio de compactificaciÃ³n de la quinta dimensiÃ³n, respectivamente. Para determinados valores de los parÃ¡metros libres, el modelo es capaz de resolver el problema de la jerarquÃ­a.}

El modelo CW/LD guarda ciertas similitudes con RS. En ambos casos el espacio 5-dimensional estÃ¡ delimitado por las branas IR y UV. El caso mÃ­nimo implica tener todo el Modelos EstÃ¡ndar confinado en la brana IR, mientras que la gravedad se propaga libremente por el bulk 5-dimensional. Sin embargo, hay diferencias notables con RS. En primer lugar, la relaciÃ³n entre $M_5$ y $M_\text{P}$ en CW/LD viene dada por
\be
M_{\text{P}}^2 = \frac{M_5^3}{k} \left ( e^{2 \pi r_c}  - 1 \right ) \, ,
\ee 
pudiendo ser esta del orden del TeV (al igual que en el caso LED). Por otro lado, el acoplamiento de \miguel{los gravitones de KK} \nuria{los gravitones de KK suena mal, jajaja, mejor los modos de Kaluza-Klein de los gravitones}a las partÃ­culas localizadas en la brana es diferente para cada gravitÃ³n:
\be
\dfrac{1}{\Lambda_{n}} =  \dfrac{1}{\sqrt{M_5^3 \pi r_c}}  \left ( 1 + \dfrac{k^2 r_c^2}{n^2} \right )^{-1/2} 
=  \dfrac{1}{\sqrt{M_5^3 \pi r_c}} \left ( 1 - \dfrac{k^2}{m_n^2} \right )^{1/2}  \,  .
\ee
Este hecho hace que describir la fenomenologÃ­a en base a $\Lambda_n$ no sea tan Ãºtil como en RS. Otra diferencia notable es que hay una relaciÃ³n muy interesante entre el valor de la curvatura $k$ y la masa del primer gravitÃ³n $m_1$, haciendo que ambos parÃ¡metros sean prÃ¡cticamente idÃ©nticos.

\miguel{En el caso CW/LD, \nuria{el modelo original ya incluye un campo escalar que estabiliza el tamaÃ±o de la quinta dimension, el campo de dilataciÃ³n (\textit{dilaton}), $S = 2 k r_c |y|$, de la mÃ©trica.} (puede estabilizarse sin necesidad de introducir ningÃºn nuevo campo). La existencia de unos potenciales en las branas IR y UV  permite fijar la posiciÃ³n de las branas de un modo similar a como se hacÃ­a en RS.}

\section{MetodologÃ­a Utilizada}

Antes de ponernos a hablar sobre los cuatro proyectos que conforman la presente Tesis, es necesario comentar las diferentes tÃ©cnicas (tanto a nivel analÃ­tico como numÃ©rico) utilizadas en el desarrollo de los mismos. 

A nivel analÃ­tico, la complejidad de los problemas estudiados ha requerido un profundo conocimiento de la teorÃ­a cuÃ¡ntica de campos. Se han utilizado los desarrollos perturbativos de dicha teorÃ­a para obtener las diferentes probabilidades de interacciÃ³n utilizadas posteriormente en los estudios fenomenolÃ³gicos. Los modelos aquÃ­ estudiados asumen Materia Oscura tipo WIMP y FIMP. En ambos casos, la evoluciÃ³n de la abundancia de Materia Oscura a lo largo de la historia tÃ©rmica del Universo requiere resolver la EcuaciÃ³n de Boltzman, que determina la evoluciÃ³n de sistemas fuera del equilibrio tÃ©rmico. Por otro lado, se ha trabajado con dos modelos de dimensiones extra:  Randall-Sundrum y Clockwork/Linear DilatÃ³n. La fenomenologÃ­a estudiada sobre estos modelos ha requerido un anÃ¡lisis exhaustivo de ambos escenarios.

Desde un punto de vista numÃ©rico, toda la fenomenologÃ­a ha sido estudiada mediante lenguaje \textit{C++}, mientras que su representaciÃ³n a nivel grÃ¡fico ha sido obtenida utilizando \textit{python}. El anÃ¡lisis de la DetecciÃ³n Indirecta de Materia Oscura realizado en uno de los modelos estudiados ha requerido el uso de software mÃ¡s especÃ­fico: \textit{micrOMEGAs}, \textit{SARAH}, \textit{gamlike}, \textit{pythia} y \textit{MadGraph}. Por otro lado, todo el estudio de la EcuaciÃ³n de Boltzman en los cuatro modelos se ha realizado mediante mÃ©todos numÃ©ricos implementados en lenguaje \textit{C++}.

Finalmente, el enfoque fenomenolÃ³gico que presenta esta Tesis ha implicado un contacto continuo con datos experimentales. El tratamiento de estos datos, asÃ­ como las diferentes cotas de exclusiÃ³n que han puesto sobre los diferentes modelos estudiados, ha requerido un uso de diversas tÃ©cnicas estadÃ­sticas. Se han utilizado diferentes distribuciones de probabilidad (tales como la conocida $\chi^2$), tÃ©cnicas de Monte Carlo, etc.

\section{Resultados y conclusiones de la Tesis}

En estÃ¡ secciÃ³n, vamos a realizar un breve resumen de los proyectos que conforman esta Tesis. Todos ellos pueden encontrarse completos en la Parte \ref{sec:papers}.

\subsection{Estudio de la DetecciÃ³n Indirecta del Modelo de \textit{Portal de Neutrinos EstÃ©riles}}

Uno de los grandes problemas abiertos en fÃ­sica de altas energÃ­as es la Materia Oscura, pero desde luego no es el Ãºnico. Entre los diversos problemas que existen actualmente en el Modelo EstÃ¡ndar de partÃ­culas, uno de los mÃ¡s importantes es la masa de los neutrinos. El modelo predice una masa nula para ellos, no obstante, hace ya mÃ¡s de medio siglo se predijo un efecto denominado \textit{oscilaciones de neutrinos} \cite{Pontecorvo:1957cp}. Este curioso fenÃ³meno, que fue confirmado experimentalmente en 1999 \cite{Fukuda:1998mi}, consiste en una oscilaciÃ³n en el sabor leptÃ³nico de los neutrinos. Las implicaciones de este hecho son muy profundas ya que Ãºnicamente puede suceder si al menos uno de los tres sabores de neutrinos es masivo\footnote{\miguel{A pesar de que el fenÃ³meno podrÃ­a explicarse con un solo neutrino masivo, la observaciÃ³n del fenomeno tanto en neutrinos atmosfericos como solares requiere que al menos dos de los tres sabores de neutrinos sean masivos.}}. No obstante, las cotas experimentales impuestas a la masa de estas partÃ­culas prÃ¡cticamente invisibles son tan fuertes que su masa debe ser muy pequeÃ±a\footnote{El lÃ­mite actual mÃ¡s fuerte viene dado por el experimento \textit{Karlsruhe Tritio Neutrino} (KATRIN) \cite{Aker:2019uuj}.}.
Este hecho potenciÃ³ el desarrollo de modelos en los que la masa de los neutrinos era generada por mecanismos de tipo \textit{balancÃ­n}\footnote{Modelo \textit{seesaw} en inglÃ©s.} \cite{GellMann:1980vs,PhysRevLett.44.912,Yanagida:1979as,Glashow1111,MINKOWSKI1977421}. Hay diferentes versiones de estos modelos, en el \textit{tipo I}, por ejemplo, se asume la existencia de neutrinos dextrÃ³giros muy masivos que justifican la pequeÃ±a masa de los neutrinos del Modelo EstÃ¡ndar. La mezcla de los neutrinos levÃ³giros con los dextrogiros da como resultado los autoestados de masa, prediciendo neutrinos con masas muy grandes y muy pequeÃ±as.

La posibilidad de que el problema de la Materia Oscura y de la masa de los neutrinos estÃ©n relacionados motivÃ³ el desarrollo del conocido como\footnote{El escenario mÃ¡s econÃ³mico, la posibilidad de que los neutrinos estÃ©riles sean la Materia Oscura, fue propuesto en Ref.~\cite{Dodelson:1993je}. A dÃ­a de hoy, esta posibilidad ha sido fuertemente estudiada y prÃ¡cticamente descartada \cite{Adhikari:2016bei}.} \textit{portal de neutrinos estÃ©riles a Materia Oscura} \cite{Escudero:2016tzx,Macias:2015cna,Escudero:2016ksa}. Este modelo se ha estudiado por diversos autores, acotÃ¡ndolo utilizando la DetecciÃ³n Directa de Materia Oscura. No obstante, es un modelo muy interesante desde el punto de vista de la DetecciÃ³n Indirecta por varios motivos. Por un lado, la DetecciÃ³n Directa en este escenario no sucede al orden mÃ¡s bajo en teorÃ­a de perturbaciones de la teorÃ­a cuÃ¡ntica de campos. Este hecho hace que sus seÃ±ales de DetecciÃ³n Directa sean bajas que en otros modelos, empeorando asÃ­ los lÃ­mites impuestos. Por otro lado, la conexiÃ³n de los neutrinos estÃ©riles con los neutrinos activos hace que las aniquilaciones de Materia Oscura produzcan, como resultado de diversas desintegraciones, excesos de fotones y partÃ­culas cargadas. Todo esto lo convierte en el candidato perfecto para ser estudiado desde el punto de vista de la DetecciÃ³n Indirecta, tal como se ha llevado a cabo en la Ref.~\cite{Folgado:2018qlv}.

En este trabajo hemos analizado un modelo particular en el que, ademÃ¡s de los neutrinos estÃ©riles, se asume la existencia de dos nuevos campos: uno escalar $\phi$ y otro fermionico $\Psi$. Estos campos son ambos singletes del Modelo EstÃ¡ndar, no obstante, estÃ¡n cargados respecto a un nuevo grupo de simetrÃ­a, $G_{\text{dark}}$, de tal forma que la combinaciÃ³n $ \overline{\Psi} \phi$ es singlete de este nuevo grupo de simetrÃ­a.

\begin{figure}[htbp]
\centering
\includegraphics[width=120mm]{figures/resultados_paper_1.pdf}
\caption[Resultados del primer articulo.]{\it LÃ­mites sobre el \textit{portal de neutrinos estÃ©riles} en el espacio de masas. La regiÃ³n amarilla muestra los lÃ­mites impuestos por los antiprotones mientras que la regiÃ³n azul son los lÃ­mites impuestos por los fotones procedentes de las galaxias enanas. Los diferentes contornos muestran la zona en la que el modelo es capaz de reproducir el GCE. La lÃ­nea discontinua azul muestra nuestra predicciÃ³n sobre el lÃ­mite de las galaxias enanas para los prÃ³ximos 15 aÃ±os.}
 \label{fig:resultados_paper_1}
\end{figure}

La mÃ¡s ligera de estas nuevas partÃ­culas \textit{oscuras} ($\phi$ y $\Psi$) es estable si todas las particulas del Modelo EstÃ¡ndar, asÃ­ como los neutrinos esteriles, son singletes de $G_{\text{dark}}$, independientemente de la naturaleza de este grupo de simetrÃ­a. Como consecuencia, debido a su estabilidad esta partÃ­cula es un buen candidato a Materia Oscura. Por simplicidad, asumimos que $G_{\text{dark}}$ es una simetrÃ­a global a baja enerÃ­a, en cualquier caso no esperamos cambios significantes en nuestro analisis fenomenolÃ³gico si esta fuese local.

Los terminos mÃ¡s relevantes en el lagrangiano vienen dados por:
\bea
\mathcal{L} &=& \mu_H^2 H^\dagger H - \lambda_H (H^\dagger H)^2  -
\mu_\phi^2 \phi^\dagger \phi - \lambda_\phi (\phi^\dagger \phi)^2 - 
\lambda_{H\phi} (H^\dagger H) \, (\phi^\dagger \phi)   
\nonumber \\
&-&\left( \phi \overline{\Psi}(  \lambda_a +  \lambda_p \gamma_5) N 
 + Y \overline {L}_L H N_{R}  + {\rm h.c.}  \right)  \, .
\eea

Los acoplamientos de Yukawa $Y$ entre los neutrinos dextrÃ³giros $N_R$ y el doblete leptÃ³nico del Modelo EstÃ¡ndar genera las masas para los neutrinos activos despuÃ©s de la ruptura espontanea de la simetrÃ­a, a traves del mecanismo \textit{balancÃ­n} de tipo I. Si bien se requieren al menos dos neutrinos estÃ©riles para generar las masas de neutrinos observadas en las oscilaciones, en nuestro anÃ¡lisis consideramos que solo una especie es mÃ¡s ligera que la Materia Oscura y, por lo tanto, relevante para la determinaciÃ³n de su abundancia y bÃºsquedas indirectas. No obstante, los resultados son fÃ¡clmtente extendibles al caso en el que tenemos dos o mÃ¡s neutrinos estÃ©riles mÃ¡s ligeros que la Materia Oscura. Bajo el supuesto de que la Materia Oscura es descrita por $\Psi$ (el anÃ¡lisis es igualmente valido en el caso de que la Materia Oscura sea $\phi$) las masas del modelo cumplen la relaciÃ³n $m_N < m_\Psi < m_\phi$.

La Fig.~\ref{fig:resultados_paper_1} muestra los resultados finales de nuestro anÃ¡lisis. Fijando la masa del mediador escalar para obtener la abundancia de Materia Oscura mediante el mecanismo \textit{freeze-out} (es decir $\langle \sigma \, v \rangle \sim 2 \times 10^{-26} cm^3/s$), la figura muestra los diferentes limites impuestos por las bÃºsquedas de fotones y antiprotones en el espacio de masas $(M_N,M_\Psi)$. Como ya hemos comentado, el experimento Fermi-LAT ha reportado un exceso de fotones inexplicable procedente del centro galÃ¡ctico (GCE). El modelo estudiado predice un pequeÃ±o exceso de fotones que podrÃ­a ser compatible con el GCE en ciertas zonas del espacio de parÃ¡metros. En nuestro analisis hemos asumidoque existen dos fuentes diferentes para el GCE: una astrofÃ­sica, responsable de la zona de alta energÃ­a del espectro de fotones, y otra procedente de las aniquilaciones de Materia Oscura, la cual explicarÃ­a la zona de baja energÃ­a del exceso,  
\be
\Phi = \Phi_{\text{astro}} + \Phi_{\text{DM}} \, .
\ee
Esta contribuciÃ³n astrofÃ­sica al flujo de fotones es siempre necesaria para reproducir el GCE, independientemente del modelo de Materia Oscura considerado.
La zona en la que puede realizarse el ajuste del exceso de fotones del centro galactico estÃ¡ delimitada por los diferentes contornos que se observan en la figura (en la leyenda estÃ¡ indicado el p-valor asociado a cada contorno). No obstante, este aumento de fotones predicho por el modelo tiene que ser compatible tambiÃ©n con el resto de medidas realizadas sobre los diferentes flujos de fotones. En concreto, el mismo experimento realiza medidas sobre los fotones procedentes de 15 galaxias enanas\footnote{Galaxias compuesta por varios millones de estrellas. En contraposiciÃ³n tenemos las galaxias normales, compuestas por varios miles de millones.}, la regiÃ³n sombreada en azul muestra la zona del espacio de parÃ¡metros de la teorÃ­a en la cual los resultados obtenidos no son compatibles con dichas mediciones al 90 \% de intervalo de confianza.

Por otro lado, el modelo tambiÃ©n predice un aumento del flujo de antiprotones. Este aumento se ha comparado con el flujo de antiprotones procedente del centro galÃ¡ctico, el cual es medido en la actualidad por el experimento AMS-02.Los resultados obtenidos muestran que existen zonas en las cuales las predicciones del modelo no serÃ­an compatibles al 95 \% de intervalo de confianza con lo observado experimentalmente (zona sombreada en amarillo en la figura).
Por Ãºltimo, tambiÃ©n se ha realizado un anÃ¡lisis del posible impacto de los resultados futuros el experimento Fermi-LAT. Basandonos en la mejora experimentada por la colaboraciÃ³n, hemos estimado que en 15 aÃ±os se habrÃ¡n detectado 45 galaxias enanas nuevas. Este hecho podrÃ­a poner fuertes cotas al modelo estudiado (lÃ­nea azul discontinua). Como comentario final, podemos decir que algunos modelos de Materia Oscura son capaces de explicar el exceso de fotones del centro galactico parcialmente\footnote{Hasta el momento todos los modelos necesitan asumir que parte del exceso es consecuencia a fenomenos astrofÃ­sicos.}. En concreto, el modelo aquÃ­ estudiado consigue reproducirlo con una precisiÃ³n muy alta. No obstante, los resultados futuros del experimento Fermi-LAT podrÃ­an excluir casi por completo la regiÃ³n del espacio de parÃ¡metros en la cual el GCE puede ser explicado por el modelo.

\subsection{Materia Oscura Escalar Mediada por Gravedad en Dimensiones Extra Deformadas}

Todas las evidencias que tenemos hoy en dÃ­a acerca de la existencia de la Materia Oscura estÃ¡n relacionadas con la interacciÃ³n gravitatoria. Este hecho induce a pensar en la posibilidad de que las partÃ­culas de Materia Oscura Ãºnicamente interactÃºen gravitatoriamente. Esta idea tan natural ha sido explorada ya para los candidatos de tipo WIMP sin demasiado exito: la intensidad de la interacciÃ³n gravitatoria es muy dÃ©bil y hace imposible obtener la cantidad de abundancia de Materia Oscura que se observa en la actualidad (al menos en el escenario WIMP). No obstante, Â¿que ocurre si pensamos en mÃ¡s de 4 dimensiones? Esta es la idea que inspirÃ³ la Ref.~\cite{Folgado:2019sgz}.

En dicho artÃ­culo tratamos de explorar si es posible obtener la abundancia de Materia Oscura actual, asumiendo que es de tipo WIMP escalar, Ãºnicamente mediante interacciÃ³n gravitatoria y bajo el supuesto de un Universo 5-dimensional de tipo Randall-Sundrum. En el escenario descrito, la Materia Oscura y el Modelo EstÃ¡ndar viven confinados en la brana infrarroja. Ambos tipos de materia interactÃºan Ãºnicamente a travÃ©s de la gravedad, cuya proyecciÃ³n sobre la brana IR es equivalente a una torre de gravitones 4-dimensionales masivos (torre de Kaluza-Klein).

El modelo queda descrito en base a cuatro parÃ¡metros fÃ­sicos: la escala de la interacciÃ³n de los gravitones 4-dimensionales con la materia, $\Lambda$; la masa del primer gravitÃ³n de la torre de KK, $m_{1}$; la masa del candidato a Materia Oscura, $m_{\text{DM}}$ y la masa del radiÃ³n, $m_r$. Nuestro estudio muestra que cuando $m_r < m_\text{DM}$ y, en consecuencia, el canal de aniquilaciÃ³n a radiones esta abierto, el valor de $m_r$ es prÃ¡cticamente irrelevante para la fenomenologÃ­a. 
Respecto a la aniquilaciÃ³n de la Materia Oscura a partÃ­culas del Modelo Estandar a traves del intercambio de radiones virtuales, esta secciÃ³n eficaz Ãºnicamente es relevante cerca de la resonancia $m_\text{DM} \backsim m_r/2$. Por lo tanto, en el estudio fenomenolÃ³gico realizado hemos fijado la masa del radion y nos hemos centrado en el resto de parÃ¡metros libres del modelo.

El mÃ©todo seguido para el anÃ¡lisis del modelo ha sido la construcciÃ³n de una malla bidimensional con diferentes valores de los parÃ¡metros $(m_{G_1},m_\text{DM})$. Para cada uno de los puntos de este mallado hemos buscado si existe algÃºn valor de $\Lambda$ para el cual se obtiene la abundancia de Materia Oscura actual (es decir, para $\langle \sigma v \rangle \backsimeq \langle \sigma v \rangle_\text{fo} = 2 \times 10^{-26} \, \text{cm}^3/\text{s}$). De este modo, para cada punto del mallado los tres parÃ¡metros libres ($m_{1}$, $m_\text{DM}$, $\Lambda$) quedan totalmente definidos. Este anÃ¡lisis nos permite establecer diferentes lÃ­mites teÃ³ricos y experimentales en el espacio de masas del modelo. 

\begin{figure}[t]
\centering
\includegraphics[width=150mm]{figures/resultados_paper_2.png}
\caption[Resultados del segundo articulo.]{\it RegiÃ³n en el plano $(m_{\text{DM}}, m_{1})$ para la cual 
$\left\langle \sigma v \right\rangle = \left\langle \sigma_{\rm fo} v \right\rangle$. La grÃ¡fica de la izquierda muestra el caso sin radiÃ³n, mientras que en la de la derecha se ha considerado $m_r = 100$ GeV. Las lÃ­neas discontinuas muestran los diferentes valores de $\Lambda$ en el plano ($m_\text{DM},m_{1}$) para los cuales se consigue la abundancia actual de Materia Oscura. La zona gris muestra la regiÃ³n en la cual es imposible conseguir la abundancia de Materia Oscura, independientemente del valor de $\Lambda$. Por otro lado, la regiÃ³n naranja nos indica los puntos en los que la abundancia se consigue gracias a los canales de interacciÃ³n en los que interviene el radiÃ³n. Respecto a los lÃ­mites sobre el modelo: la zona de cuadraditos verde representa el lÃ­mite de unitariedad; la zona de cuadraditos rosa representa la zona en la que la teorÃ­a efectiva deja de tener validez, es decir $\Lambda < m_{1}$; la zona roja representa los lÃ­mites impuestos por el experimento Xenon1T sobre la secciÃ³n eficaz de DetecciÃ³n Directa; la regiÃ³n azul es la zona eliminada por las bÃºsquedas de resonancias en el LHC usando los datos de 36 fb$^{-1}$ at $\sqrt{s} = 13$ TeV. Finalmente, las lÃ­neas punteadas son las predicciones de exclusiÃ³n para las fases \textit{Run-III} (con $\sim 300$ fb$^{-1}$) y \textit{High Luminosity} (con $\sim 3000$ fb$^{-1}$) del LHC.}
 \label{fig:resultados_paper_2}
\end{figure}

En la Fig.~\ref{fig:resultados_paper_2} pueden verse los resultados finales del anÃ¡lisis fenomenolÃ³gico sobre el modelo. En la parte izquierda se ha explorado el caso sin radiÃ³n, asumiendo que podrÃ­a encontrarse algÃºn mÃ©todo alternativo para estabilizar el radio de la quinta dimensiÃ³n. Por otro lado, en la parte derecha se ha considerado que la masa del radiÃ³n es $m_r = 100$ GeV (es importante recordar que la fenomenologÃ­a no se ve afectada por el valor de esta masa). La zona sombreada en gris es la regiÃ³n en la que no es posible obtener la abundancia actual de Materia Oscura para ningÃºn valor de $\Lambda$, mientras que la zona naranja representa la regiÃ³n del espacio de parÃ¡metros en la que la abundancia se consigue gracias a las contribuciones de los canales de interacciÃ³n radiÃ³nicos. La zona sombreada con cuadraditos verdes se conoce como lÃ­mite de unitariedad y representa el punto a partir del cual la secciÃ³n eficaz de interacciÃ³n es tan alta que la teorÃ­a de campos deja de tener sentido, esto sucede para\footnote{\miguel{En el escenario WIMP las partÃ­culas de Materia Oscura tienen una velocidad relativa muy pequeÃ±a. Este hecho implica que $s \backsimeq m_{\text{DM}}^2 (4 + v^2_{\text{rel}}) $, donde $v_{\text{rel}} \ll 1 $ es la velocidad relativa de las partÃ­culas de Materia Oscura. Además, para conseguir la abundancia de Materia Oscura observada en la actualidad debe cumplirse $\sigma = \sigma_{\text{fo}}$. Como consecuencia, este lÃ­mite se convierte en un lÃ­mite sobre la masa de la Materia Oscura $m_{\text{DM}}^2 \lesssim 1/\sigma_{\text{fo}}$. Por lo tanto, enel plano de masas ($m_\text{DM}$, $m_1$) la zona excluida por unitariedad aparece como una linea vertical.}} $\sigma > 1/s$. AdemÃ¡s de este lÃ­mite, existe otra restriccion teÃ³rica: si $\Lambda < m_{\text{DM}}, m_{1}$ la teorÃ­a efectiva que describe la interacciÃ³n de estos campos cuÃ¡nticos deja de tener sentido (ya que deberÃ­an estar integrados). Esto ocurre en la regiÃ³n de cuadraditos rosa.

Hasta el momento, hemos hablado de las diferentes restricciones al modelo por motivos teÃ³ricos, pero estos no son los Ãºnicos lÃ­mites que pueden establecerse: los actuales experimentos de DetecciÃ³n Directa y las bÃºsquedas de resonancias en los experimentos ATLAS y CMS del LHC pueden aportar mucha informaciÃ³n a nuestro anÃ¡lisis. De este modo, las zonas sombreadas en rojo representan los puntos en los que la secciÃ³n eficaz de DetecciÃ³n Directa estÃ¡ ya excluida por los actuales experimentos. Por otro lado, la zona azul es la excluida por las bÃºsquedas de resonancias (gravitones 4-dimensionales en nuestro caso) en el LHC, se han utilizado los datos tomados a $\sqrt{s} = 13$ TeV con 36 fb$^{-1}$ en el canal $\gamma \gamma$. Las dos lÃ­neas punteadas muestran nuestra predicciÃ³n sobre los lÃ­mites futuros que serÃ¡n impuestos por el LHC despuÃ©s de las futuras fases \textit{Run-3} (con $\sim 300$ fb$^{-1}$) y \textit{High Luminosity} (con $\sim 3000$ fb$^{-1}$), en el caso de que no se detecte ninguna resonancia.

El estudio realizado muestra que, en las regiones no excluidas del espacio de parÃ¡metros, la fenomenologÃ­a estÃ¡ dominada por los canales de interacciÃ³n relacionados con los gravitones. En dichas regiones, de acuerdo con nuestro anÃ¡lisis, los canales de interacciÃ³n radiÃ³nicos siempre son subdominantes. Para ser mÃ¡s exactos, la abundancia se consigue gracias a la aniquilaciÃ³n de Materia Oscura directamente en gravitones.

Aunque ya se habÃ­an realizado anÃ¡lisis similares en Randall-Sundrum, este trabajo es el primero que tiene en cuenta los canales de aniquilaciÃ³n de Materia Oscura directamente a gravitones en regiones tan altas del espacio de masas (varios TeV). AsÃ­ mismo, se ha estudiado un diagrama totalmente olvidado en la literatura hasta el momento: la aniquilaciÃ³n a gravitones sin mediador, procedente del desarrollo a segundo orden del lagrangiano de interacciÃ³n. Aunque el impacto de este diagrama sobre la fenomenologÃ­a no cambia drÃ¡sticamente los resultados, debe ser aÃ±adido por consistencia ya que es del mismo orden que el resto de diagramas estudiados. Por otro lado, cabe destacar que este anÃ¡lisis Ãºnicamente se ha realizado para Materia Oscura escalar. No obstante, en la Ref.~\cite{Folgado:2020vjb} que estÃ¡ actualmente en trÃ¡mites de publicaciÃ³n, se analizan los casos de Materia Oscura fermiÃ³nica y vectorial. En este estudio se ve que la Materia Oscura de tipo fermionico estÃ¡ claramente desfavorecida respecto a la escalar y vectorial ya que el canal dominante (la aniquilaciÃ³n directamente a gravitones) estÃ¡ mÃ¡s suprimido que en el resto de casos.

\subsection{Materia Oscura Mediada por Gravedad en Dimensiones Extra Tipo \textit{Clockwork/Linear DilatÃ³n}}

Analizadas las implicaciones de la existencia de Materia Oscura tipo WIMP con interacciones puramente gravitatoria en el escenario de Randall-Sundrum, la pregunta de que ocurrirÃ­a en el novedoso Clockwork/Linear DilatÃ³n casi surge de forma natural. Esta idea inspirÃ³ la Ref.~\cite{Folgado:2019gie}. La estructura de este escenario es diferente a la que tenÃ­amos en RS: la torre de KK de gravitones masivos en este caso tiene una separaciÃ³n muy pequeÃ±a y variable. Este hecho dificulta en gran medida el anÃ¡lisis numÃ©rico de su fenomenologÃ­a.

A nivel conceptual, la estrategia para abordar el modelo es idÃ©ntica a la empleada en el caso RS. La gran diferencia con el modelo anterior son los parÃ¡metros elegidos para estudiar la fenomenologÃ­a. En CW/LD los acoplamientos de los gravitones 4-dimensionales masivos al resto de partÃ­culas dependen del orden del gravitÃ³n dentro de la torre. Por ello, es mÃ¡s Ãºtil caracterizar el modelo en funciÃ³n de $M_5$ directamente, en lugar de usar los acoplamientos efectivos $\Lambda_n$ de los gravitones 4-dimensionales. Por otro lado, la masa del primer gravitÃ³n coincide prÃ¡cticamente con el valor de la curvatura a lo largo de la quinta dimensiÃ³n $m_{1} = k$. Otra diferencia notable entre ambos escenarios es la estabilizaciÃ³n del tamaÃ±o de la dimensiÃ³n extra. En RS es necesario introducir un nuevo campos escalar en el \textit{bulk} con el fin de estabilizar dinamicamente $r_c$. En cambio, en CW/LD el dilatÃ³n presente en la mÃ©trica puede utilizarse para escribir los potenciales en la brana y estabilizar asÃ­ el tamaÃ±o de la quinta dimensiÃ³n. En este caso, la masa del radiÃ³n (modo cero de la torre de dilatones 4-dimensionales) estÃ¡ fijada por los parÃ¡metros fundamentales del modelo (ya que deriva directamente de la mÃ©trica). No obstante, hay diferentes formas de realizar la estabilizaciÃ³n usando el dilatÃ³n, el caso mÃ¡s simple es asumir que la tensiÃ³n de las branas es infinita. Este escenario, recibe el nombre de lÃ­mite rigido.

\begin{figure}[htbp]
\centering
\includegraphics[width=150mm]{figures/resultados_paper_3.png}
\caption[Resultados del tercer articulo.]{\it RegiÃ³n en el plano $(m_{\rm DM}, k)$ para la cual $\left\langle \sigma v \right\rangle = \left\langle \sigma_{\rm fo} v \right\rangle$. Las grÃ¡ficas superiores muestran los resultados para el caso de Materia Oscura escalar, la inferior izquierda el caso fermiÃ³nico y la inferior derecha el vectorial. La grÃ¡fica superior izquierda muestra las diferentes zonas de exclusiÃ³n teniendo en cuenta Ãºnicamente la interacciÃ³n con gravitones. Por otro lado, en la grÃ¡fica superior derecha se han considerado ambas, la interacciÃ³n mediante gravitones y mediante dilatones, para el caso de Materia Oscura escalar. En los casos fermiÃ³nico y vectorial no se muestra el caso sin dilatones ya que la contribuciÃ³n de los mismos es despreciable y no varÃ­a los resultados. Las lÃ­neas discontÃ­nuas muestran los diferentes valores de $M_5$ en el plano ($m_\text{DM},k$) para los cuales se consigue la abundancia actual de Materia Oscura, mientras que la zona gris muestra la regiÃ³n en la cual es imposible conseguir dicha abundancia, independientemente del valor de $M_5$.
Respecto a los lÃ­mites sobre el modelo: la zona de cuadraditos verde representa el lÃ­mite de unitariedad ($m_{\rm DM} \gtrsim 1/\sqrt{\sigma_{\rm fo}}$); la regiÃ³n de cuadraditos rosa representa el Ã¡rea en la que la teorÃ­a efectiva deja de tener validez ($M_5 < k, m_\text{DM}$) y, finalmente, la regiÃ³n azul representa los lÃ­mites impuestos por las bÃºsquedas no-resonantes en el LHC usando los datos de 36 fb$^{-1}$ a $\sqrt{s} = 13$ TeV para el canal $\gamma \gamma$ \cite{Giudice:2017fmj}.}
 \label{fig:resultados_paper_3}
\end{figure}

La Fig.~\ref{fig:resultados_paper_3} muestra los diferentes lÃ­mites obtenidos para este escenario. AnÃ¡logamente al caso RS, $M_5$ se ha utilizado para fijar la abundancia actual de Materia Oscura para cada punto del espacio ($m_{\text{DM}},k$). Los diferentes lÃ­mites estudiados son los mismos que en el caso anterior: la regiÃ³n de cuadraditos rosa muestra los lÃ­mites de la teorÃ­a efectiva ($M_5 < k, m_\text{DM}$), la regiÃ³n de cuadraditos verdes el lÃ­mite de unitariedad ($m_{\rm DM} \gtrsim 1/\sqrt{\sigma_{\rm fo}}$) y, finalmente, la zona sombreada en azul los lÃ­mites impuestos por el LHC. En el caso de los lÃ­mites experimentales, debido a la proximidad de las resonancias en la torre de gravitones, el lÃ­mite mÃ¡s estricto impuesto por el LHC viene de las bÃºsquedas en el espectro continuo de energÃ­as, en lugar de las bÃºsquedas de resonancias. Estos lÃ­mites han sido calculados usando los datos de 36 fb$^{-1}$ a $\sqrt{s} = 13$ TeV para el canal $\gamma \gamma$ \cite{Giudice:2017fmj}. Finalmente, cabe destacar que, en este caso, los lÃ­mites impuestos por las bÃºsquedas de DetecciÃ³n Directa de Materia Oscura corresponden a valores de ($m_\text{DM},k$) menores que los mostrados en la Figura. 

Otra diferencia notable con el caso RS es que aquÃ­ no solo hay que considerar el radiÃ³n en la fenomenologÃ­a, si no tambiÃ©n toda la torre de KK de los dilatones. No obstante, en CW/LD el radiÃ³n y los dilatones derivan directamente de la mÃ©trica del modelo, no es necesario un mecanismo externo para estabilizar el tamaÃ±o de la quinta dimensiÃ³n. Este hecho hace que la masa de los mismos este intrÃ­nsecamente ligada a los parÃ¡metros fundamentales del modelo, sin agregar de este modo ningÃºn grado nuevo de libertad al espacio de parÃ¡metros de la teorÃ­a.

En este trabajo se han analizado los tres posibles tipos de Materia Oscura: escalar, fermiÃ³nica y vectorial. Las dos figuras superiores corresponden al caso escalar sin tener en cuenta la torre de radiÃ³n y dilatones (izquierda) y teniÃ©ndola en cuenta (derecha), respectivamente. Este es el Ãºnico caso en el que los dilatones juegan un papel importante en la fenomenologÃ­a del modelo y por ello merece la pena mostrar cuÃ¡l es su impacto sobre los resultados finales. Las grÃ¡ficas inferiores corresponden al caso fermiÃ³nico (izquierda) y al caso vectorial (derecha). Se puede ver claramente que el caso fermiÃ³nico estÃ¡ desfavorecido respecto a los otros dos. Este hecho se debe a que en el caso fermiÃ³nico el canal dominante, la aniquilaciÃ³n de Materia Oscura directamente a gravitones, sufre una supresiÃ³n debido al momento angular total.

El anÃ¡lisis llevado a cabo en este trabajo representa el primer estudio fenomenolÃ³gico del modelo CW/LD con presencia de Materia Oscura. Los resultados anteriores, al igual que en RS, son prometedores en el sentido de que toda la regiÃ³n no excluida podrÃ¡ ser analizada en los prÃ³ximos aÃ±os por el LHC. Como comentario final sobre la Materia Oscura tipo WIMP pÃºramente gravitatoria, podemos decir que en ambos escenarios es posible reproducir la abundancia actual en el rango $m_\text{DM} \in [1,10] \, \text{TeV}$. No obstante, los valores necesarios, tanto de $\Lambda$ en RS como de $M_5$ en CW/LD, para ello son excesivamente grandes como para resolver el problema de la jerarquÃ­a.

\subsection{Materia Oscura FIMP en Dimensiones Extra Deformadas}

Hasta el momento, todos los modelos analizados consideran partÃ­culas tipo WIMP. No obstante, la Materia Oscura tipo FIMP es muy interesante para el caso en el que la interacciÃ³n es puramente gravitatoria. En el Ãºltimo proyecto incluido en esta Tesis hemos explorado la posibilidad de reproducir la abundancia de Materia Oscura actual utilizando partÃ­culas FIMP en un escenario tipo RS \cite{Bernal:2020fvw}. Este caso plantea complicaciones matemÃ¡ticas y numÃ©ricas muy diferentes al caso WIMP. Entre estos problemas, el mÃ¡s importante es que la abundancia final predicha por el modelo depende en gran medida de las condiciones iniciales. Este hecho hace que, mientras que en el caso WIMP\footnote{Como consecuencia del \textit{milagro WIMP}.} la abundancia actual se reproduce para un valor constante de la secciÃ³n eficaz de interacciÃ³n ($\left\langle \sigma v \right\rangle = \left\langle \sigma_{\rm fo} v \right\rangle$), en el caso FIMP es necesario resolver siempre la ecuaciÃ³n diferencial que determina su evoluciÃ³n, la conocida como ecuaciÃ³n de Boltzmann.

\begin{figure}[htbp]
\centering
\includegraphics[width=110mm]{figures/resultados_paper_4.pdf}
\caption[Resultados del cuarto articulo.]{\it Valores de la temperatura de reheating (lineas negras) para los cuales un determinado valor de la escala de interacciÃ³n en la brana y la masa del primer graviton reproducen la abundancia de Materia Oscura actual para $m_\text{DM} = 1$ MeV y $m_r = m_1/10^3$. La zona azul representa la regiÃ³n excluida por las bÃºsquedas de resonancias del LHC. La regiÃ³n roja muestra el lÃ­mite de la teorÃ­a efectiva $m_1>\Lambda$. Finalmente, la regiÃ³n verde muestra la zona en la que el valor de la vida media del radiÃ³n entra en conflicto con las observaciones de la NucleosÃ­ntesis del Big Bang.}
 \label{fig:resultados_paper_4}
\end{figure}

Por otro lado, aquÃ­ la abundancia tambiÃ©n tiene una fuerte dependencia con un nuevo parÃ¡metro: la temperatura mÃ¡xima del Universo, conocida como temperatura de \textit{reheating} ($T_{\text{rh}}$). Debido a la complejidad del espacio de parÃ¡metros, el analisis en este escenario se ha llevado a cabo para un valor determinado de la masa de la Materia Oscura: $m_{\textit{DM}} = 1$ MeV, no obstante, los resultados son similares para otros valores $m_{\textit{DM}} $. En la Fig.~\ref{fig:resultados_paper_4} se muestran los valores necesarios de la temperatura de reheating para obtener la abundancia observada. La regiÃ³n azul sombreada muestra los lÃ­mites experimentales impuestos por las bÃºsquedas de resonancias en el canal $pp \rightarrow G_1 \rightarrow \gamma \, \gamma$ en el LHC (y las dos predicciones para las futuras etapas del experimento). Por otro lado, los lÃ­mites teÃ³ricos en este escenario vienen determinados por la validez de la teorÃ­a efectiva (regiÃ³n roja) y la \textit{NucleosÃ­ntesis del Big Bang}. Este Ãºltimo lÃ­mite se traduce en una restricciÃ³n sobre la vida media de los gravitones y del radiÃ³n: si la $\tau>1$ s se podrÃ­an producir modificaciones en las observaciones sobre la NucleosÃ­ntesis del Big Bang que deberÃ­an estar reflejadas en los datos experimentales actuales. En los modelos analizados anteriormente, este lÃ­mte no aparecia ya que la vida media de los gravitones y radion/dilatones siempre era mayor que 1 segundo. 

A la vista de los resultados obtenidos, vemos que el caso FIMP estÃ¡ mucho menos excluido que el caso WIMP en el escenarios de RS y que la abundancia de Materia Oscura actual se consigue en una gran regiÃ³n muy amplia del espacio de parÃ¡metros. A pesar de ello, los valores obtenidos para los parÃ¡metros libres de la teorÃ­a estÃ¡n lejos de resolver el problema de la jerarquÃ­a. Por otro lado, los experimentos actuales aÃºn no son capaces de explorar los parÃ¡metros tÃ­picos de los modelos FIMP. No obstante, el hecho de que los modelos de Materia Oscura tipo FIMP sean capaces de explicar la abundancia actual en un rango del espacio de parÃ¡metros tan amplio es una gran motivaciÃ³n para el futuro desarrollo de experimentos. Actualmente estamos trabajando en el estudio anÃ¡logo para el caso CW/LD.

\subsection{ConclusiÃ³n}

%En esta Tesis hemos estudiado la fenomenologÃ­a de diferentes modelos de Materia Oscura, centrÃ¡ndonos principalmente en los candidatos de tipo WIMP. En este escenario las partÃ­culas de Materia Oscura se encontraban en equilibrio termodinÃ¡mico con el resto de partÃ­culas que componen el Modelo EstÃ¡ndar en el Universo primigenio. A causa de su expansiÃ³n, el Universo sufriÃ³ un proceso de enfriamiento y las partÃ­culas de Materia Oscura terminaron por desacoplarse del plasma primigenio, dejando un remanente que ha llegado hasta nuestros dÃ­as. Este proceso es denominado como \textit{freeze-out}.


%Entre los modelos estudiados en esta Tesis, se ha explorado la posibilidad de que el problema de la Materia Oscura pueda resolverse al mismo tiempo que el de la masa de los neutrinos mediante el Portal de Neutrinos EstÃ©riles. Por la estructura del modelo, este es un candidato perfecto para ser acotado usando la DetecciÃ³n Indirecta. Para ello, primero se ha estudiado la posibilidad de que el exceso de fotones del centro galÃ¡ctico sea consecuencia de las aniquilaciones de Materia Oscura gracias a los neutrinos EstÃ©riles. Se ha visto que, efectivamente, el exceso puede ser reproducido para un pequeÃ±o rango de masas, el cual se encuentra actualmente en tensiÃ³n con otras medidas experimentales: la detecciÃ³n de fotones procedentes de las galaxias enanas y de antiprotones procedentes del centro galÃ¡ctico. AsÃ­ mismo, se ha visto que a lo largo de los prÃ³ximos aÃ±os la mejora de las prestaciones del experimento Fermi-LAT harÃ¡, previsiblemente, que los datos recolectados acerca de las galaxias enanas sean incompatibles con la regiÃ³n del espacio de parÃ¡metros en la que es posible reproducir el exceso de fotones del centro galÃ¡ctico.

%Por otro lado, se ha estudiado la posibilidad de que la Materia Oscura Ãºnicamente presente interacciÃ³n gravitatoria. Esta idea se sustenta en el hecho de que todas las pruebas que tenemos de la existencia de la Materia Oscura estÃ¡n relacionadas Ãºnicamente con la interacciÃ³n gravitatoria. En 4 dimensiones, como consecuencia de la debilidad de la interacciÃ³n, es imposible obtener la cantidad exacta de Materia Oscura que existe actualmente en nuestro Universo. Por este motivo hemos estudiado la viabilidad de esta idea en 5 dimensiones. Efectivamente, se ha comprobado que en espacios 5-dimensionales se puede obtener la abundancia actual de Materia Oscura utilizando Ãºnicamente interacciÃ³n gravitatoria. En este contexto se han analizado dos posibles modelos de dimensiones extra: el conocido modelo Randall-Sundrum y el novedoso \textit{Clockwork/Linear DilatÃ³n}. Los resultados obtenidos en ambos casos son muy prometedores, la abundancia de Materia Oscura se obtiene en una amplia regiÃ³n del espacio de parÃ¡metros que puede ser acotada utilizando los resultados del LHC. En concreto, se ha estudiado el impacto de las bÃºsquedas resonantes y no resonantes en los detectores ATLAS y CMS excluyendo asÃ­ una amplia regiÃ³n del espacio de parÃ¡metros de las dos teorÃ­as. AsÃ­ mismo, en el caso del modelo Randall-Sundrum se ha estudiado el posible impacto de las prÃ³ximas fases del LHC, viendo que la exclusiÃ³n prÃ¡cticamente alcanzarÃ¡ zonas ya eliminadas por diferentes limitaciones teÃ³ricas.

%Por Ãºltimo, mÃ¡s allÃ¡ del escenario WIMP, se ha estudiado otro candidato a Materia Oscura que se caracteriza por su dÃ©bil interacciÃ³n, la Materia Oscura tipo FIMP. En este escenario, la Materia Oscura interacciona tan dÃ©bilmente con el resto de partÃ­culas que jamÃ¡s llegÃ³ a estar en equilibrio en el Universo primigenio. La abundancia de Materia Oscura medida actualmente serÃ­a consecuencia de un proceso totalmente diferente al del caso WIMP, el denominado \textit{freeze-in}. Como consecuencia de su dÃ©bil interacciÃ³n, la Materia Oscura tipo FIMP es un candidato perfecto si Ãºnicamente asumimos interacciÃ³n gravitatoria. En este contexto se ha estudiado la posibilidad de obtener la abundancia de Materia Oscura en el escenario de Randall-Sundrum 5-dimensional. Nuestro anÃ¡lisis muestra que la regiÃ³n del espacio de parÃ¡metros de la teorÃ­a en la cual es posible reproducir la abundancia actual de Materia Oscura es enorme. Las diferentes cotas experimentales y teÃ³ricas limitan mucho menos el espacio de parÃ¡metros que en el caso WIMP. AsÃ­ mismo, las previsiones sobre los futuros lÃ­mites impuestos por el LHC apenas restringen la regiÃ³n permitida. De este modo, el candidato FIMP es mÃ¡s prometedor que el candidato WIMP en el escenario de Randall-Sundrum y la inaccesibilidad del LHC a ciertas regiones permitidas del espacio de parÃ¡metros representan una motivaciÃ³n para nuevos experimentos de fÃ­sica de altas energÃ­as.

Nuestro escaso conocimiento acerca de la naturaleza de la Materia Oscura hace que el conjunto de modelos que pueden explicar las evidencias actuales sea enorme. Esta Tesis ha contribuido a explorar parte de estos modelos y acotar un poco mÃ¡s lo que sabemos de ella, estudiando la fenomenologÃ­a de diferentes candidatos. En general, los resultados obtenidos hacen que esperemos con ansia los resultados de los experimentos futuros, tanto en materia de DetecciÃ³n Indirecta, como en bÃºsquedas del LHC. La relevancia de estos futuros datos es tal que en los prÃ³ximos aÃ±os la existencia de los candidatos de tipo WIMP y FIMP puede verse corroborada o seriamente comprometida. Por otro lado, la dÃ©bil interacciÃ³n de los candidatos de tipo FIMP hace que su futuro experimental sea bastante mÃ¡s incierto. Como comentario final, es cierto que los modelos aquÃ­ estudiados representan una Ã­nfima parte de todo el abanico de posibilidades existentes en la actualidad para explicar este escurridizo tipo de materia. No obstante, espero que hayan arrojado algo de luz sobre tan oscuro misterio.

%Nuestro escaso conocimiento acerca de la naturaleza de la Materia Oscura hace que el conjunto de modelos que pueden explicar las evidencias actuales sea enorme. Esta Tesis ha contribuido a explorar parte de estos modelos y acotar un poco mÃ¡s lo que sabemos de ella, estudiando la fenomenologÃ­a de diferentes candidatos. En general, los resultados obtenidos hacen que tengamos un ojo puesto en los experimentos futuros, tanto en materia de DetecciÃ³n Indirecta, como en bÃºsquedas del LHC. La relevancia de estos futuros datos es tal que en los prÃ³ximos aÃ±os la existencia de los candidatos de tipo WIMP y FIMP puede verse corroborada o seriamente comprometida. Como comentario final, es cierto que los modelos aquÃ­ estudiados representan una Ã­nfima parte de todo el abanico de posibilidades existentes en la actualidad para explicar este escurridizo tipo de materia. No obstante, espero que hayan arrojado algo de luz sobre tan oscuro misterio.


==> Chapters/Resumen_Tesis/Resumen_Tesis_malo.tex <==
\inputencoding{latin1}
\include{Umlaute}       % ISO-8859-1 encoding
\inputencoding{utf8} % back to UTF-8

\chapter{Resumen de la Tesis}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Motivación Histórica}

Desde tiempos inmemoriales, uno de los más profundos deseos del ser humano ha sido descubrir la composición última de la materia que nos rodea. Ya los primeros escritos griegos hablan sobre la modelización de la naturaleza en base a 4 elementos fundamentales; a saber, agua, tierra, fuego y viento. El paso de los siglos afinó mucho más esta prematura descripción. En el siglo XVII, se sintetizó por primera vez un elemento químico\footnote{En 1669 el alquimista Hennig Brand sintetizó por accidente fósforo, bautizándolo con este nombre por el brillo que desprendía.}, y tan solo dos siglos después (1869), ya existía una tabla periódica de los elementos, un claro reflejo de nuestro anhelo por encontrar orden en el caos.

El elevado número de elementos descubiertos en el siglo XX motivó la búsqueda de una estructura mucho más fundamental, aún totalmente desconocida. Fue Niels Bohr quien dió forma a esta idea, proponiendo la teoría atómica actual \cite{Bohr:1913:CAMa,Bohr:1913:CAMb,Bohr:1913:CAMc}, apoyandose en los modelos atómicos propuestos previamente por Joseph John Thomson y Ernest Rutherford. Su elegante modelo explicaba toda forma de matéria utilizando únicamente tres tipos de partículas: neutrones y protones, que componían el núcleo de los diferentes elementos atómicos, y electrones, los cuales orbitaban alrededor de dichos núcleos. Los átomos quedaban descritos pues como pequeños sistemas planetarios, solo que las fuerzas implicadas en su estabilidad eran totalmente diferentes a la gravitatoria.

\begin{figure}[htbp]
\centering
\includegraphics[width=80mm]{figures/Standard_Model_of_Elementary_Particles.pdf}
\caption[Modelo Estándar de las interacciones fundamentales]{\it Modelo Estándar de las interacciones fundamentales: las partículas moradas, verdes y rojas representan, respectivamente, los quarks, leptones y bosones de gauge. Por otro lado, la amarilla representa el Bosón de Higgs. Imagen tomada de Ref.~\cite{citaSM}.}
 \label{fig:modelo_estandar}
\end{figure}

\miguel{A lo largo del siglo XX el desarrollo de la mecánica cuántica cambió totalmente la forma de entender el mundo microscópico. A la fuerza gravitatoria y electromagnetica se le sumaron dos nuevas interacciones: débil y fuerte. Por otro lado, los protones y neutrones, que en el modelo de Bohr eran constituyentes fundamentales de la materia, pasaron a ser partículas compuestas por quarks}. El resultado último de toda la revolución cuántica fue el Modelo Estándar de la física de partículas \cite{PhysRevLett.19.1264,GLASHOW1961579,Salam:1968rm,PhysRevLett.13.321,PhysRev.145.1156,PhysRevLett.13.508,PhysRevLett.13.585,PhysRev.155.1554,PhysRev.139.B1006,PhysRevD.2.1285,FRITZSCH1973365}, esquematizado en la Fig.~\ref{fig:modelo_estandar}. El modelo describe la naturaleza a nivel microscópico utilizando un total de doce partículas elementales, o campos, y cuatro tipos de interacción. Los éxitos del Modelo Estándar fueron totalmente rotundos, con él se han realizado las predicciones más precisas de la historia de la ciencia. No obstante, tiene ciertas limitaciones, como el hecho de que es incapaz de describir la gravedad cuántica. En el Capitulo \ref{sec:SM} se ha realizado una descripción detallada del modelo, profundizando en sus predicciones y fallos.

\miguel{Hoy, casi medio siglo después de que fuese propuesto, sabemos que el Modelo Estandar únicamente es capaz de explicar el $5\%$ del contenido del Universo, el $95\%$ restante continua envuelto en un halo de misterio}. Observaciones astrofísicas y cosmológicas indican que el $26\%$ del Universo está compuesto por un nuevo tipo de materia que no sigue las mismas reglas que la materia bariónica\footnote{Nombre que recibe la materia descrita por el Modelo Estándar.}, comúnmente denominada \textit{Materia Oscura}. El resto del Universo es aún más enigmático si cabe. Actualmente se cree que está compuesto por algún tipo de energía que explicaría la expansión acelerada del Universo, pero esto es otra historia muy diferente a la de la Materia Oscura y queda lejos de los objetivos del trabajo aquí realizado.

La motivación de esta Tesis es intentar arrojar algo de luz sobre ese gran porcentaje de materia que nuestra ciencia actual no ha sido capaz de explicar, haciéndola un poco menos oscura de lo que su nombre indica.


\section{El Modelo Estándar de las Interacciones Fundamentales: La Piedra Angular de la Física de Altas Energías} 
\label{sec:modelo_estandar}

En esta sección vamos a realizar un breve resumen de los conceptos más importantes del Modelo Estándar (en el Capitulo \ref{sec:SM} se han explicado todos los detalles técnicos del mismo). El Modelo Estándar de la física de partículas\footnote{Típicamente abreviado como SM, del inglés Standard Model.} es una teoría cuántica de campos con simetría gauge de los grupos unitarios $SU(3)_C \times SU(2)_L \times U(1)_Y$. El modelo describe con gran precisión tres de las cuatro interacciones fundamentales que existen en la naturaleza: débil, electromagnética y fuerte. La complejidad de la estructura de la interacción gravitatoria hace que sea muy complicado describirla como una teoría de campos gauge, actualmente se trabaja activamente en el tema\footnote{Algunos autores defienden que quizá el origen de la interacción gravitatoria sea totalmente diferente al resto de fuerzas fundamentales. La gravedad emergente (propuesta por Andrei Sakharov en 1967, el artículo original en inglés puede encontrarse en Ref.~\cite{Sakharov_1991}), por ejemplo, sugiere que dicha interacción no es más que el residuo de una serie de grados de libertad aún desconocidos, tal como la mecánica de fluidos, que deriva de la mecánica estadística.}. El resto de las interacciones fundamentales quedan descritas con gran precisión por el modelo mediante el intercambio de diferentes campos de spin 1, que constituyen el sector gauge de la teoría. Mientras que el grupo $SU(3)_C$  se asocia a la interacción fuerte, los grupos $SU(2)_L \times U(1)_Y$ describen la interacción electrodébil\footnote{Las interacciones electromagnéticas y débiles fueron unificadas en los años 70 por Sheldon Lee Glashow, Abdus Salam y Steven Weinberg.}

Mientras que las partículas de spin $1$, o bosones, describen las interacciones del modelo, los constituyentes fundamentales de la materia son los fermiones, partículas de spin $1/2$: quarks y leptones. Curiosamente, la naturaleza replica los fermiones en 3 familias casi idénticas, únicamente diferenciadas por las masas de sus constituyentes: 
\bea
\label{familia_1_CS}
\nth{1} \, \text{Family}: L_{1} \equiv \left( \begin{array}{c}
\nu_e  \\
e^{-}  \end{array} \right)_{L} \, ; \, e_1 \equiv e^{-}_{_R} \, ; \, 
Q_1 \equiv \left( \begin{array}{c}
u  \\
d  \end{array} \right)_{L} \, ; \, U_1 \equiv u_R \, ; \, D_1 \equiv d_R \, , \nonumber \\
\label{familia_2_CS}
\nth{2} \, \text{Family}: L_{2}\equiv\left( \begin{array}{c}
\nu_{\mu}  \\
\mu^{-}  \end{array} \right)_{L} \, ; \, e_2 \equiv \mu^{-}_{_R} \, ; \,
Q_2 \equiv\left( \begin{array}{c}
c  \\
s  \end{array} \right)_{L} \, ; \, U_2 \equiv c_R \, ; \, D_2 \equiv s_R \, , \nonumber \\
\label{familia_3_CS}
\nth{3} \, \text{Family}: L_{3}\equiv\left( \begin{array}{c}
\nu_{\tau}  \\
\tau^{-}  \end{array} \right)_{L} \, ; \, e_3 \equiv \tau^{-}_{_R} \, ; \, 
Q_3 \equiv\left( \begin{array}{c}
t  \\
b  \end{array} \right)_{L} \, ; \, U_3 \equiv t_R \, ; \, D_3 \equiv b_R \, . \nonumber
\eea
\miguel{Por otro lado, el modelo trata de forma diferente a partículas con quiralidad dextrógira y levógira, agrupando las primeras en singletes y las segundas en dobletes de $SU(2)_L$}. De este modo, los quarks y leptones levógiros vienen representados por $Q_i$ (compuesto por los quarks tipo \textit{up} y tipo \textit{down}, con cargas eléctricas $+2/3$ y $-1/3$ de la carga fundamental del electrón, respectivamente) y $L_i$ (compuesto por los leptones cargados y los neutrinos, con cargas eléctricas $-1$ y $0$, respectivamente). Por otro lado, los quarks dextrógiros están representados por los singletes $U_i$ y $D_i$, mientras que los leptones cargados dextrógiros vienen dados por $e_i$.
Los neutrinos dextrógiros no están incluidos en el modelo original, aunque hay muchas líneas de investigación abiertas en la actualidad sobre la posibilidad de su existencia.

Aparte de todo lo comentado, el modelo incluye un campo de spin 0, el campo de Higgs. Los bosones gauge de la teoría débil, es decir $Z$ y $W^\pm)$, tienen masa. Este hecho parecía incompatible con la construcción de un modelo basado en simetrías ya que la invariancia gauge prohíbe términos de masa para los bosones gauge. Por ello, fue necesario desarrollar un mecanismo que dotase de masa estas partículas. La solución a este problema llegó de la mano de Robert Brout, Francois Englert, Gerald Guralnik, Carl Richard Hagen, Peter Higgs y Tom Kibble (en estricto orden alfabético), constituyendo lo que actualmente se conoce como \textit{mecanismo de Higgs} \cite{PhysRevLett.13.321,PhysRev.145.1156,PhysRevLett.13.585,PhysRev.155.1554}.

La idea del mecanismo de Higgs se basa en la \textit{ruptura espontánea de la simetría}\footnote{Del inglés \textit{Spontaneous Symmetry Breaking}.} (SSB) y consiste en agregar a la teoría un campo complejo escalar doblete de $SU(2)_L$:
\be
\Phi = \left( \begin{array}{c}
\Phi^+  \\
\Phi^0  \end{array} \right) = 
\left( \begin{array}{c}
\Phi^+  \\
\dfrac{1}{\sqrt{2}}(v + \phi_1 + i\phi_2)  \end{array} \right) \, .
\ee
Este peculiar campo presenta lo que se conoce como \textit{valor esperado de vacío}\footnote{Del inglés de \textit{Vacuum Expectation Value}.} (VEV) no nulo en su componente neutra, produciendo de este modo una ruptura de la simetría electrodébil (que no es una simetría exacta del vacío) y dando como resultado la simetría electromagnética\footnote{La abreviación QED viene de \textit{Quantum Electrodynamics} \cite{10.1143/PTP.1.27,10.1143/ptp/2.3.101,10.1143/ptp/3.2.101,PhysRev.74.224,PhysRev.74.1439,Feynman:1948ur,Feynman:1949zx}, nombre que recibe la teoría gauge que describe la interacción electromagnética.},
\be
SU(2)_L\times U(1)_Y \longrightarrow U(1)_{QED}.
\ee

\miguel{Durante la SSB, tanto la parte cargada del doblete como la parte imaginaria de la componente neutra son absorbidos como grados de libertad longitudinales por los bosones gauge de la teoría, los cuales pasan a comportarse como bosones masivos.} Por otro lado, la parte real del campo cargado, $\phi_1$, se queda presente en el espectro de partículas del Modelo Estándar como una partícula de spin 0, el popular \textit{bosón de Higgs}. Detectado en 2012 por los experimentos ATLAS \cite{Aad_2012} y CMS del LHC \cite{Chatrchyan_2012}, confirmando el modelo.

El grupo $SU(2)_L\times U(1)_Y$ no presenta simetría quiral, necesaria para escribir los términos de masa de los fermiones en el lagrangiano del modelo. No obstante, el mecanismo de Higgs soluciona este problema ya que $U(1)_{\text{QED}}$ si presenta dicha simetría. En consecuencia, después de la SSB, el VEV del campo de Higgs permite la formación de los términos de masa para estas partículas.

Para una exposición detallada y completa del Modelo Estándar en español ver Ref.~\cite{gelmini2014el}.

\section{La Necesidad de la Materia Oscura}

\miguel{Como ya hemos comentado, el Modelo Estandar de partículas solo puede explicar un porcentaje pequeño de la materia que nos rodea, conocida como \textit{bariónica}. El resto de materia que puebla el Universo recibe el nombre de Materia Oscura\footnote{Su nombre se debe a que no emite ni refleja ningún tipo de luz.}}. A pesar de que este exótico tipo de materia es un fuerte campo de estudio en la actualidad, los primeros indicadores de su existencia son ya casi centenarios \cite{Zwicky:1933gu}. No obstante, las primeras pruebas sólidas se las debemos a los trabajos de Vera Cooper Rubin, Kent Ford y Ken Freeman, llevados a cabo allá por los años 60 \cite{1970ApJ...159..379R,1970ApJ...160..811F}.

A pesar de los grandes exitos cosechados por el Modelo Estándar, hoy sabemos que no es, ni mucho menos, el final de la física de partículas. La que aparentemente era la conclusión de la física de altas energías, únicamente es capaz de explicar un porcentaje muy pequeño de la materia del Universo, el resto sigue siendo un misterio. Las observaciones astrofísicas y cosmológicas más recientes \cite{Aghanim:2018eyx} nos indican que el $26\%$ del contenido de energía del Universo es un nuevo tipo de materia, conocida como Materia Oscura\footnote{Su nombre se debe a que no emite ni refleja ningún tipo de luz.}. A pesar de que este exótico tipo de materia es un fuerte campo de estudio en la actualidad, los primeros indicadores de su existencia son ya casi centenarios \cite{Zwicky:1933gu}. No obstante, las primeras pruebas sólidas se las debemos a los trabajos de Vera Cooper Rubin, Kent Ford y Ken Freeman, llevados a cabo allá por los años 60 \cite{1970ApJ...159..379R,1970ApJ...160..811F}.

\subsection{Evidencias de la Existencia de Materia Oscura}
\label{sec:res:evidencias}

La evidencia más clara que tenemos a día de hoy de la existencia de la Materia Oscura son las curvas de rotación de las galaxias. El contenido en masa de una galaxia puede medirse en base a su luminosidad, mediante técnicas astrofísicas. De este modo, tenemos una clara idea de cuanta materia bariónica hay en una determinada galaxia y como está distribuida dentro de ella. Conocida la masa de la galaxia, la velocidad de rotación de un objeto situado a una distancia $R$ del centro de la misma puede determinarse a partir de las leyes de Kepler\footnote{$v = \sqrt{MG/R}$, donde $M$ es la masa contenida en la esfera de radio $R$ y $G$ la constante de gravitación universal.}. De acuerdo con esto, la distribución de materia bariónica observada nos indica que la velocidad de rotación debería disminuir conforme nos acercamos al borde galáctico. Sin embargo, medidas directas sobre la velocidad de rotación indican lo contrario: en la mayoría de los casos esta velocidad de rotación permanece constante.

Las curvas de rotación de las galaxias son la evidencia más famosa de la existencia de este exótico tipo de materia, pero no la única. La teoría de la Relatividad General predice que el campo gravitatorio producido por un gran cúmulo de materia es capaz de desviar los rayos de luz, el conocido como efecto \textit{lente gravitatoria}. De este modo, puede utilizarse la luz procedente de galaxias lejanas para, mediante ciertos estudios sobre la trayectoria de los haces de luz, determinar la cantidad de materia que hay en los cúmulos de galaxias situados en su trayectoria. Este análisis confirma la presencia de Materia Oscura en la mayoría de cúmulos de galaxias estudiados.

Aparte de las evidencias astrofísicas, hay muchas otras evidencias cosmológicas que confirman la existencia de la Materia Oscura. En la Sec.~\ref{sec:evidences} se ha realizado una breve descripción de todas ellas.

\subsection{Características Fundamentales}

A pesar de las evidencias de su existencia, a día de hoy aún no se ha realizado ninguna observación directa de la Materia Oscura. No obstante, podemos inferir mucho acerca de su naturaleza:
\begin{itemize}
\item La Materia Oscura debe ser no bariónica: algunos candidatos bariónicos han sido propuestos a lo largo de los años, como es el caso de los MACHOs\footnote{Del inglés \textit{Massive Compact Halo Objects}.} \cite{1986ApJ...304....1P}. No obstante, los límites sobre esta clase de modelos son tan fuertes en la actualidad que están prácticamente descartados en su totalidad.
\item Debe ser \textit{fría} o \textit{cálida}: según la distancia recorrida, como consecuencia de movimientos aleatorios, por las partículas de Materia Oscura en el Universo primigenio, podemos catalogarla en tres grandes grupos: \textit{calinte}, \textit{cálida} y \textit{fría}. Si la distancia recorrida es mayor, igual o menor que el tamaño de una protogalaxia \miguel{(unos 100 años luz)}, la Materia Oscura será caliente, cálida o fría, respectivamente. En la actualidad se han realizado numerosas simulaciones numéricas de la evolución del Universo con diferentes tipos de materia. Si la Materia Oscura fuese caliente, de acuerdo con estas simulaciones, el Universo tendría un aspecto muy diferente al que conocemos hoy en día \cite{primack2001happened}.
\item Debe colisionar muy débilmente consigo misma: el motivo de esto es que recientes observaciones astrofísicas, tales como las realizadas sobre el conocido como \textit{cúmulo bala}\footnote{Este curioso cúmulo es el resultado de dos cúmulos actualmente en colisión. En él se observa un efecto muy exótico, el centro de masas del cúmulo resultante se encuentra desplazado. Esta característica solo puede ser explicada mediante la existencia de grandes cantidades de Materia Oscura en su composición. La alternativa requeriría una modificación de las leyes más fundamentales de la dinámica relativista.}, imponen restricciones a la autointeracción de la Materia Oscura \cite{Dave_2001,Feng_2009,Agrawal_2017,Randall_2008,Kahlhoefer_2013}:
\be
\sigma/m \lesssim 10^{-24} \, \text{cm}^2/\text{GeV} .
\ee
\item Débilmente interactiva con la materia bariónica: \miguel{aparte de la interacción gravitatoria, la única interacción posible que podría llegar a tener la Materia Oscura es la débil. Respecto a lo que al electromagnetismo se refiere, las diversas implicaciones que supone la existencia de Materia Oscura cargada han sido profundamente estudiadas en la literatura \cite{DERUJULA1990173}, descartando prácticamente esta opción por motivos experimentales\footnote{En la actualidad las técnicas de detección de partículas cargadas son tan avanzadas que de existir la Materia Oscura eléctricamente cargada, esta ya debería haber sido observada.} \cite{Taoso:2007qk}.
Por otro lado, de existir la Materia Oscura fuertemente interactiva\footnote{Fuertemente en el sentido de interacción a través de la interacción fuerte.}, ésta dejaría huella incluso en el flujo de calor terrestre \cite{Mack:2007xj}. Las fuertes implicaciones de este tipo de candidatos hacen que esten excluidos casi en su totalidad.}
\item Debe ser estable: la Materia Oscura que observamos hoy en día en el Universo es prácticamente un fósil térmico: es el remanente de la que la que componía el Universo primigenio. La única forma de que ese remanente haya sobrevivido hasta nuestros días es que la Materia Oscura sea estable o, en su defecto, que su vida media sea mayor que la edad del Universo.
\end{itemize}

En la Sec.~\ref{sec:Properties} se ha realizado un estudio mucho más profundo de todas estas propiedades.

\subsection{Candidatos Estudiados}

Hasta el momento hemos hablado de las diferentes evidencias y características de la Materia Oscura. Pero ¿cuál es su naturaleza? En el escenario científico actual se han propuesto muchos candidatos a Materia Oscura, desde todo tipo de partículas con interacciones parecidas a las que ya conocemos, hasta candidatos altamente exóticos como agujeros negros primigenios \cite{10.1093/mnras/168.2.399,1975ApJ...201....1C,10.1093/mnras/152.1.75}. Todo esto ha sido detallado en la Sec.~\ref{sec:candidates}. En este resumen únicamente hablaremos sobre los dos candidatos estudiados en esta Tesis: las partículas WIMP \cite{PhysRevLett.39.165} y las FIMP \cite{Hall:2009bx}.

\subsubsection{Materia Oscura tipo WIMP}

Las partículas WIMP\footnote{Su nombre deriva del inglés \textit{Weakly Interactive Massive Particles}, es decir, partículas masivas débilmente interactivas.} son partículas con masas típicamente desde el GeV hasta varios TeV. Este candidato se basa en la suposición de que las partículas de Materia Oscura se encontraban en equilibrio térmico con el resto de partículas del Modelo Estándar en el Universo primigenio. La abundancia que observamos en la actualidad sería pues el resultado de un proceso denominado \textit{freeze-out}.

Para entender bien el concepto de \textit{freeze-out}, debemos remontarnos a los primeros instantes del Universo, justo después del Big Bang. En aquella época, los átomos no existían, las diferentes partículas que poblaban el Universo se encontraban en un equilibrio continuo de aniquilación/producción, formando un plasma de altísima temperatura. Poco a poco, el Universo fue expandiéndose, enfriando dicho plasma. El enfriamiento del Universo provocó que algunos de los procesos que mantenían este equilibrio dejasen de tener lugar, desacoplando de este modo las diferentes especies de partículas de este \textit{caldo} primigenio.

Cuando la temperatura del Universo fue demasiado baja como para que la creación de partículas de Materia Oscura fuese posible, está se desacopló del \textit{caldo} primigenio. Como consecuencia, la abundancia de estas partículas comenzó a disminuir, hasta que fue tan pequeña que la probabilidad de que dos partículas de Materia Oscura se encontrasen y se aniquilasen se volvió prácticamente nula. A dicha temperatura, conocida como temperatura de \textit{freeze-out}, la abundancia de Materia Oscura superviviente se convirtió en un leve remanente, un mero fósil térmico, que ha llegado hasta nuestros días.

Este candidato a Materia Oscura ha gozado de gran acogida por los físicos teóricos desde que fuese propuesto alla por los años 70. El motivo de tal popularidad es que en el rango de masas mencionado, curiosamente, para reproducir la abundancia de Materia Oscura actual, se necesita que la interacción entre ésta y las partículas del Modelo Estándar sea justo del orden de la interacción electrodébil. Hecho, cuanto menos sorprendente, que se conoce como \textit{Milagro WIMP}. En este rango de masas la sección eficaz necesaria para conseguir dicha abundancia es prácticamente independiente del valor de la masa de la partícula WIMP,
\be
\langle \sigma v \rangle \backsimeq 2 \times 10^{-26}\, \text{cm}^3/\text{s} \backsim 1 \, \text{pb} \, .
\ee
Los detalles matemáticos y técnicos de este candidato a Materia Oscura se encuentran explicados en la Sec.~\ref{Sec:freezeout}.

\subsubsection{Materia Oscura tipo FIMP}

Complementariamente al caso WIMP, existe la Materia Oscura tipo FIMP\footnote{Nombre que deriva del ingles \textit{Feebly Interactive Massive Particle}.} la cual jamás llegó al equilibrio térmico con el resto de partículas del Modelo Estándar. En este escenario la Materia Oscura fue producida por diversos procesos durante la época de enfriamiento del Universo, después del Big Bang, siendo nula en el origen de los tiempos. Cuando la temperatura del Universo fue suficientemente baja, esta producción se congeló, dejando un remanente que ha llegado hasta nuestros días. Este mecanismo de producción recibe el nombre de \textit{freeze-in}\footnote{El mecanismo de producción fue propuesto en Ref.~\cite{Chung:1998rq}. Aunque en aquella época ni el mecanismo se conocía por dicho nombre, ni el candidato como FIMP.} y está detallado en la Sec.~\ref{Sec:freezein}.

\miguel{La Materia Oscura FIMP no ha llegado a alcanzar la popularidad de la Materia Oscura tipo WIMP. Hay varios motivos para ello pero el principal es que debido a su baja intensidad de interacción es muy dificil buscar pruebas experimentales de su existencia.}

\section{Detección de Materia Oscura}

Como hemos comentado en la Sec.~\ref{sec:evidences}, y resumido en Sec.~\ref{sec:res:evidencias}, tenemos muchas evidencias de la existencia de a Materia Oscura. No obstante, no se ha conseguido realizar ninguna observación directa de estas elusivas partículas\footnote{Existe una llamativa excepción: el experimento DAMA/Libra ha medido variaciones en la modulación solar que pueden ser interpretadas como Materia Oscura \cite{Bernabei:2008yi,Bernabei:2010mq}. No obstante, esta señal no está libre de controversia entre la comunidad científica ya que ningún otro experimento ha reportado absolutamente nada en el rango de masas en el que DAMA/Libra mide dicha señal.}. A pesar de esto, las técnicas de detección de Materia Oscura han avanzado mucho en los últimos años, poniendo cotas cada vez más restrictivas a la existencia de estas partículas aparentemente invisibles.
Dentro del gran abanico de experimentos de detección, estos pueden clasificarse en dos grandes grupos: la \textit{Detección Directa}\footnote{Del ingles \textit{Direct Detection.}} DD y la \textit{Deteccion Indirecta}\footnote{Del ingles \textit{Indirect Detection.}} ID.

\subsection{Detección Directa}

La idea de la Detección Directa (cuyos detalles técnicos se discuten en profundidad en la Sec.~\ref{Sec:DD}) fue propuesta por primera vez por Mark Goodman y Edward Witten \cite{Goodman:1984dc}. Como la Materia Oscura no presenta cargas eléctricas, es imposible detectarla mediante técnicas electromagnéticas. No obstante, la existencia de colisiones entre la DM y los núcleos atómicos abre una puerta para su observación directa. 

En general, esta clase de detecciones se realizan en experimentos ubicados bajo tierra. Ejemplos notables son Xenon1T \cite{PhysRevLett.121.111302} o LUX \cite{Akerib:2016vxi}, los cuales están compuestos por grandes cantidades de Xenón. La colisión de la Materia Oscura con los átomos de Xenón produciría una excitación de estos últimos, que finalmente se traduciría en la emisión de un fotón. Hasta el momento, no se ha realizado ninguna detección en dichos experimentos, lo cual pone fuertes límites sobre los modelos de Materia Oscura, haciendo que los escenarios más simples y \textit{naturales} estén prácticamente descartados.

\begin{figure}[htbp]
\centering
\includegraphics[width=130mm]{figures/direct_detection_bounds.pdf}
\caption[Estatus actual de los experimentos de detección directa.]{\it Límites actuales a la sección eficaz de interacción de Materia Oscura con nucleones. La región verde está excluida por los experimentos de Detección Directa con un 90\% de intervalo de confianza. Las dos zonas rojas muestran las regiones en las que DAMA/LIBRA afirma haber observado Materia Oscura. La zona amarilla representa el \textit{suelo  de neutrinos} \cite{Billard:2013qya}.}
 \label{fig:direct_detection_bounds_resumen}
\end{figure}

Uno puede hacerse una idea del panorama actual de estos experimentos mirando la Fig.~\ref{fig:direct_detection_bounds_resumen}. En ella, la zona verde muestra los valores de la sección eficaz de Detección Directa, como función de la masa de la Materia Oscura, que ya han sido descartados por los experimentos. Por otro lado, para hacernos una idea de magnitud de la zona ya eliminada, podemos mirar lo cerca que se encuentra de ella la región amarilla. Esta región muestra lo que se conoce como \textit{suelo de neutrinos}\footnote{En ingles conocido como \textit{neutrino floor}.} \cite{Billard:2013qya} y representa \miguel{la sección eficaz} para la que los experimentos de detección comenzarán a observar colisiones producidas por los neutrinos. Realizar exclusiones mediante experimentos de Detección Directa en esta región es complicado, puesto que la señal de ambos tipos de colisión es indistinta. Las dos regiones rojas muestran las observaciones de DAMA/LIBRA en zonas totalmente excluidas por el resto de experimentos.

\subsection{Detección Indirecta}

La observación directa de las colisiones de las partículas de Materia Oscura con los núcleos atómicos no es la única técnica para detectarla. Diferentes experimentos astronómicos llevan años intentando observar los posibles productos de las aniquilaciones de las partículas de Materia Oscura en los rayos cósmicos que nos llegan a la Tierra. Es posible distinguir entre tres tipos de flujos de partículas: fotones, neutrinos y partículas cargadas (como electrones, positrones, etc).

En general, de los diferentes flujos de partículas que llegan a la Tierra, los resultados más prometedores (en lo que a Materia Oscura se refiere) vienen de los fotones. Desde 2008 la colaboración Fermi-LAT analiza el flujo de fotones procedente de diferentes \textit{galaxias enanas} \cite{Fermi-LAT:2016uux,Ackermann:2015zua}. Hasta el momento el estudio se restringe a 15 ejemplares y por el momento los resultados no muestran ningún exceso en el flujo analizado que no pueda ser explicado por el Modelo Estándar de partículas. Esto pone cotas a modelos de nueva física en los cuales la Materia Oscura pueda aniquilarse a partículas que finalmente se desintegren en fotones, generalmente en el rango de masas $m_{\text{DM}} \in (0.5,500) $ GeV. No obstante, desde 2009 el mismo experimento ha estado reportando un exceso inexplicable de fotones procedente del centro galáctico\footnote{Popularmente conocido como \textit{Galactic Center $\gamma$-ray excess} (GCE) \cite{Goodenough:2009gk, Vitale:2009hr, Hooper:2010mq, Gordon:2013vta, Hooper:2011ti, Daylan:2014rsa, 2011PhLB..705..165B, Calore:2014xka, Abazajian:2014fta,Zhou:2014lva}.}. Aunque su origen aún es desconocido, este exceso, que se observa a una energía $\sim 3$ GeV, puede ser explicado por diferentes modelos de Materia Oscura.

Por otro lado, las señales procedentes de flujos de antipartículas cargadas acotan de una forma mucho menos restrictiva los modelos de Materia Oscura. El problema con esta clase de flujos es su propagación desde el punto en el que son generados hasta la Tierra (donde finalmente los detectamos). Hoy en día existen diversos modelos para ello, pero su precisión aún tiene que ser perfeccionada para que los límites impuestos por esta clase de flujos sean realmente restrictivos.

En la Sec.~\ref{Sec:ID} se ha realizado un análisis exhaustivo de la Detección Indirecta de Materia Oscura.

\section{Dimensiones Extra}

\miguel{De entre las cuatro fuerzas fundamentales de la naturaleza, no cabe ninguna duda de que la gravedad es la más complicada de entender a nivel cuántico. A pesar de los muchos esfuerzos por parte de la comunidad científica, aún no tenemos una teoría cuántica para describirla.
Por otro lado, la gravedad es la más débil de las interacciones fundamentales. Tal es el caso, que de existir nueva física a la escala gravitatoria, el Modelo Estándar se enfrentaría a un serio problema}: las correcciones a la masa del bosón de Higgs son muy sensibles a la escala de la nueva física. Teniendo en cuenta la diferencia entre la escala de Planck\footnote{La escala de la interacción gravitatoria.} y la escala electrodébil, de aparecer nueva física a la escala gravitatoria las correcciones a la masa del Higgs serían enormes, entrando en serias inconsistencias matemáticas. A este fenómeno se le conoce como \textit{problema de la jerarquía} (para un analisis más detallado del problema mirar la Sec.~\ref{sec:hierarchyproblem}). Entre las diversas propuestas que se han realizado para intentar resolver este problema se encuentran las dimensiones extra.

\subsection{Dimensiones Extra \textit{Grandes} (LED)}

El primer modelo de dimensiones extra que se propuso para dar solución al problema de la jerarquía fue \textit{Large Extra-Dimensions} (LED) \cite{ArkaniHamed:1998rs}. En este escenario se asume que las nuevas dimensiones tienen una forma similar a las tres espaciales ya conocidas, es decir, presentarían un aspecto plano. De acuerdo con el modelo LED, el tamaño de estas nuevas dimensiones sería finito o, en otras palabras, estarían compactificadas. Por otro lado, mientras que la gravedad se propaga libremente por el espacio 5-dimensional, el resto de campos del Modelo Estándar se encuentran confinados en unas hipersuperficies 4-dimensionales denominadas \textit{branas}. Este hecho hace que la gravedad se diluya a través de las dimensiones extra, haciendo que en la brana (donde nosotros vivimos confinados) su intensidad parezca anómalamente débil. De este modo, la escala de la gravitación, que para nosotros es $M_\text{P} = 1.22 \times 10^{19}$ GeV, en el espacio extra-dimensional completo sería $M_D$. \miguel{Ambas escalas están relacionadas a través del radio de compactificación de las dimensiones extra ($r_c$):
\be
M_\text{P}^2 = M_{D}^{D-2} (2\pi r_c)^D.
\ee 
}

Para el caso particular de 5 dimensiones, el espacio-tiempo queda definido en este modelo por la métrica:
\be
ds^2 = \eta_{\mu \nu}dx^\mu dx^\nu + r_c^2dy^2,
\ee
Donde la dimensión extra está representada por $y$. Este parámetro puede escogerse de manera que $M_5 \backsim \text{TeV}$, resolviendo así el problema de la jerarquía.
No obstante, si imponemos esta condición, el modelo LED 5-dimensional está excluido totalmente a día de hoy: agregar una única dimensión extra en LED predice correcciones de la ley de la gravitación universal que podrían observarse en distancias parecidas al tamaño del Sistema Solar. \miguel{No obstante, aunque el modelo esté excluido para una única dimensión extra, con dos o más dimensiones es posible resolver el problema de la jerarquía sin entrar en contradicciones con la ley de la gravitación universal.}

\subsection{Dimensiones Extra Deformadas: Modelo de Randall-Sundrum}

A pesar de que los modelos LED presentan diversos problemas, pusieron la semilla para modelos futuros muy interesantes. El caso más popular es el modelo propuesto por Lisa Randall y Raman Sundrum a finales de los años 90, conocido como \textit{dimensiones extra deformadas} o \textit{modelo de Randall-Sundrum} (RS) \cite{Randall:1999ee}. En dicho modelo, las nuevas dimensiones presentan curvatura, a diferencia de LED, donde eran planas. En el modelo original de RS el espacio extra-dimensional está delimitado por dos branas. Todos los campos de materia viven atrapados en una de ellas (brana \textit{infrarroja} (IR), también llamada brana del TeV), mientras que la otra brana se encuentra vacía (brana \textit{ultravioleta} (UV) o de Planck). Por otro lado, la gravedad se propaga libremente por el espacio extra-dimensional (comúnmente conocido como \textit{bulk}). La geometría del modelo hace que los diferentes parámetros fundamentales con dimensión de masa sufran un proceso de deformación exponencial a lo largo del bulk, resolviendo así el problema de la jerarquía.

Concretamente, para el caso 5-dimensional (una única dimensión extra), la métrica que definiría este espacio tiempo vendría dada por
\be
ds^2 = e^{-2  kR|y|}\eta_{\mu \nu} dx^\mu dx^\nu - r_c^2 dy \, ,
\label{RS_metric_resumen}
\ee
Donde $k$ es la curvatura a lo largo de la dimensión extra y $r_c$ su radio de compactificación. El factor exponencial que multiplica la parte 4-dimensional de la métrica recibe el nombre de factor de deformación.
$M_5$ y $M_\text{P}$ quedarían entonces relacionados mediante los dos parámetros libres de la teoría:
\be
\bar{M_\text{P}}^2 = \frac{M_5}{k} \left( 1 - e^{-2 k \pi r_c} \right) \, .
\ee
Vemos que hay una clara diferencia con el modelo LED: en RS $M_5\backsimeq M_\text{P}$. Sin embargo, la modificación que sufren los parámetros medidos en la brana IR, debido a la presencia del factor de deformación, resuelve el problema de la jerarquía para $k\,r_c \backsim 10 $.

\miguel{En RS la gravedad puede describirse a través del intercambio de gravitones no masivos 5-dimensionales, los cuales surgen de perturbaciones sobre la componente 4-dimensional de la métrica
\be
G^{(4)}_{\mu \nu} = e^{-2kr_c|y|} (\eta_{\mu \nu} + 2M_5^{-2/3} h_{\mu \nu}) \, .
\label{perturbacion_4dim}
\ee
No obstante, la proyección de este campo 5-dimensional sobre las branas es equivalente a una torre de gravitones 4-dimensionales masivos, comúnmente conocidos como modos de Kaluza-Klein (KK). La escala efectiva de la interacción de estos gravitones 4-dimensionales con los campos confinados en la brana IR viene dada por
\be
\Lambda \equiv \bar{M_\text{P}} e^{-k \pi r_c} \, .
\ee
Por otro lado, cada gravitón de esta torre de partículas tiene una masa diferente que dependerá de los parámetros libres ($k,r_c$) del modelo y de su respectivo orden dentro de la torre. No obstante, establecida la masa del primer gravitón $m_1$, la masa del resto de gravitones queda totalmente fijada. La fenomenología de los modelos de RS puede ser descrita mediante los parámetros ($\Lambda,m_1$), en lugar de ($k,r_c$). Este hecho puede ser muy útil debido a su relación con observables fenomenológicos.}

\miguel{El modelo asume que la distancia entre las branas está fijada, no obstante, no aporta ningún mecanismo para estabilizar este parámetro dinámicamente. La solución a este problema fue propuesta por Walter D. Goldberger y Mark B. Wise \cite{Goldberger:1999wh,Goldberger:1999uk}. Este mecanismo utiliza un nuevo campo escalar que se propaga libremente por el \textit{bulk}, induciendo unos potenciales localizados en las branas. Los mínimos de estos potenciales en la brana IR y UV son diferentes, lo que genera un valor esperado de vacío para este nuevo campo escalar. El tamaño de la quinta dimensión ($r_c$) está entonces relacionado con este valor esperado de vacio.
Por otro lado, el nuevo campo escalar se mezcla con el ya presente en el \textit{bulk}, el graviescalar $G_{55}^{(5)}$ (el cual emerge de las perturbaciones sobre la parte 5-dimensional de la métrica). Al campo resultante de esta mezcla se le conoce como radión. La masa de este nuevo campo no está determianda por el modelo y representa un nuevo grado de libertad.}

El modelo de RS ha gozado de gran popularidad desde que fue propuesto a finales de los 90's. La literatura sobre modelos de física más allá del Modelo Estándar desarrollados en este escenario es inmensa. En la Sec.~\ref{sc:warped} se ha realizado un análisis de los detalles técnicos del modelo.  

\subsection{Dimensiones extra tipo \textit{Clockwork/Linear Dilaton}}

\miguel{Durante casi dos decadas lo modelos de RS fueron los únicos que resolvian el problema de la jerarquía mediante la introducción de dimensiones con curvatura. No obstante, en 2016 Gian Giudice y Matthew McCullough propusieron un nuevo modelo de dimensiones extra curvadas. Este nuevo modelo, propuesto en Ref.~\cite{Giudice:2016yja} y cuya fenomenología fue estudiada en Ref.~\cite{Giudice:2017fmj}, se conoce con el nombre de \textit{Clockwork/Linear Dilaton} (CW/LD).}

\miguel{Este modelo, que fue encontrado como límite continuo de los modelos \textit{Clockwork} discretos, puede caracterizarse a traves de la métrica:
\be
\label{eq:5dmetric_resumen}
ds^2 = e^{4/3 k r_c |y|} \left ( \eta_{\mu \nu} dx^{\mu}dx^{\nu} - r_c^2 \, dy^2 \right ) \, ,
\ee
donde $k$ y $r_c$ representan la curvatura y el radio de compactificación de la quinta dimensión, respectivamente. Para determinados valores de los parámetros libres, el modelo es capaz de resolver el problema de la jerarquía.}

El modelo CW/LD guarda ciertas similitudes con RS. En ambos casos el espacio 5-dimensional está delimitado por las branas IR y UV. El caso mínimo implica tener todo el Modelos Estándar confinado en la brana IR, mientras que la gravedad se propaga libremente por el bulk 5-dimensional. Sin embargo, hay diferencias notables con RS. En primer lugar, la relación entre $M_5$ y $M_\text{P}$ en CW/LD viene dada por
\be
M_{\text{P}}^2 = \frac{M_5^3}{k} \left ( e^{2 \pi r_c}  - 1 \right ) \, ,
\ee 
pudiendo ser esta del orden del TeV (al igual que en el caso LED). Por otro lado, el acoplamiento de \miguel{los gravitones de KK} a las partículas localizadas en la brana es diferente para cada gravitón:
\be
\dfrac{1}{\Lambda_{n}} =  \dfrac{1}{\sqrt{M_5^3 \pi r_c}}  \left ( 1 + \dfrac{k^2 r_c^2}{n^2} \right )^{-1/2} 
=  \dfrac{1}{\sqrt{M_5^3 \pi r_c}} \left ( 1 - \dfrac{k^2}{m_n^2} \right )^{1/2}  \,  .
\ee
Este hecho hace que describir la fenomenología en base a $\Lambda_n$ no sea tan útil como en RS. Otra diferencia notable es que hay una relación muy interesante entre el valor de la curvatura $k$ y la masa del primer gravitón $m_1$, haciendo que ambos parámetros sean prácticamente idénticos.

\miguel{En el caso CW/LD, el tamaño de la quinta dimension puede estabilizarse sin necesidad de introducir ningún nuevo campo. La forma del modelo genera unos potenciales en las branas IR y UV a traves del campo de dilatación (\textit{dilaton}), $S = 2 k r_c |y|$, de la métrica. Esto permite fijar la posición de las branas de un modo similar a como se hacía en RS.}

\section{Metodología Utilizada}

Antes de ponernos a hablar sobre los cuatro proyectos que conforman la presente Tesis, es necesario comentar las diferentes técnicas (tanto a nivel analítico como numérico) utilizadas en el desarrollo de los mismos. 

A nivel analítico, la complejidad de los problemas estudiados ha requerido un profundo conocimiento de la teoría cuántica de campos. Se han utilizado los desarrollos perturbativos de dicha teoría para obtener las diferentes probabilidades de interacción utilizadas posteriormente en los estudios fenomenológicos. Los modelos aquí estudiados asumen Materia Oscura tipo WIMP y FIMP. En ambos casos, la evolución de la abundancia de Materia Oscura a lo largo de la historia térmica del Universo requiere resolver la Ecuación de Boltzman, que determina la evolución de sistemas fuera del equilibrio térmico. Por otro lado, se ha trabajado con dos modelos de dimensiones extra:  Randall-Sundrum y Clockwork/Linear Dilatón. La fenomenología estudiada sobre estos modelos ha requerido un análisis exhaustivo de ambos escenarios.

Desde un punto de vista numérico, toda la fenomenología ha sido estudiada mediante lenguaje \textit{C++}, mientras que su representación a nivel gráfico ha sido obtenida utilizando \textit{python}. El análisis de la Detección Indirecta de Materia Oscura realizado en uno de los modelos estudiados ha requerido el uso de software más específico: \textit{micrOMEGAs}, \textit{SARAH}, \textit{gamlike}, \textit{pythia} y \textit{MadGraph}. Por otro lado, todo el estudio de la Ecuación de Boltzman en los cuatro modelos se ha realizado mediante métodos numéricos implementados en lenguaje \textit{C++}.

Finalmente, el enfoque fenomenológico que presenta esta Tesis ha implicado un contacto continuo con datos experimentales. El tratamiento de estos datos, así como las diferentes cotas de exclusión que han puesto sobre los diferentes modelos estudiados, ha requerido un uso de diversas técnicas estadísticas. Se han utilizado diferentes distribuciones de probabilidad (tales como la conocida $\chi^2$), técnicas de Monte Carlo, etc.

\section{Resultados y conclusiones de la Tesis}

En está sección, vamos a realizar un breve resumen de los proyectos que conforman esta Tesis. Todos ellos pueden encontrarse completos en la Parte \ref{sec:papers}.

\subsection{Estudio de la Detección Indirecta del Modelo de \textit{Portal de Neutrinos Estériles}}

Uno de los grandes problemas abiertos en física de altas energías es la Materia Oscura, pero desde luego no es el único. Entre los diversos problemas que existen actualmente en el Modelo Estándar de partículas, uno de los más importantes es la masa de los neutrinos. El modelo predice una masa nula para ellos, no obstante, hace ya más de medio siglo se predijo un efecto denominado \textit{oscilaciones de neutrinos} \cite{Pontecorvo:1957cp}. Este curioso fenómeno, que fue confirmado experimentalmente en 1999 \cite{Fukuda:1998mi}, consiste en una oscilación en el sabor leptónico de los neutrinos. Las implicaciones de este hecho son muy profundas ya que únicamente puede suceder si al menos uno de los tres sabores de neutrinos es masivo\footnote{\miguel{A pesar de que el fenómeno podría explicarse con un solo neutrino masivo, la observación del fenomeno tanto en neutrinos atmosfericos como solares requiere que al menos dos de los tres sabores de neutrinos sean masivos.}}. No obstante, las cotas experimentales impuestas a la masa de estas partículas prácticamente invisibles son tan fuertes que su masa debe ser muy pequeña\footnote{El límite actual más fuerte viene dado por el experimento \textit{Karlsruhe Tritio Neutrino} (KATRIN) \cite{Aker:2019uuj}.}.
Este hecho potenció el desarrollo de modelos en los que la masa de los neutrinos era generada por mecanismos de tipo \textit{balancín}\footnote{Modelo \textit{seesaw} en inglés.} \cite{GellMann:1980vs,PhysRevLett.44.912,Yanagida:1979as,Glashow1111,MINKOWSKI1977421}. Hay diferentes versiones de estos modelos, en el \textit{tipo I}, por ejemplo, se asume la existencia de neutrinos dextrógiros muy masivos que justifican la pequeña masa de los neutrinos del Modelo Estándar. La mezcla de los neutrinos levógiros con los dextrogiros da como resultado los autoestados de masa, prediciendo neutrinos con masas muy grandes y muy pequeñas.

La posibilidad de que el problema de la Materia Oscura y de la masa de los neutrinos estén relacionados motivó el desarrollo del conocido como\footnote{El escenario más económico, la posibilidad de que los neutrinos estériles sean la Materia Oscura, fue propuesto en Ref.~\cite{Dodelson:1993je}. A día de hoy, esta posibilidad ha sido fuertemente estudiada y prácticamente descartada \cite{Adhikari:2016bei}.} \textit{portal de neutrinos estériles a Materia Oscura} \cite{Escudero:2016tzx,Macias:2015cna,Escudero:2016ksa}. Este modelo se ha estudiado por diversos autores, acotándolo utilizando la Detección Directa de Materia Oscura. No obstante, es un modelo muy interesante desde el punto de vista de la Detección Indirecta por varios motivos. Por un lado, la Detección Directa en este escenario no sucede al orden más bajo en teoría de perturbaciones de la teoría cuántica de campos. Este hecho hace que sus señales de Detección Directa sean bajas que en otros modelos, empeorando así los límites impuestos. Por otro lado, la conexión de los neutrinos estériles con los neutrinos activos hace que las aniquilaciones de Materia Oscura produzcan, como resultado de diversas desintegraciones, excesos de fotones y partículas cargadas. Todo esto lo convierte en el candidato perfecto para ser estudiado desde el punto de vista de la Detección Indirecta, tal como se ha llevado a cabo en la Ref.~\cite{Folgado:2018qlv}.

En este trabajo hemos analizado un modelo particular en el que, además de los neutrinos estériles, se asume la existencia de dos nuevos campos: uno escalar $\phi$ y otro fermionico $\Psi$. Estos campos son ambos singletes del Modelo Estándar, no obstante, están cargados respecto a un nuevo grupo de simetría, $G_{\text{dark}}$, de tal forma que la combinación $ \overline{\Psi} \phi$ es singlete de este nuevo grupo de simetría.

\begin{figure}[htbp]
\centering
\includegraphics[width=120mm]{figures/resultados_paper_1.pdf}
\caption[Resultados del primer articulo.]{\it Límites sobre el \textit{portal de neutrinos estériles} en el espacio de masas. La región amarilla muestra los límites impuestos por los antiprotones mientras que la región azul son los límites impuestos por los fotones procedentes de las galaxias enanas. Los diferentes contornos muestran la zona en la que el modelo es capaz de reproducir el GCE. La línea discontinua azul muestra nuestra predicción sobre el límite de las galaxias enanas para los próximos 15 años.}
 \label{fig:resultados_paper_1}
\end{figure}

La más ligera de estas nuevas partículas \textit{oscuras} ($\phi$ y $\Psi$) es estable si todas las particulas del Modelo Estándar, así como los neutrinos esteriles, son singletes de $G_{\text{dark}}$, independientemente de la naturaleza de este grupo de simetría. Como consecuencia, debido a su estabilidad esta partícula es un buen candidato a Materia Oscura. Por simplicidad, asumimos que $G_{\text{dark}}$ es una simetría global a baja enería, en cualquier caso no esperamos cambios significantes en nuestro analisis fenomenológico si esta fuese local.

Los terminos más relevantes en el lagrangiano vienen dados por:
\bea
\mathcal{L} &=& \mu_H^2 H^\dagger H - \lambda_H (H^\dagger H)^2  -
\mu_\phi^2 \phi^\dagger \phi - \lambda_\phi (\phi^\dagger \phi)^2 - 
\lambda_{H\phi} (H^\dagger H) \, (\phi^\dagger \phi)   
\nonumber \\
&-&\left( \phi \overline{\Psi}(  \lambda_a +  \lambda_p \gamma_5) N 
 + Y \overline {L}_L H N_{R}  + {\rm h.c.}  \right)  \, .
\eea

Los acoplamientos de Yukawa $Y$ entre los neutrinos dextrógiros $N_R$ y el doblete leptónico del Modelo Estándar genera las masas para los neutrinos activos después de la ruptura espontanea de la simetría, a traves del mecanismo \textit{balancín} de tipo I. Si bien se requieren al menos dos neutrinos estériles para generar las masas de neutrinos observadas en las oscilaciones, en nuestro análisis consideramos que solo una especie es más ligera que la Materia Oscura y, por lo tanto, relevante para la determinación de su abundancia y búsquedas indirectas. No obstante, los resultados son fáclmtente extendibles al caso en el que tenemos dos o más neutrinos estériles más ligeros que la Materia Oscura. Bajo el supuesto de que la Materia Oscura es descrita por $\Psi$ (el análisis es igualmente valido en el caso de que la Materia Oscura sea $\phi$) las masas del modelo cumplen la relación $m_N < m_\Psi < m_\phi$.

La Fig.~\ref{fig:resultados_paper_1} muestra los resultados finales de nuestro análisis. Fijando la masa del mediador escalar para obtener la abundancia de Materia Oscura mediante el mecanismo \textit{freeze-out} (es decir $\langle \sigma \, v \rangle \sim 2 \times 10^{-26} cm^3/s$), la figura muestra los diferentes limites impuestos por las busquedas de fotones y antiprotones en el espacio de masas $(M_N,M_\Psi)$. Como ya hemos comentado, el experimento Fermi-LAT ha reportado un exceso de fotones inexplicable procedente del centro galáctico (GCE). El modelo estudiado predice un pequeño exceso de fotones que podría ser compatible con el GCE en ciertas zonas del espacio de parámetros. La zona en la que esto ocurre está delimitada por los diferentes contornos que se observan en la figura (en la leyenda está indicado el p-valor asociado a cada contorno). No obstante, este aumento de fotones predicho por el modelo tiene que ser compatible también con el resto de medidas realizadas sobre los diferentes flujos de fotones. En concreto, el mismo experimento realiza medidas sobre los fotones procedentes de 15 galaxias enanas\footnote{Galaxias compuesta por varios millones de estrellas. En contraposición tenemos las galaxias normales, compuestas por varios miles de millones.}, la región sombreada en azul muestra la zona del espacio de parámetros de la teoría en la cual los resultados obtenidos no son compatibles con dichas mediciones.

Por otro lado, el modelo también predice un aumento del flujo de antiprotones. Este aumento se ha comparado con el flujo de positrones procedente del centro galáctico, el cual es medido en la actualidad por el experimento AMS-02.Los resultados obtenidos muestran que existen zonas en las cuales las predicciones del modelo no serían compatibles con lo observado experimentalmente (zona sombreada en amarillo en la figura).
Por último, también se ha realizado un análisis del posible impacto de experimentos de Detección Indirecta futuros sobre el modelo. En concreto, se ha visto que la mejora en los datos del flujo procedente de las galaxias enanas, realizado por el experimento Fermi-LAT, podría poner fuertes cotas al modelo estudiado (línea azul discontinua).

\subsection{Materia Oscura Escalar Mediada por Gravedad en Dimensiones Extra Deformadas}

Todas las evidencias que tenemos hoy en día acerca de la existencia de la Materia Oscura están relacionadas únicamente con la interacción gravitatoria. Este hecho induce a pensar en la posibilidad de que las partículas de Materia Oscura únicamente interactúen gravitatoriamente. Esta idea tan natural ha sido explorada ya y presenta un serio problema: la intensidad de la interacción gravitatoria es muy débil y hace imposible obtener la cantidad de abundancia de Materia Oscura que se observa en la actualidad (al menos en el escenario WIMP). No obstante, ¿que ocurre si pensamos en más de 4 dimensiones? Esta es la idea que inspiró la Ref.~\cite{Folgado:2019sgz}.

En dicho artículo tratamos de explorar si es posible obtener la abundancia de Materia Oscura actual, asumiendo que es de tipo WIMP escalar, únicamente mediante interacción gravitatoria y bajo el supuesto de un Universo 5-dimensional de tipo Randall-Sundrum. En el escenario descrito, la Materia Oscura y el Modelo Estándar viven confinados en la brana infrarroja. Ambos tipos de materia interactúan únicamente a través de la gravedad, la cual se propaga por la brana en forma de gravitones 4-dimensionales masivos (describiendo una torre de Kaluza-Klein).

El modelo queda descrito en base a cuatro parámetros físicos: la escala de la interacción de los gravitones 4-dimensionales con la materia, $\Lambda$; la masa del primer gravitón de la torre de KK, $m_{1}$; la masa del candidato a Materia Oscura, $m_{\text{DM}}$ y la masa del radión, $m_r$. Nuestro estudio muestra que cuando $m_r < m_\text{DM}$ y, en consecuencia, el canal de aniquilación a radiones esta abierto, los resultados obtenidos son prácticamente independientes del valor de $m_r$. 
Respecto a la aniquilación de la Materia Oscura a partículas del Modelo Estandar a traves del intercambio de radiones virtuales, esta sección eficaz únicamente es relevante cerca de la resonancia $m_\text{DM} \backsim m_r/2$. Por tanto, en el estudio fenomenológico realizado hemos fijado la masa del radion y ns hemos centrado en el resto de parámetros libres del modelo.

El método seguido para el análisis del modelo ha sido la construcción de una malla bidimensional con diferentes valores de los parámetros $(m_{G_1},m_s)$. Para cada uno de los puntos de este mallado hemos buscado si existe algún valor de $\Lambda$ para el cual se obtiene la abundancia de Materia Oscura actual. De este modo, para cada punto del mallado los tres parámetros libres quedan totalmente definidos. Este análisis nos permite establecer diferentes límites teóricos y experimentales en el espacio de masas del modelo. 

\begin{figure}[t]
\centering
\includegraphics[width=150mm]{figures/resultados_paper_2.png}
\caption[Resultados del segundo articulo.]{\it Límites sobre Materia Oscura escalar puramente gravitatoria en RS. La gráfica de la izquierda muestra el caso sin radión, mientras que en la de la derecha se ha considerado $m_r = 100$ GeV. Las líneas discontinuas muestran los diferentes valores de $\Lambda$ en el plano ($m_\text{DM},m_{1}$) para los cuales se consigue la abundancia actual de Materia Oscura. La zona gris muestra la región en la cual es imposible conseguir la abundancia de Materia Oscura, independientemente del valor de $\Lambda$. Por otro lado, la región naranja nos indica los puntos en los que la abundancia se consigue gracias a los canales de interacción relacionados con el radión. Respecto a los límites sobre el modelo: la zona de cuadraditos verde representa el límite de unitariedad; la zona de cuadraditos rosa representa la zona en la que la teoría efectiva deja de tener validez; la zona roja representa los límites impuestos por el experimento Xenon1T sobre la sección eficaz de Detección Directa; la región azul representa los límites impuestos por las búsquedas de resonancias en el LHC. Finalmente, las líneas punteadas son las predicciones de exclusión para las fases \textit{Run-III} y \textit{High Luminosity} del LHC.}
 \label{fig:resultados_paper_2}
\end{figure}

En la Fig.~\ref{fig:resultados_paper_2} pueden verse los resultados finales del análisis fenomenológico sobre el modelo. En la parte izquierda se ha explorado el caso sin radión, asumiendo que podría encontrarse algún método alternativo para estabilizar el radio de la quinta dimensión. Por otro lado, en la parte derecha se ha considerado que la masa del radión es $m_r = 100$ GeV (es importante recordar que la fenomenología no se ve afectada por el valor de esta masa). La zona sombreada en gris es la región en la que no es posible obtener la abundancia actual de Materia Oscura para ningún valor de $\Lambda$, mientras que la zona naranja representa la región del espacio de parámetros en la que la abundancia se consigue gracias a las contribuciones de los canales de interacción radiónicos. La zona sombreada con cuadraditos verdes se conoce como límite de unitariedad y representa el punto a partir del cual la sección eficaz de interacción es tan alta que pone en peligro el desarrollo perturbativo de la teoría cuántica de campos. Además de este límite, existe otra restriccion teórica: si $\Lambda < m_{\text{DM}}, m_{1}$ la teoría efectiva que describe la interacción de estos campos cuánticos deja de tener sentido. Esto ocurre en la región de cuadraditos rosa.

Hasta el momento, hemos hablado de las diferentes restricciones al modelo por motivos teóricos, pero estos no son los únicos límites que pueden establecerse: los actuales experimentos de Detección Directa y las búsquedas de resonancias en los experimentos ATLAS y CMS del LHC pueden aportar mucha información a nuestro análisis. De este modo, las zonas sombreadas en rojo representan los puntos en los que la sección eficaz de Detección Directa está ya excluida por los actuales experimentos. Por otro lado, la zona azul es la excluida por las búsquedas de resonancias (gravitones 4-dimensionales en nuestro caso) en el LHC. Las dos líneas punteadas muestran nuestra predicción sobre los límites futuros que serán impuestos por el LHC después de las futuras fases \textit{Run-3} y \textit{High Luminosity}.

El estudio realizado muestra que, en las regiones no excluidas del espacio de parámetros, la fenomenología está dominada por los canales de interacción relacionados con los gravitones. En dichas regiones, de acuerdo con nuestro analisis, los canales de interacción radiónicos siempre son subdominantes. Para ser más exactos, la abundancia se consigue gracias a la aniquilación de Materia Oscura directamente en gravitones.

Aunque ya se habían realizado análisis similares en Randall-Sundrum, este trabajo es el primero que tiene en cuenta los canales de aniquilación de Materia Oscura directamente a gravitones en regiones tan altas del espacio de masas (varios TeV). Así mismo, se ha estudiado un canal totalmente olvidado en la literatura hasta el momento: la aniquilación a gravitones sin mediador, procedente del desarrollo a segundo orden del lagrangiano de interacción. Por otro lado, cabe destacar que este análisis únicamente se ha realizado para Materia Oscura escalar. No obstante, en la Ref.~\cite{Folgado:2020vjb} que está actualmente en trámites de publicación, se analizan los casos de Materia Oscura fermiónica y vectorial.

\subsection{Materia Oscura Mediada por Gravedad en Dimensiones Extra Tipo \textit{Clockwork/Linear Dilatón}}

Analizadas las implicaciones de la existencia de Materia Oscura tipo WIMP puramente gravitatoria en el escenario de Randall-Sundrum, la pregunta de que ocurriría en el novedoso Clockwork/Linear Dilatón casi surge de forma natural. Esta idea inspiró la Ref.~\cite{Folgado:2019gie}. Este escenario presenta más complicaciones técnicas que RS: la torre de KK de gravitones masivos en este caso tiene una separación muy pequeña e inconstante. Este hecho dificulta en gran medida el análisis numérico de su fenomenología.

A nivel conceptual, la estrategia para abordar el modelo es idéntica a la empleada en el caso RS. La gran diferencia con el modelo anterior son los parámetros elegidos para estudiar la fenomenología. En CW/LD los acoplamientos de los gravitones 4-dimensionales masivos al resto de partículas dependen de la posición del respectivo gravitón dentro de la torre. Por ello, es más útil caracterizar el modelo en función de $M_5$ directamente. Por otro lado, la masa del primer gravitón coincide prácticamente con el valor de la curvatura a lo largo de la quinta dimensión $m_{1} = k$.

\begin{figure}[htbp]
\centering
\includegraphics[width=150mm]{figures/resultados_paper_3.png}
\caption[Resultados del tercer articulo.]{\it Límites sobre Materia Oscura puramente gravitatoria en CW/LD. Las gráficas superiores muestran los resultados para el caso de Materia Oscura escalar, la inferior izquierda el caso fermiónico y la inferior derecha el vectorial. La gráfica superior izquierda muestra las diferentes zonas de exclusión teniendo en cuenta únicamente la interacción con gravitones. Por otro lado, en la gráfica superior derecha se han considerado ambas, la interacción mediante gravitones y mediante dilatones, para el caso de Materia Oscura escalar. En los casos fermiónico y vectorial no se muestra el caso sin dilatones ya que la contribución de los mismos es ínfima para los resultados. Las líneas discontinuas muestran los diferentes valores de $M_5$ en el plano ($m_\text{DM},k$) para los cuales se consigue la abundancia actual de Materia Oscura. Mientras que la zona gris muestra la región en la cual es imposible conseguir dicha abundancia, independientemente del valor de $M_5$.
Respecto a los límites sobre el modelo: la zona de cuadraditos verde representa el límite de unitariedad; la región de cuadraditos rosa representa el área en la que la teoría efectiva deja de tener validez y, finalmente, la región azul representa los límites impuestos por las búsquedas no-resonantes en el LHC.}
 \label{fig:resultados_paper_3}
\end{figure}

La Fig.~\ref{fig:resultados_paper_3} muestra los diferentes límites obtenidos para este escenario. Análogamente al caso RS, $M_5$ se ha utilizado para fijar la abundancia actual de Materia Oscura para cada punto del espacio ($m_{\text{DM}},k$). Los diferentes límites estudiados son los mismos que en el caso anterior: la región de cuadraditos rosa muestra los límites de la teoría efectiva, la región de cuadraditos verdes el límite de unitariedad y, finalmente, la zona sombreada en azul los límites impuestos por el LHC. En el caso de los límites experimentales, debido a la proximidad de las resonancias en la torre de gravitones, el límite más estricto impuesto por el LHC viene de las búsquedas en el espectro continuo de energías, en lugar de las búsquedas de resonancias. Finalmente, cabe destacar que, en este caso, los límites impuestos por las búsquedas de Detección Directa de Materia Oscura son tan pequeños que no aparecen en la región de masas seleccionada en la figura. 

Otra diferencia notable con el caso RS es que aquí no solo hay que considerar el radión, si no también toda la torre de KK de los dilatones. No obstante, en CW/LD el radión y los dilatones derivan directamente de la métrica del modelo, no es necesario un mecanismo externo para estabilizar el tamaño de la quinta dimensión. Este hecho hace que la masa de los mismos este intrínsecamente ligada a los parámetros fundamentales del modelo, sin agregar de este modo ningún grado nuevo de libertad al espacio de parámetros de la teoría.

En este trabajo se han analizado los tres posibles tipos de Materia Oscura: escalar, fermiónica y vectorial. Las dos figuras superiores corresponden al caso escalar sin tener en cuenta la torre de radión y dilatones (izquierda) y teniéndola en cuenta (derecha), respectivamente. Este es el único caso en el que los dilatones juegan un papel importante en la fenomenología del modelo y por ello merece la pena mostrar cuál es su impacto sobre los resultados finales. Las gráficas inferiores corresponden al caso fermiónico (izquierda) y al caso vectorial (derecha). Se puede ver claramente que el caso fermiónico está desfavorecido respecto a los otros dos. Este hecho se debe a que en el caso fermiónico el canal dominante, la aniquilación de Materia Oscura directamente a gravitones, sufre una supresión debido al momento angular total.

El análisis llevado a cabo en este trabajo representa el primer estudio fenomenológico del modelo CW/LD con presencia de Materia Oscura. Los resultados anteriores, al igual que en RS, son prometedores en el sentido de que toda la región no excluida podrá ser analizada en los próximos años por el LHC. Como comentario final sobre la Materia Oscura tipo WIMP púramente gravitatoria, podemos decir que en ambos escenarios es posible reproducir la abundancia actual en el rango $m_\text{DM} \in [1,10] \, \text{TeV}$. No obstante, los valores necesarios, tanto de $\Lambda$ en RS como de $M_5$ en CW/LD, para ello son excesivamente grandes como para resolver el problema de la jerarquía.

\subsection{Materia Oscura FIMP en Dimensiones Extra Deformadas}

Hasta el momento, todos los modelos analizados consideran partículas tipo WIMP. No obstante, la Materia Oscura tipo FIMP es muy interesante para el caso en el que la interacción es puramente gravitatoria. En el último proyecto incluido en esta Tesis hemos explorado la posibilidad de reproducir la abundancia de Materia Oscura actual utilizando partículas FIMP en un escenario tipo RS \cite{Bernal:2020fvw}. Este caso plantea complicaciones matematicas y numéricas muy diferentes al caso WIMP. Entre estos problemas, el más importante es que la abundancia final predicha por el modelo depende en gran medida de las condiciones iniciales. Este hecho hace que, mientras que en el caso WIMP\footnote{Como consecuencia del \textit{milagro WIMP}.} la abundancia actual se reproduze para un valor constante y fijo de la sección eficaz de interacción, en el caso FIMP es necesario resolver siempre la ecuación diferencial que fija su evolución, la conocida como ecuación de Boltzmann.

\begin{figure}[htbp]
\centering
\includegraphics[width=110mm]{figures/resultados_paper_4.pdf}
\caption[Resultados del cuarto articulo.]{\it Valores de la temperatura de reheating (lineas negras) para los cuales un determinado valor de la escala de interacción en la brana y la masa del primer graviton reproducen la abundancia de Materia Oscura actual para $m_\text{DM} = 1$ MeV y $m_r = m_1/10^3$. La zona azul representa la región excluida por las busquedas de resonancias del LHC. La región roja mustra el límite de la teoría efectiva $m_1>\Lambda$. Finalmente, la región verde muestra la zona en la que el valor de la vida media del radión entra en conflicto con las observaciones de la Nucleosíntesis del Big Bang.}
 \label{fig:resultados_paper_4}
\end{figure}

Por otro lado, aquí la abundancia también tiene una fuerte dependencia con un nuevo parametro: la temperatura máxima del Universo, conocida como temperatura de \textit{reheating}. Debido a la complejidad del espacio de parámetros, el analisis en este escenario se ha llevado a cabo para un valor determinado de la masa de la Materia Oscura: $m_{\textit{DM}} = 1$ MeV. En la Fig.~\ref{fig:resultados_paper_4} se muestran los valores necesarios de la temperatura de reheating para obtener la abundancia observada. La región azul sombreada muestra los límites experimentales impuestos por las busquedas de resonancias en el LHC (y las dos predicciones para las futuras etapas del experimento). Por otro lado, los límites teóricos en este escenario vienen determinados por la validez de la teoría efectiva (región roja) y la \textit{Nucleosíntesis del Big Bang}. Este último límite no aparecia en los modelos anteriores, se trata de una restricción sobre la vida media de los gravitones y del radión: si la $\tau>1$ s se podrían producir modificaciones en las observaciones sobre la Nucleosíntesis del Big Bang que deberían estar reflejadas en los datos experimentales actuales.

A diferencia del caso WIMP, vemos que a nivel experimental el modelo RS con FIMP está mucho menos excluido y abre todo un abanico de posiblidades para que ser explorado por futuros experimentos. Actualmente estamos trabajando en el estudio análogo para el caso CW/LD.

\subsection{Conclusión}

%En esta Tesis hemos estudiado la fenomenología de diferentes modelos de Materia Oscura, centrándonos principalmente en los candidatos de tipo WIMP. En este escenario las partículas de Materia Oscura se encontraban en equilibrio termodinámico con el resto de partículas que componen el Modelo Estándar en el Universo primigenio. A causa de su expansión, el Universo sufrió un proceso de enfriamiento y las partículas de Materia Oscura terminaron por desacoplarse del plasma primigenio, dejando un remanente que ha llegado hasta nuestros días. Este proceso es denominado como \textit{freeze-out}.


%Entre los modelos estudiados en esta Tesis, se ha explorado la posibilidad de que el problema de la Materia Oscura pueda resolverse al mismo tiempo que el de la masa de los neutrinos mediante el Portal de Neutrinos Estériles. Por la estructura del modelo, este es un candidato perfecto para ser acotado usando la Detección Indirecta. Para ello, primero se ha estudiado la posibilidad de que el exceso de fotones del centro galáctico sea consecuencia de las aniquilaciones de Materia Oscura gracias a los neutrinos Estériles. Se ha visto que, efectivamente, el exceso puede ser reproducido para un pequeño rango de masas, el cual se encuentra actualmente en tensión con otras medidas experimentales: la detección de fotones procedentes de las galaxias enanas y de antiprotones procedentes del centro galáctico. Así mismo, se ha visto que a lo largo de los próximos años la mejora de las prestaciones del experimento Fermi-LAT hará, previsiblemente, que los datos recolectados acerca de las galaxias enanas sean incompatibles con la región del espacio de parámetros en la que es posible reproducir el exceso de fotones del centro galáctico.

%Por otro lado, se ha estudiado la posibilidad de que la Materia Oscura únicamente presente interacción gravitatoria. Esta idea se sustenta en el hecho de que todas las pruebas que tenemos de la existencia de la Materia Oscura están relacionadas únicamente con la interacción gravitatoria. En 4 dimensiones, como consecuencia de la debilidad de la interacción, es imposible obtener la cantidad exacta de Materia Oscura que existe actualmente en nuestro Universo. Por este motivo hemos estudiado la viabilidad de esta idea en 5 dimensiones. Efectivamente, se ha comprobado que en espacios 5-dimensionales se puede obtener la abundancia actual de Materia Oscura utilizando únicamente interacción gravitatoria. En este contexto se han analizado dos posibles modelos de dimensiones extra: el conocido modelo Randall-Sundrum y el novedoso \textit{Clockwork/Linear Dilatón}. Los resultados obtenidos en ambos casos son muy prometedores, la abundancia de Materia Oscura se obtiene en una amplia región del espacio de parámetros que puede ser acotada utilizando los resultados del LHC. En concreto, se ha estudiado el impacto de las búsquedas resonantes y no resonantes en los detectores ATLAS y CMS excluyendo así una amplia región del espacio de parámetros de las dos teorías. Así mismo, en el caso del modelo Randall-Sundrum se ha estudiado el posible impacto de las próximas fases del LHC, viendo que la exclusión prácticamente alcanzará zonas ya eliminadas por diferentes limitaciones teóricas.

%Por último, más allá del escenario WIMP, se ha estudiado otro candidato a Materia Oscura que se caracteriza por su débil interacción, la Materia Oscura tipo FIMP. En este escenario, la Materia Oscura interacciona tan débilmente con el resto de partículas que jamás llegó a estar en equilibrio en el Universo primigenio. La abundancia de Materia Oscura medida actualmente sería consecuencia de un proceso totalmente diferente al del caso WIMP, el denominado \textit{freeze-in}. Como consecuencia de su débil interacción, la Materia Oscura tipo FIMP es un candidato perfecto si únicamente asumimos interacción gravitatoria. En este contexto se ha estudiado la posibilidad de obtener la abundancia de Materia Oscura en el escenario de Randall-Sundrum 5-dimensional. Nuestro análisis muestra que la región del espacio de parámetros de la teoría en la cual es posible reproducir la abundancia actual de Materia Oscura es enorme. Las diferentes cotas experimentales y teóricas limitan mucho menos el espacio de parámetros que en el caso WIMP. Así mismo, las previsiones sobre los futuros límites impuestos por el LHC apenas restringen la región permitida. De este modo, el candidato FIMP es más prometedor que el candidato WIMP en el escenario de Randall-Sundrum y la inaccesibilidad del LHC a ciertas regiones permitidas del espacio de parámetros representan una motivación para nuevos experimentos de física de altas energías.

Nuestro escaso conocimiento acerca de la naturaleza de la Materia Oscura hace que el conjunto de modelos que pueden explicar las evidencias actuales sea enorme. Esta Tesis ha contribuido a explorar parte de estos modelos y acotar un poco más lo que sabemos de ella, estudiando la fenomenología de diferentes candidatos. En general, los resultados obtenidos hacen que esperemos con ansia los resultados de los experimentos futuros, tanto en materia de Detección Indirecta, como en búsquedas del LHC. La relevancia de estos futuros datos es tal que en los próximos años la existencia de los candidatos de tipo WIMP y FIMP puede verse corroborada o seriamente comprometida. Por otro lado, la débil interacción de los candidatos de tipo FIMP hace que su futuro experimental sea bastante más incierto. Como comentario final, es cierto que los modelos aquí estudiados representan una ínfima parte de todo el abanico de posibilidades existentes en la actualidad para explicar este escurridizo tipo de materia. No obstante, espero que hayan arrojado algo de luz sobre tan oscuro misterio.

%Nuestro escaso conocimiento acerca de la naturaleza de la Materia Oscura hace que el conjunto de modelos que pueden explicar las evidencias actuales sea enorme. Esta Tesis ha contribuido a explorar parte de estos modelos y acotar un poco más lo que sabemos de ella, estudiando la fenomenología de diferentes candidatos. En general, los resultados obtenidos hacen que tengamos un ojo puesto en los experimentos futuros, tanto en materia de Detección Indirecta, como en búsquedas del LHC. La relevancia de estos futuros datos es tal que en los próximos años la existencia de los candidatos de tipo WIMP y FIMP puede verse corroborada o seriamente comprometida. Como comentario final, es cierto que los modelos aquí estudiados representan una ínfima parte de todo el abanico de posibilidades existentes en la actualidad para explicar este escurridizo tipo de materia. No obstante, espero que hayan arrojado algo de luz sobre tan oscuro misterio.

